Standard Model Physics at the HL-LHC and HE-LHC

The successful operation of the Large Hadron Collider (LHC) and the excellent performance of the ATLAS, CMS, LHCb and ALICE detectors in Run-1 and Run-2 with $pp$ collisions at center-of-mass energies of 7, 8 and 13 TeV as well as the giant leap in precision calculations and modeling of fundamental interactions at hadron colliders have allowed an extraordinary breadth of physics studies including precision measurements of a variety physics processes. The LHC results have so far confirmed the validity of the Standard Model of particle physics up to unprecedented energy scales and with great precision in the sectors of strong and electroweak interactions as well as flavour physics, for instance in top quark physics. The upgrade of the LHC to a High Luminosity phase (HL-LHC) at 14 TeV center-of-mass energy with 3 ab$^{-1}$ of integrated luminosity will probe the Standard Model with even greater precision and will extend the sensitivity to possible anomalies in the Standard Model, thanks to a ten-fold larger data set, upgraded detectors and expected improvements in the theoretical understanding. This document summarises the physics reach of the HL-LHC in the realm of strong and electroweak interactions and top quark physics, and provides a glimpse of the potential of a possible further upgrade of the LHC to a 27 TeV $pp$ collider, the High-Energy LHC (HE-LHC), assumed to accumulate an integrated luminosity of 15 ab$^{-1}$.

==> authors_empty.tex <==
\author{{\bf Editors} \\
{\rm 
Patrizia Azzi$^1$, Stephen Farry$^2$, Paolo Nason$^3$, Alessandro Tricoli$^4$, Dieter Zeppenfeld$^5$ 
}
\\
{\bf LIST OF CONTRIBUTORS IS BEING COMPILED} 
}
\institute{
$^1$ INFN, Padova, Italy, $^2$ University of Liverpool, U.K.$^3$ INFN, sez. di Milano Bicocca, Università di Milano-Bicocca, Italy, $^4$ Brookhaven National Laboratory, U.S.A., 
$^5$ Institut für Theoretische Physik, Karlsruher Institut für Technologie, Germany}


==> authors_firstcirculation.tex <==
\author{Editors: \\
P. Azzi$^{1}$
, S. Farry$^{2}$
, P. Nason$^{3,67}$
, A. Tricoli$^{4}$
, D. Zeppenfeld$^{5}$
\\ \vspace*{4mm} 
 Contributors: 
 \\ R. Abdul Khalek$^{6}$
, J. Alimena$^{7}$
, N. Andari$^{8}$
, L. Aperio Bella$^{9}$
, A.J. Armbruster$^{9}$
, J. Baglio$^{10}$
, S.  Bailey$^{11}$
, E. Bakos$^{12}$
, A. Bakshi$^{13}$
, C. Baldenegro$^{14}$
, F. Balli$^{8}$
, A. Barker$^{13}$
, W. Barter$^{15}$
, J. de Blas$^{16}$
$^{,1}$
, F. Blekman$^{17}$
, D. Bloch$^{18}$
, A.  Bodek$^{19}$
, M. Boonekamp$^{8}$
, E. Boos$^{20}$
, J.D. Bossio Sola$^{21}$
, L. Cadamuro$^{22}$
, S. Camarda$^{9}$
, F. Campanario$^{23}$
, M. Campanelli$^{24}$
, Q.-H. Cao$^{25}$
, V. Cavaliere$^{4}$
, A. Cerri$^{26}$
, G.S. Chahal$^{15,56}$
, B. Chargeishvili$^{27}$
, C. Charlot$^{28}$
, S.-L. Chen$^{29}$
, T. Chen$^{30}$
, L. Cieri$^{3}$
, M. Ciuchini$^{31}$
, G. Corcella$^{32}$
, J.M. Cruz-Martinez$^{33}$
, M. Czakon$^{34}$
, A. Dainese$^{1}$
, N.P. Dang$^{35}$
, L. Darm{\'e}$^{36}$
, S. Dawson$^{4}$
, H. De la Torre$^{37}$
, M. Deile$^{9}$
, F. Deliot$^{8}$
, S. Demers$^{38}$
, A. Denner$^{39}$
, F. Derue$^{40}$
, L. Di Ciaccio$^{41}$
, W.K. Di Clemente$^{42}$
, D. Dominguez Damiani$^{43}$
, L. Dudko$^{20}$
, A. Durglishvili$^{27}$
, M.  D{\"u}nser$^{9}$
, J. Ebadi$^{44}$
, R. B. Ferreira De Faria$^{45}$
, G. Ferrera$^{33,100}$
, A. Ferroglia$^{99}$
, T. M. Figy$^{30}$
, K.D. Finelli$^{46}$
, M.C.N. Fiolhais$^{45}$
, E. Franco$^{47}$
, R. Frederix$^{48}$
, B. Fuks$^{49,50}$
, B. Galhardo$^{45}$
, J. Gao$^{51}$
, J. R.  Gaunt$^{9}$
, T. Gehrmann$^{52}$
, A. Gehrmann-De Ridder$^{53}$
, J. Giljanovic$^{54}$
, F. Giuli$^{55}$
, E.W.N. Glover$^{56}$
, M. D. Goodsell$^{49}$
, E. Gouveia$^{45}$
, C. Goy$^{41}$
, M. Grazzini$^{52}$
, J.F. Grosse-Oetringhaus$^{9}$
, P. Gunnellini$^{57}$
, C. Gwenlan$^{11}$
, L. A. Harland-Lang$^{11}$
, P.F. Harrison$^{58}$
, G. Heinrich$^{59}$
, C. Helsens$^{9}$
, C. Helsens$^{9}$
, M. Herndon$^{60}$
, O. Hindrichs$^{61}$
, A. Hoang$^{62}$
, K. Hoepfner$^{34}$
, J.M. Hogan$^{63}$
$^{,64}$
, A. Huss$^{9}$
%AT, G. Isidori$^{52}$
, S. Jahn$^{65}$
, Sa. Jain$^{66}$
, S. P. Jones$^{9}$
, A.W. Jung$^{13}$
, H. Jung$^{43}$
, S. Kallweit$^{67}$
, D. Kar$^{68}$
, A. Karlberg$^{52}$
, M. Kerner$^{52}$
, M.K. Khandoga$^{8}$
, Hamzeh Khanpour$^{69}$
, S. Khatibi$^{70}$
, A.  Khukhunaushvili$^{71}$
, J. Kieseler$^{9}$
%AT, F. Krauss$^{56}$
, J. Kretzschmar$^{2}$
, J. Kroll$^{42}$
, E. Kryshen$^{72}$
, V.S. Lang$^{43}$
, L. Lechner$^{73}$
, C.A. Lee$^{4}$
, M. Leigh$^{74}$
, D. Lelas$^{47}$
, R. Les$^{75}$
, I. M. Lewis$^{14}$
, B. Li$^{37}$
, Y. Li$^{43}$
, J. Lidrych$^{43}$
%AT, Z. Ligeti$^{76}$
, J.M. Lindert$^{56}$
, Y. Liu$^{77}$
, K. Lohwasser$^{78}$
, K. Long$^{60}$
, D. Lontkovskyi$^{17}$
, G. Majumder$^{66}$
, M. Mancini$^{17}$
, P. Mandrik$^{79}$
, M.L. Mangano$^{9}$
, I. Marchesini$^{17}$
, C. Mayer$^{80}$
, K. Mazumdar$^{66}$
, J.A. McFayden$^{9}$
, P. M. Mendes Amaral Torres Lagarelhos$^{45}$
, A.B. Meyer$^{43}$
, S. Mikhalcov$^{81}$
, S. Mishima$^{82}$
, A. Mitov$^{83}$
, M. Mohammadi Najafabadi$^{44}$
, M. Moreno Ll{\'a}cer$^{9}$
, M. Mulders$^{9}$
, M. Narain$^{63}$
, A. Nisati$^{47}$
, T. Nitta$^{84}$
, A. Onofre$^{85}$
, S. Pagan Griso$^{76}$
, D. Pagani$^{48}$
, A. Papanastasiou$^{83}$
, K. Pedro$^{86}$
, M. Pellen$^{83}$
, M. Perfilov$^{20}$
, B.A. Petersen$^{9}$
, M. Pierini$^{9}$
, J. Pires$^{87}$
, M.-A. Pleier$^{4}$
, S. Pl{\"a}tzer$^{62}$
, K. Potamianos$^{43}$
, S. Pozzorini$^{52}$
, A. C. Price$^{56}$
, M. Rauch$^{5}$
, E. Re$^{9}$
$^{,88}$
, L. Reina$^{89}$
, J. Reuter$^{43}$
, J. Rojo$^{90}$
, C. Royon$^{14}$
, A. Savin$^{60}$
, S. Sawant$^{66}$
, B. Schneider$^{86}$
, R. Schoefbeck$^{73}$
, M. Schoenherr$^{9}$
, H. Sch{\"a}fer-Siebert$^{5}$
, M.  Seidel$^{9}$
, T. Shears$^{2}$
, L. Silvestrini$^{47}$
$^{,9}$
, M. Sjodahl$^{91}$
, K. Skovpen$^{17}$
, D. Spitzbart$^{73}$
, P. Starovoitov$^{92}$
, C. J. E. Suster$^{93}$
, P. Tan$^{86}$
, R.  Taus$^{19}$
, D. Teague$^{60}$
, K. Terashi$^{94}$
, J. Terron$^{95}$
, S. Uplap$^{66}$
, F. Veloso$^{45}$
, M. Verzetti$^{52}$
, M. A. Vesterinen$^{58}$
, V.E. Vladimirov$^{58}$
, P. Volkov$^{20}$
, G. Vorotnikov$^{20}$
, M. Vranjes Milosavljevic$^{12}$
, N. Vranjes$^{12}$
, E. Vryonidou$^{9}$
, D. Walker$^{56}$
, M. Wiesemann$^{9}$
, Y. Wu$^{96}$
, T. Xu$^{8}$
, S. Yacoob$^{74}$
, H. Yokoya$^{101}$
, J. Zahreddine$^{40}$
, G. Zanderighi$^{11}$
, M. Zaro$^{90}$
, O. Zenaiev$^{43}$
, G. Zevi Della Porta$^{97}$
, C. Zhang$^{98}$
, W. Zhang$^{63}$
, H. Zhu$^{96}$
, H.L. Zhu$^{96}$
, R. Zlebcik$^{43}$
, F. N. Zubair$^{9}$
%AT---missing in above list, should we add him (EFT contribution) --- Duarte Azevedo ---
\vspace*{1cm} 
 }
\institute{
\small $^{1}$ Sezione di Padova, Istituto Nazionale di Fisica Nucleare (INFN)
, $^{2}$ Department of Physics, University of Liverpool
, $^{3}$ Sezione di Milano-Bicocca, Istituto Nazionale di Fisica Nucleare (INFN)
, $^{4}$ Department of Physics, Brookhaven National Laboratory (BNL)
, $^{5}$ Institut f{\"u}r Theoretische Physik (TP), Karlsruher Institut f{\"u}r Technologie (KIT)
, $^{6}$ Department of Physics and Astronomy, Vrije University
, $^{7}$ Ohio State University (OSU)
, $^{8}$ Universit{\'e} Paris-Saclay
, $^{9}$ European Organization for Nuclear Research (CERN)
, $^{10}$ Fachbereich Physik, Eberhard Karls Universit{\"a}t T{\"u}bingen
, $^{11}$ University of Oxford
, $^{12}$ Institute of Physics Belgrade
, $^{13}$ Purdue University
, $^{14}$ Department of Physics and Astronomy, University of Kansas
, $^{15}$ Department of Physics, Imperial College London
, $^{16}$ Dipartimento di Fisica, Universit{\`a} degli Studi di Padova
, $^{17}$ Department of Physics and Astrophysics (DNTK), Vrije Universiteit Brussel (VUB)
, $^{18}$ Institut Pluridisciplinaire Hubert Curien (IPHC)
, $^{19}$ Rochester University
, $^{20}$ Skobeltsyn Institute of Nuclear Physics (SINP), Lomonosov Moscow State University
, $^{21}$ Departamento de Fisica, Universidad de Buenos Aires
, $^{22}$ Department of Physics, University of Florida
, $^{23}$ Universitat de Valencia-CSIC
, $^{24}$ Department of Physics {\&} Astronomy, University College London
, $^{25}$ School of Physics, Peking University
, $^{26}$ Department of Physics and Astronomy, University of Sussex
, $^{27}$ High Energy Physics Institute (HEPI-TSU), Ivane Javakhishvili Tbilisi State University
, $^{28}$ Laboratoire Leprince-Ringuet (LLR)
, $^{29}$ Institute of Particle Physics, Central China Normal University (CCNU)
, $^{30}$ Department of Mathematics, Statistics, and Physics, Wichita State University, Wichita
, $^{31}$ Sezione di Roma Tre, Istituto Nazionale di Fisica Nucleare (INFN)
, $^{32}$ Laboratori Nazionali di Frascati (LNF), Istituto Nazionale di Fisica Nucleare (INFN)
, $^{33}$ Dipartimento di Fisica, Universit{\`a} degli Studi di Milano
, $^{34}$ Rheinisch-Westf{\"a}lische Technische Hochschule (RWTH) Aachen
, $^{35}$ Department of Physics, University of Louisville
, $^{36}$ Narodowe Centrum Bada{\'n} J{\k{a}}drowych (NCBJ)
, $^{37}$ Department of Physics, University of Michigan
, $^{38}$ Department of Physics, Yale University
, $^{39}$ Department of Physics and Astronomy, Julius Maximilian University W{\"u}rzburg
, $^{40}$ Laboratoire de Physique Nucl{\'e}aire et de Hautes Energies (LPNHE)
, $^{41}$ LAPP, Universit{\'e} Grenoble Alpes, Universit{\'e} Savoie Mont-Blanc, CNRS/IN2P3, Annecy, France
, $^{42}$ Department of Physics {\&} Astronomy, University of Pennsylvania
, $^{43}$ Deutsches Elektronen-Synchrotron  (DESY)
, $^{44}$ Institute for Research in Fundamental Sciences (IPM)
, $^{45}$ Laboratorio de Instrumentacao e Fisica Experimental de Particulas (LIP)
, $^{46}$ Department of Physics, Boston University
, $^{47}$ Sezione di Roma, Istituto Nazionale di Fisica Nucleare (INFN)
, $^{48}$ Fakult{\"a}t f{\"u}r Physik, Technische Universit{\"a}t M{\"u}nchen (TUM)
, $^{49}$ Sorbonne Universit{\'e}, CNRS, Laboratoire de Physique Th{\'e}orique et Hautes {\'E}nergies, LPTHE, F-75005 Paris, France
, $^{50}$ Institut Universitaire de France, 103 boulevard Saint-Michel, 75005 Paris, France
, $^{51}$ Department of Physis, Shanghai Jiao Tong University
, $^{52}$ Physik-Institut, Universit{\"a}t Z{\"u}rich
, $^{53}$ Departement Physik (D-PHYS), Eidgen{\"o}ssische Technische Hochschule (ETH) Z{\"u}rich
, $^{54}$ Faculty of Electrical Engineering, Mechanical Engineering and Naval Architecture in Split (FESB), University of Split
, $^{55}$ Dipartimento di Fisica, Universit{\`a} degli Studi di Roma ''Tor Vergata''
, $^{56}$ Institute for Particle Physics Phenomenology, University of Durham, UK
, $^{57}$ Fakult{\"a}t f{\"u}r Physik, Institut f{\"u}r Experimentalphysik (IExpPh), Universit{\"a}t Hamburg
, $^{58}$ Department of Physics, The University of Warwick
, $^{59}$ Werner-Heisenberg-Institut, Max-Planck-Institut f{\"u}r Physik
, $^{60}$ Department of Physics, University of Wisconsin
, $^{61}$ Department of Physics and Astronomy, University of Rochester
, $^{62}$ Theoretische Physik, Universit{\"a}t Wien
, $^{63}$ Department of Physics, Brown University
, $^{64}$ Bethel University, St. Paul, USA
, $^{65}$ Max-Planck-Institut f{\"u}r Kernphysik
, $^{66}$ Department of High Energy Physics (DHEP), Tata institute of fundamental research (TIFR)
, $^{67}$ Dipartimento di Fisica ''G. Occhialini'', Universit{\`a} degli studi di  Milano Bicocca
, $^{68}$ University of the Witwatersrand
, $^{69}$ Department of Physics, University of Science and Technology of Mazandaran
, $^{70}$ Department of Physics, University of Tehran
, $^{71}$ Cornell University
, $^{72}$ Petersburg Nuclear Physics Institute (PNPI)
, $^{73}$ {\"O}sterreichische Akademie der Wissenschaft (OEAW)
, $^{74}$ Department of Physics, University of Cape Town
, $^{75}$ Department of Physics, University of Toronto
, $^{76}$ Physics Division, Lawrence Berkeley National Laboratory (LBNL)
, $^{77}$ College of Nuclear Science and Technology, Beijing Normal University (BNU)
, $^{78}$ Department of Physics and Astronomy, University of Sheffield
, $^{79}$ Institute of High Energy Physics (IHEP)
, $^{80}$ The Henryk Niewodnicza{\'n}ski Institute of Nuclear Physics (IFJ), Polish Academy of Sciences (PAN)
, $^{81}$ Research Institute for Nuclear Problems of Byelorussian State University
, $^{82}$ High Energy Accelerator Research Organization (KEK)
, $^{83}$ Cavendish Laboratory, University of Cambridge
, $^{84}$ Department of Physics, Waseda University
, $^{85}$ Department of Mathematics, Univerisdade do Minho
, $^{86}$ Fermi National Accelerator Laboratory (FNAL)
, $^{87}$ CFTP, Instituto Superior T{\'e}cnico, Universidade de Lisboa
, $^{88}$ Laboratoire d'Annecy-le-Vieux de Physique Th{\'e}orique (LAPTH)
, $^{89}$ Physics Department, Florida State University
, $^{90}$ National Institute for Subatomic Physics (NIKHEF)
, $^{91}$ Department of Physics, Division of Particle Physics, Lund University
, $^{92}$ Ruprecht-Karls-Universit{\"a}t Heidelberg
, $^{93}$ School of Physics, University of Sydney
, $^{94}$ International Center for Elementary Particle Physics (ICEPP), University of Tokyo
, $^{95}$ Departamento de F{\'\i}sica Te{\'o}rica, Universidad Autonoma de Madrid (UAM)
, $^{96}$ Department of Modern Physics (DMP), University of Science and Technology of China (USTC)
, $^{97}$ University of California, San Diego, La Jolla, USA
, $^{98}$ Institute of High Energy Physics (IHEP), Chinese Academy of Sciences (CAS)
, $^{99}$ Physics Department, New York City College of Technology, CUNY, 300 Jay Street, Brooklyn, NY 11201 USA
, $^{100}$ Sezione di Milano, Istituto Nazionale di Fisica Nucleare (INFN)
, $^{101}$ Korea Inst. Advanced Study, Seoul
}


==> authors_old.tex <==
\author{Editors: \\P. Azzi$^{1}$, S. Farry$^{2}$, P. Nason$^{3,4}$, A. Tricoli$^{5}$, D. Zeppenfeld$^{6}$
\\ \vspace*{4mm} 
Contributors: 
\\ R. Abdul Khalek$^{7,8}$, J. Alimena$^{9}$, N. Andari$^{10}$, L. Aperio Bella$^{11}$, A.J. Armbruster$^{11}$, J. Baglio$^{12}$, S.  Bailey$^{13}$, E. Bakos$^{14}$, A. Bakshi$^{15}$, C. Baldenegro$^{16}$, F. Balli$^{17}$, A. Barker$^{15}$, W. Barter$^{18}$, J. de Blas$^{19,1}$, F. Blekman$^{20}$, D. Bloch$^{21}$, A.  Bodek$^{22}$, M. Boonekamp$^{17}$, E. Boos$^{23}$, J.D. Bossio Sola$^{24}$, L. Cadamuro$^{25}$, S. Camarda$^{11}$, F. Campanario$^{26}$, M. Campanelli$^{27}$, J.M. Campbell$^{28}$, Q.-H. Cao$^{29,30,31}$, V. Cavaliere$^{5}$, A. Cerri$^{32}$, G.S. Chahal$^{18,33}$, B. Chargeishvili$^{34}$, C. Charlot$^{35}$, S.-L. Chen$^{36}$, T. Chen$^{37}$, L. Cieri$^{3}$, M. Ciuchini$^{38}$, G. Corcella$^{39}$, R. Covarelli$^{40,41}$, J.M. Cruz-Martinez$^{42}$, M. Czakon$^{43}$, A. Dainese$^{1}$, N.P. Dang$^{44}$, L. Darm{\'e}$^{45}$, S. Dawson$^{5}$, H. De la Torre$^{46}$, M. Deile$^{11}$, F. Deliot$^{17}$, S. Demers$^{47}$, A. Denner$^{48}$, F. Derue$^{49}$, L. Di Ciaccio$^{50}$, W.K. Di Clemente$^{51}$, D. Dominguez Damiani$^{52}$, L. Dudko$^{23}$, A. Durglishvili$^{34}$, M. D{\"u}nser$^{11}$, J. Ebadi$^{53}$, R.B. Ferreira De Faria$^{54}$, G. Ferrera$^{42,55}$, A. Ferroglia$^{56}$, T.M. Figy$^{37}$, K.D. Finelli$^{57}$, M.C.N. Fiolhais$^{58,54}$, E. Franco$^{59}$, R. Frederix$^{60}$, B. Fuks$^{61,62}$, B. Galhardo$^{54,63}$, J. Gao$^{64}$, J.R. Gaunt$^{11}$, T. Gehrmann$^{65}$, A. Gehrmann-De Ridder$^{66}$, D. Giljanovic$^{67,35}$, F. Giuli$^{68}$, E.W.N. Glover$^{33}$, M.D. Goodsell$^{69}$, E. Gouveia$^{54}$, P. Govoni$^{3,4}$, C. Goy$^{50}$, M. Grazzini$^{65}$, A. Grohsjean$^{52}$, J.F. Grosse-Oetringhaus$^{11}$, P. Gunnellini$^{70}$, C. Gwenlan$^{71}$, L.A. Harland-Lang$^{13}$, P.F. Harrison$^{72}$, G. Heinrich$^{73}$, C. Helsens$^{11}$, M. Herndon$^{74}$, O. Hindrichs$^{75}$, V. Hirschi$^{66}$, A. Hoang$^{76}$, K. Hoepfner$^{43}$, J.M. Hogan$^{77,78}$, A. Huss$^{11}$, S. Jahn$^{79}$, Sa. Jain$^{80}$, S.P. Jones$^{11}$, A.W. Jung$^{15}$, H. Jung$^{52}$, S. Kallweit$^{4}$, D. Kar$^{81}$, A. Karlberg$^{65}$, M. Kerner$^{65}$, M.K. Khandoga$^{17}$, H. Khanpour$^{82}$, S. Khatibi$^{83}$, A. Khukhunaishvili$^{84}$, J. Kieseler$^{11}$, J. Kretzschmar$^{2}$, J. Kroll$^{51}$, E. Kryshen$^{85}$, V.S. Lang$^{52}$, L. Lechner$^{86}$, C.A. Lee$^{5}$, M. Leigh$^{87}$, D. Lelas$^{59}$, R. Les$^{88}$, I.M. Lewis$^{16}$, B. Li$^{89}$, Q. Li$^{90}$, Y. Li$^{91}$, J. Lidrych$^{52}$, Z. Ligeti$^{92}$, J.M. Lindert$^{93,33}$, Y. Liu$^{94}$, K. Lohwasser$^{95}$, K. Long$^{74}$, D. Lontkovskyi$^{20}$, G. Majumder$^{80}$, M. Mancini$^{20}$, P. Mandrik$^{96}$, M.L. Mangano$^{11}$, I. Marchesini$^{20}$, C. Mayer$^{97}$, K. Mazumdar$^{80}$, J.A. McFayden$^{11}$, P.M. Mendes Amaral Torres Lagarelhos$^{54}$, A.B. Meyer$^{52}$, S. Mikhalcov$^{98}$, S. Mishima$^{99}$, A. Mitov$^{100}$, M. Mohammadi Najafabadi$^{53}$, M. Moreno Ll{\'a}cer$^{11}$, M. Mulders$^{11}$, M. Narain$^{78}$, A. Nisati$^{59,101}$, T. Nitta$^{102}$, A. Onofre$^{103}$, S. Pagan Griso$^{92,104}$, D. Pagani$^{60}$, E. Palencia Cortezon$^{105}$, A. Papanastasiou$^{100}$, K. Pedro$^{28}$, M. Pellen$^{100}$, M. Perfilov$^{23}$, L. Perrozzi$^{66}$, B.A. Petersen$^{11}$, M. Pierini$^{11}$, J. Pires$^{106}$, M.-A. Pleier$^{5}$, S. Pl{\"a}tzer$^{76}$, K. Potamianos$^{91}$, S. Pozzorini$^{65}$, A.C. Price$^{93}$, M. Rauch$^{6}$, E. Re$^{11,107}$, L. Reina$^{108}$, J. Reuter$^{52}$, J. Rojo$^{8}$, C. Royon$^{16}$, S. Saito$^{80}$, A. Savin$^{74}$, S. Sawant$^{80}$, B. Schneider$^{28}$, R. Schoefbeck$^{86}$, M. Schoenherr$^{33,11}$, H. Sch{\"a}fer-Siebert$^{6}$, M. Seidel$^{11}$, M. Selvaggi$^{11}$, T. Shears$^{2}$, L. Silvestrini$^{59,11}$, M. Sjodahl$^{109}$, K. Skovpen$^{20}$, N. Smith$^{28}$, D. Spitzbart$^{86}$, P. Starovoitov$^{110}$, C.J.E. Suster$^{111}$, P. Tan$^{28}$, R. Taus$^{22}$, D. Teague$^{74}$, K. Terashi$^{112}$, J. Terron$^{113}$, S. Uplap$^{80}$, F. Veloso$^{54}$, M. Verzetti$^{65}$, M.A. Vesterinen$^{72}$, V.E. Vladimirov$^{72}$, P. Volkov$^{23}$, G. Vorotnikov$^{23}$, M. Vranjes Milosavljevic$^{14}$, N. Vranjes$^{14}$, E. Vryonidou$^{11}$, D. Walker$^{93}$, M. Wiesemann$^{11}$, Y. Wu$^{114}$, T. Xu$^{10}$, S. Yacoob$^{87}$, E. Yazgan$^{115}$, J. Zahreddine$^{49}$, G. Zanderighi$^{11,73}$, M. Zaro$^{8}$, O. Zenaiev$^{52}$, G. Zevi Della Porta$^{116}$, C. Zhang$^{115}$, W. Zhang$^{78}$, H.L. Zhu$^{114,5}$, R. Zlebcik$^{52}$, F.N. Zubair$^{11}$
\vspace*{1cm} 
}
\institute{$^{1}$~INFN Sezione di Padova, Padova, Italy \\$^{2}$~Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom \\$^{3}$~INFN Sezione di Milano-Bicocca, Milano, Italy \\$^{4}$~Universit{\`a} degli Studi di Milano-Bicocca, Dipartimento di Fisica ''G.Occhialini'', Piazza della Scienza 3, 20126 Milan, Italy \\$^{5}$~Brookhaven National Laboratory (BNL) \\$^{6}$~Karlsruher Institut f{\"u}r Technologie (KIT), Institut f{\"u}r Theoretische Physik (TP), Wolfgang-Gaede-Str. 1, 76131 Karlsruhe, Germany \\$^{7}$~Department of Physics and Astronomy, VU University, NL-1081 HV Amsterdam \\$^{8}$~Nikhef National Institute for Subatomic Physics, Amsterdam, Netherlands \\$^{9}$~The Ohio State University, Columbus, USA \\$^{10}$~IRFU, CEA, Universit{\'e} Paris-Saclay \\$^{11}$~European Laboratory for Particle Physics, CERN \\$^{12}$~Institut for Theoretical Physics, Eberhard Karls University T{\"u}bingen, Auf der Morgenstelle 14, D-72076 T{\"u}bingen, Germany \\$^{13}$~Rudolf Peierls Centre, Beecroft Building, Parks Road, Oxford, OX1 3PU \\$^{14}$~Institute of Physics, University of Belgrade \\$^{15}$~Purdue University, West Lafayette, USA \\$^{16}$~The University of Kansas, Lawrence, USA \\$^{17}$~IRFU, CEA, Universit{\'e} Paris-Saclay \\$^{18}$~Imperial College, London, United Kingdom \\$^{19}$~Universit{\`a} di Padova, Padova, Italy \\$^{20}$~Vrije Universiteit Brussel, Brussel, Belgium \\$^{21}$~Universit{\'e} de Strasbourg, CNRS, IPHC UMR 7178, Strasbourg, France \\$^{22}$~University of Rochester, Rochester, NY, USA \\$^{23}$~Skobeltsyn Institute of Nuclear Physics, Lomonosov Moscow State University, Moscow, Russia \\$^{24}$~Universidad de Buenos Aires \\$^{25}$~University of Florida, Gainesville, USA \\$^{26}$~Theory Division, IFIC, University of Valencia-CSIC, E-46980 Paterna, Valencia, Spain \\$^{27}$~Department of Physics and Astronomy, University College London \\$^{28}$~Fermi National Accelerator Laboratory, P.O. Box 500 Batavia, 60510 USA \\$^{29}$~Department of Physics and State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing 100871, China \\$^{30}$~ Collaborative Innovation Center of Quantum Matter, Beijing 100871, China \\$^{31}$~ Center for High Energy Physics, Peking University, Beijing 100871, China \\$^{32}$~Department of Physics and Astronomy, University of Sussex, Brighton, United Kingdom \\$^{33}$~Institute for Particle Physics Phenomenology, University of Durham, Durham, UK \\$^{34}$~High Energy Physics Institute of Tbilisi State University \\$^{35}$~LLR, Ecole polytechnique, CNRS/IN2P3, Universit{\'e} Paris-Saclay, Palaiseau, France \\$^{36}$~Key Laboratory of Quark and Lepton Physics (MoE) and Institute of Particle Physics, Central China Normal University, China \\$^{37}$~Department of Mathematics, Statistics, and Physics, Wichita State University, Wichita, KS, 67260, USA \\$^{38}$~INFN Sezione di Roma Tre, Via della Vasca Navale 84, I-00146 Roma, Italy \\$^{39}$~INFN, Laboratori Nazionali di Frascati, Frascati (RM), Italy \\$^{40}$~ Istituto Nazionale di Fisica Nucleare (INFN) Sezione di Torino , Italy \\$^{41}$~ Universit{\`a} di Torino, Torino, Italy \\$^{42}$~ Universita' di Milano, Dipartimento di Fisica \\$^{43}$~RWTH Aachen University, III. Physikalisches Institut A, Aachen, Germany \\$^{44}$~University of Louisville \\$^{45}$~Narodowe Centrum Bada{\'n} J{\k{a}}drowych (NCBJ), Ho{\.z}a 69, 00-681 Warszawa, Poland \\$^{46}$~Michigan State University, Department of Physics and Astronomy \\$^{47}$~Department of Physics, Yale University, New Haven CT, United States of America \\$^{48}$~Universit{\"a}t W{\"u}rzburg, Institut f{\"u}r Theoretische Physik und Astrophysik, Emil-Hilb-Weg 22, 97074 W{\"u}rzburg, Germany \\$^{49}$~Laboratoire de Physique Nucl{\'e}aire et de Hautes Energies (LPNHE), Sorbonne Universit{\'e}, Paris-Diderot Sorbonne Paris Cit{\'e}, CNRS/IN2P3 \\$^{50}$~LAPP, Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS/IN2P3, Annecy \\$^{51}$~Department of Physics and Astronomy, University of Pennsylvania \\$^{52}$~Deutsches Elektronen-Synchrotron, Hamburg, Germany \\$^{53}$~School of Physics, Institute for Research in Fundamental Sciences (IPM), P.O. Box 19395-5531, Tehran, Iran \\$^{54}$~Laborat{\'o}rio de Instrumenta{\c{c}}{\~a}o e F{\'\i}sica Experimental de Part{\'\i}culas - LIP, Lisboa \\$^{55}$~INFN, Sezione di Milano, Via Celoria 16, I-20133 Milan, Italy \\$^{56}$~Physics Department, New York City College of Technology, CUNY, 300 Jay Street, Brooklyn, NY 11201 USA \\$^{57}$~Boston University, Department of Physics \\$^{58}$~Science Department, Borough of Manhattan Community College, New York, NY 10007, USA and LIP, Lisboa \\$^{59}$~INFN Roma I \\$^{60}$~Technische Universit{\"a}t M{\"u}nchen \\$^{61}$~Laboratoire de Physique Th{\'e}orique et Hautes {\'E}nergies (LPTHE), Boite 126, T13-14 4{\`e}me {\'e}tage, 4 place Jussieu, F-75252 Paris CEDEX 05, France \\$^{62}$~Institut Universitaire de France, 103 boulevard Saint-Michel, 75005 Paris, France \\$^{63}$~Laborat{\'o}rio de Instrumenta{\c{c}}{\~a}o e F{\'\i}sica Experimental de Part{\'\i}culas - LIP, Coimbria \\$^{64}$~School of Physics and Astronomy, Shanghai Jiao Tong University, Shanghai, China \\$^{65}$~Physik-Institut, Universitaet Zurich, 8057 Zurich, Switzerland \\$^{66}$~Department of Physics, ETH Zurich, CH-8093 Zurich, Switzerland \\$^{67}$~University of Split, Split, Croatia \\$^{68}$~Universit{\`a} di Roma Tor Vergata, Dipartimento di Fisica, Roma, Italy \\$^{69}$~Laboratoire de Physique Theorique et Hautes Energies, UMR 7589, Sorbonne Universit{\'e} et CNRS, Bo{\^\i}te 126, T13-14 4{\`e}me {\'e}tage, 4 place Jussieu, F-75252 Paris CEDEX 05, France \\$^{70}$~University of Hamburg, Hamburg, Germany \\$^{71}$~Denys Wilkinson Building, University of Oxford, Oxford, OX1 3RH \\$^{72}$~Department of Physics, University of Warwick, Coventry, United Kingdom \\$^{73}$~Max Planck Institute for Physics, Foehringer Ring 6, 80805 Munich, Germany \\$^{74}$~University of Wisconsin - Madison, Madison, USA \\$^{75}$~University of Rochester, Rochester, USA \\$^{76}$~University of Vienna, Vienna, Austria \\$^{77}$~Bethel University, St. Paul, USA \\$^{78}$~Brown University, Providence, USA \\$^{79}$~Max Planck Institute for Physics, Foehringer Ring 6, 80805 Munich, Germany \\$^{80}$~Tata Institute of Fundamental Research, Mumbai, India \\$^{81}$~School of Physics, University of the Witwatersrand \\$^{82}$~Department of Physics, University of Science and Technology of Mazandaran, P.O.Box 48518-78195, Behshahr, IRAN \\$^{83}$~Department of Physics, University of Tehran, North Karegar Ave., Tehran 14395-547, Iran \\$^{84}$~Cornell University, PHysics Department, Ithaca, NY, USA \\$^{85}$~Petersburg Nuclear Physics Institute (PNPI) Gatchina \\$^{86}$~Institut f{\"u}r Hochenergiephysik, Wien, Austria \\$^{87}$~University of Cape Town \\$^{88}$~Department of Physics, University of Toronto \\$^{89}$~University of Michigan, Department of Physics \\$^{90}$~State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing, China \\$^{91}$~DESY, Hamburg and Zeuthen \\$^{92}$~Lawrence Berkeley National Laboratory \\$^{93}$~Durham University, Institute for Particle Physics Phenomenology, Ogden Centre for Fundamental Physics, South Road, Durham DH1 3LE, United Kingdom \\$^{94}$~College of Nuclear Science and Technology,Beijing Normal University,100875 Beijing, China, Beijing Radiation Center, Beijing 100875, China \\$^{95}$~University of Sheffield \\$^{96}$~Institute for High Energy Physics of National Research Centre 'Kurchatov Institute', Protvino, Russia \\$^{97}$~Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland \\$^{98}$~Research Institute for Nuclear Problems of Byelorussian State University \\$^{99}$~Institute of Particle and Nuclear Studies, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan \\$^{100}$~Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom \\$^{101}$~ Sapienza Universita' di Roma, Dipartimento di Fisica \\$^{102}$~Waseda University, Waseda Research Institute for Science and engineering (WISE) \\$^{103}$~Physics Department, University of Minho, 4710 - 057, Braga \\$^{104}$~ University of California, Berkeley \\$^{105}$~Universidad de Oviedo, Oviedo, Spain \\$^{106}$~CFTP, Instituto Superior T{\'e}cnico, Universidade de Lisboa, Avenida Rovisco Pais 1, 1049 Lisboa, Portugal \\$^{107}$~LAPTh, 9 Chemin de Bellevue, F-74941 Annecy Cedex, France \\$^{108}$~Physics Department, Florida State University \\$^{109}$~Department of Astronomy and Theoretical Physics, Lund University, Sweden \\$^{110}$~Kirchhoff-Institut f{\"u}r Physik \\$^{111}$~University of Sydney \\$^{112}$~International Center for Elementary Particle Physics and Department of Physics, The University of Tokyo \\$^{113}$~Physics Department, Universidad Autonoma de Madrid \\$^{114}$~University of Science and Technology of China \\$^{115}$~Institute of High Energy Physics, Chinese Academy of Sciences \\$^{116}$~University of California (UC), Department of Physics, 9500 Gilman Dr. La Jolla, CA 92093-0319, USA
}

==> authors_wg1.tex <==
\author{{\bf Editors and Conveners:} \\
Patrizia Azzi$^a$, Stephen Farry$^b$, Paolo Nason$^c$, Alessandro Tricoli$^d$, Dieter Zeppenfeld$^e$ 
\\
{\bf Contributors:}
Lucia Di Ciaccio$^{1}$, Corinne Goy$^{1}$, Maarten Boonekamp$^{2}$, Jan Kretzschmar$^{3}$, Nansi Andari$^{2}$, Josh Mcfayden$^{4}$, Fabrice Balli$^{2}$, Tairan Xu$^{2}$, Mykola Khandoga$^{2}$, Marija Vranjes Milosavljevic$^{5}$, Nenad Vranjes$^{5}$, Evelin Bakos$^{5}$, Yusheng Wu$^{6}$, Bing Li$^{7}$, Heling Zhu$^{6}$, Aaron James Armbruster$^{4}$, Ludovica Aperio Bella$^{4}$, Stefano Camarda$^{4}$, Juan Terron$^{8}$, Pavel Starovoitov$^{9}$, Jonathan David Bossio Sola$^{10}$, Bakar Chargeishvili$^{11}$, Sergey Mikhalcov$^{12}$, Frederic Derue$^{13}$, Jad Zahreddine$^{13}$, Marc-Andr\'e Pleier$^{14}$, Claire Alexandra Lee$^{14}$, Joe Kroll$^{15}$, Sahal Yacoob$^{16}$, William Kennedy Di Clemente$^{15}$, Karolos Potamianos$^{17}$, Fathima Noushin Zubair$^{4}$, Matthew Leigh$^{16}$, Yichen Li$^{17}$, Ant\'onio Onofre$^{18}$, Miguel Fiolhais$^{18}$, Frederic Deliot$^{2}$, Ricardo Bruno Ferreira De Faria$^{18}$, Pedro Miguel Mendes Amaral Torres Lagarelhos$^{18}$, Filipe Veloso$^{18}$, Bruno Galhardo$^{18}$, Archil Durglishvili$^{11}$, Kevin Daniel Finelli$^{19}$, Carl Suster$^{20}$, Simone Pagan Griso$^{21}$, Sarah Demers$^{22}$, Brian Petersen$^{4}$, Aleandro Nisati$^{23}$, Nguyen Phuong Dang$^{24}$, Hector De la Torre$^{25}$, Alessandro Tricoli$^{14}$, Viviana Cavaliere$^{14}$, Tatsumi Nitta$^{26}$, Robert Les$^{27}$, Koji Terashi$^{28}$, Mario Campanelli$^{29}$, Kristin Lohwasser$^{30}$, Valerie Susanne Lang$^{17}$, Deepak Kar$^{31}$, Clement Helsens$^{4}$, Mar\'ia Moreno Ll\'acer$^{4}$, Alessandro Cerri$^{32}$, 
%%%CMS}
\institute{
$^a$ INFN, Padova, Italy, $^b$ University of Liverpool, U.K.$^c$ INFN, sez. di Milano Bicocca, Università di Milano-Bicocca, Italy, $^d$ Brookhaven National Laboratory, U.S.A., 
$^e$ Institut für Theoretische Physik, Karlsruher Institut für Technologie, Germany,
$^{1}$ LAPP, Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS/IN2P3, Annecy,
$^{10}$ Universidad de Buenos Aires,
$^{11}$ High Energy Physics Institute of Tbilisi State University,
$^{12}$ Research Institute for Nuclear Problems of Byelorussian State University,
$^{13}$ Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Sorbonne Universit\'e, Paris-Diderot Sorbonne Paris Cit\'e, CNRS/IN2P3,
$^{14}$ Brookhaven National Laboratory (BNL),
$^{15}$ Department of Physics and Astronomy, University of Pennsylvania,
$^{16}$ University of Cape Town,
$^{17}$ DESY, Hamburg and Zeuthen,
$^{18}$ Laborat\'orio de Instrumenta\c{c}\~ao e F\'isica Experimental de Part\'iculas - LIP, Lisboa,
$^{19}$ Boston University, Department of Physics,
$^{2}$ IRFU, CEA, Université Paris-Saclay,
$^{20}$ University of Sydney,
$^{21}$ Lawrence Berkeley National Laboratory and University of California, Berkeley,
$^{22}$ Yale University,
$^{23}$ INFN Roma and Sapienza Universita' di Roma, Dipartimento di Fisica,
$^{24}$ University of Louisville ,
$^{25}$ Michigan State University, Department of Physics and Astronomy,
$^{26}$ Waseda University, Waseda Research Institute for Science and engineering (WISE),
$^{27}$ Department of Physics, University of Toronto,
$^{28}$ International Center for Elementary Particle Physics and Department of Physics, The University of Tokyo,
$^{29}$ Department of Physics and Astronomy, University College London,
$^{3}$ University of Liverpool,
$^{30}$ University of Sheffield,
$^{31}$ School of Physics, University of the Witwatersrand,
$^{32}$ University of Sussex,
$^{4}$ European Laboratory for Particle Physics, CERN,
$^{5}$ Institute of Physics, University of Belgrade,
$^{6}$ University of Science and Technology of China ,
$^{7}$ University of Michigan, Department of Physics,
$^{8}$ Physics Department, Universidad Autonoma de Madrid,
$^{9}$ Kirchhoff-Institut f\"{u}r Physik,
}


==> electroweak/ew_precision/ew_precision_old.tex <==
\subsection{Precision electroweak measurements}


%Number of Pages: 10 \\
%Contributors
%\begin{enumerate}
%\item Name1, Surname1
%\item Name2, Surname2
%\end{enumerate}



\subsubsection{Diboson production}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%{\bf **AT** Contribution by Sally Dawson, Michael Lewis, Julian Baglio}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\documentclass[aps,prd,nofootinbib]{revtex4}
%twocolumn
%AT \documentclass[12pt,nofootinbib,preprint,superscriptaddress]{revtex4}
%\pdfoutput=1


%
% LOCAL DEFINITIONS ------------------------------------------------------------
%
\def\nn{\nonumber}
\def\sfrac#1#2{{\textstyle{#1\over #2}}}
\def\lsim{\mbox{\raisebox{-.6ex}{~$\stackrel{<}{\sim}$~}}}
\def\gsim{\mbox{\raisebox{-.6ex}{~$\stackrel{>}{\sim}$~}}}
\newcommand{\La}{\mathcal{L}}

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{document}

%\begin{centering}
%{\bf Projections for measurements of anomalous 3-gauge boson couplings at a HE/LHC and HL/LHC}
%\\
%Julien Baglio, Sally Dawson, and Ian M. Lewis\\


\newcommand{\zz}{\ensuremath{ZZ}}                                                                                                                                                 
\newcommand{\ww}{\ensuremath{W^+W^-}}
\newcommand{\wz}{\ensuremath{W^\pm Z}}
\newcommand\as{\alpha_{\mathrm{S}}} 
\def\citere#1{\mbox{Ref.~\cite{#1}}}
\def\citeres#1{\mbox{Refs.~\cite{#1}}}
\newcommand\powheg{{\sc Powheg}}
\newcommand\Matrix{{\sc Matrix}}
\newcommand\Munich{{\sc Munich}}
\newcommand\OpenLoops{{\sc OpenLoops}}
\newcommand\Collier{{\sc Collier}}
\newcommand\GINAC{{\sc Ginac}}
\newcommand{\CutTools}{{\sc CutTools}}
\newcommand{\OneLOop}{{\sc OneLOop}}
\newcommand{\qt}{\ensuremath{q_T}}
%\newcommand{\pt}{\ensuremath{p_T}}

\newcommand{\nameobservable}[1]{{#1}}
\newcommand{\captiontext}{}
\newcommand{\GeV}{\,\mathrm{GeV}}


%\subsubsection*{Gauge-boson pair production with M{\small ATRIX}}

We present NNLO QCD predictions for \ww{}, \wz{} and \zz{} production in proton--proton collisions.
We consider two LHC upgrade scenarios,
namely a high-luminosity~(HL) LHC running at $\sqrt{s}=14\,{\rm TeV}$ with an
assumed integrated luminosity of $3\,{\rm ab}^{-1}$, and a high-energy~(HE) LHC at  $\sqrt{s}=27\,{\rm TeV}$ with $15\,{\rm ab}^{-1}$\,.
More precisely, we investigate the inclusive hard-scattering processes
\begin{align*}
  & pp\to \ell^+\nu_\ell \,\ell^{\prime -}  {\bar \nu}_{\ell^\prime}+X\,,\\
  & pp \to \ell\nu_\ell \,\ell^{\prime +} \ell^{\prime -}+X\,,\\
  & pp \to \ell^+ \ell^- \ell^{\prime +} \ell^{\prime -}+X\, ,
\end{align*}
where all off-shell effects and interference contributions are fully accounted for. 

All results are obtained with the public parton-level NNLO framework {\sc Matrix}. This program, and earlier versions of it,
have been used to compute state-of-the-art QCD predictions for gauge-boson pair production processes \cite{Grazzini:2013bna,Grazzini:2015nwa,Cascioli:2014yka,Grazzini:2015hta,Gehrmann:2014fva,Grazzini:2016ctr,Grazzini:2016swo,Grazzini:2017ckn,Kallweit:2018nyv}.\footnote{It was
  also used in the NNLL+NNLO computation for \ww{} and \zz{} production of \citere{Grazzini:2015wpa}, and in the NNLOPS computation for \ww{} production of \citere{Re:2018vac}.}
All tree-level and one-loop amplitudes are evaluated with 
\OpenLoops{}\footnote{\OpenLoops{} relies on the fast and stable
tensor reduction of \Collier{}~\cite{Denner:2014gla,Denner:2016kdg},
supported by a rescue system based on quad-precision
\CutTools\cite{Ossola:2007ax} with \OneLOop\cite{vanHameren:2010cp}
to deal with exceptional phase-space
points.}~\cite{Cascioli:2011va,Buccioni:2017yxi}.
At two-loop level we use the $q\bar{q}\to VV'$ amplitudes of \citere{Gehrmann:2015ora}.

We apply the complex mass scheme~\cite{Denner:2005fg} throughout, 
i.e.\ we use complex $W$- and $Z$-boson masses and define the EW mixing angle as $\cos\theta_W^2=(m_W^2-i\Gamma_W\,m_W)/(m_Z^2-i\Gamma_Z\,m_Z)$.
For the input of the weak parameters we employ the $G_\mu$ scheme with $\alpha=\sqrt{2}\,G_\mu |(m_W^2-i\Gamma_W\,m_W)\sin^2\theta_W|/\pi$\,.
We set $G_F = 1.16639\times 10^{-5}$\,GeV$^{-2}$, $m_W=80.399$\,GeV, $\Gamma_W=2.1054$\,GeV, $m_Z = 91.1876$\,GeV, $\Gamma_Z=2.4952$\,GeV, $m_H = 125$\,GeV and $\Gamma_H = 0.00407$\,GeV. Furthermore, we use a diagonal CKM matrix.

The number of light quarks is chosen differently for the processes under consideration:
All \ww{} results are obtained by applying the four-flavour scheme (4FS) with massive top and bottom quarks in order to consistently
remove top-quark contamination by omitting the (separately IR finite) partonic processes with real bottom-quark emissions.
In the 4FS, we use the on-shell bottom mass $m_b = 4.92$\,GeV.
For all other processes we apply the five-flavour scheme (5FS) with a vanishing bottom mass $m_b = 0$.
The top quark is treated as massive and unstable throughout,
and we set $m_t = 173.2$\,GeV as well as $\Gamma_t = 1.44262$\,GeV.\footnote{Massive
top-quark contributions are neglected in the virtual two-loop corrections, but are kept everywhere else in the computations.}

We use the MMHT2014~\cite{Harland-Lang:2014zoa} sets of parton distribution functions~(PDFs) with $n_f=4$ or $n_f=5$ active quark flavours,
consistently with the flavour scheme under consideration.                             
N$^n$LO ($n=0,1,2$) predictions are obtained by using PDFs at the same perturbative order and
the evolution of $\as$ at $(n+1)$-loop order, as provided by the corresponding PDF set.
To be precise, in the 5FS we use {\tt MMHT2014lo68cl}, {\tt MMHT2014nlo68cl}, and
  {\tt MMHTnnlo68cl} at LO, NLO, and NNLO.
  In the 4FS we use {\tt MSTW2008lo68cl\_nf4}, {\tt MMHT2014nlo68cl\_nf4}, and
 {\tt MMHT2014nnlo68cl\_nf4} at LO, NLO, and NNLO.

Our central predictions are obtained by setting the factorization and renormalization 
scales to $\mu_F=\mu_R=\mu_0\equiv E_{\mathrm{T,}V_1}+E_{\mathrm{T,}V_2}$,
with $E_{\mathrm{T,}V_i}= \sqrt{M^2_{V_i}+p^2_{\mathrm{T,}V_i}}$, where $M_{V_i}$ is the invariant mass 
and $p_{{\rm T,}V_i}$ the transverse momentum of the respective vector boson.
Uncertainties from missing higher-order
contributions are estimated in the usual way by independently varying $\mu_F$ and $\mu_R$ in the range $0.5\mu_0<\mu_F,\mu_R<2\mu_0$ with the constraint $0.5<\mu_F/\mu_R<2$.


\begin{table}[t]
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c c | c c c c c}
\toprule
\multicolumn{2}{c|}{$\sigma$ [fb]}

& LO
& NLO
& NLO$^\prime$$+gg$
& NNLO
& \multirow{2}{*}{\Large $\frac{\sigma_{\rm NNLO}({\rm 27\,TeV})}{\sigma_{\rm NNLO}({\rm 14\,TeV})}$}
\\
\multicolumn{2}{c|}{\footnotesize (correction)}
& 
& {\footnotesize (NLO/LO$-$1)}
& {\footnotesize (NLO$^\prime$$+gg$/NLO$-$1)}
& {\footnotesize (NNLO/NLO$-$1)}
\\
\midrule
\multirow{ 4}{*}{\vspace{-0.25cm}\ww{}}
& 
\multirow{ 2}{*}{$\sqrt{s}=14$\,TeV}
& $897.27(9)^{     +4.3 \%}_{     -5.3 \%}$
& $1303.3(1)^{     +2.7 \%}_{     -2.2 \%}$ 
& $1386.1(2)^{     +3.7 \%}_{     -2.9 \%}$ 
& $1485.(1)^{     +2.4 \%}_{     -2.2 \%}$ 
& \multirow{ 4}{*}{\vspace{-0.25cm} 2.33}
\\
&
&
& {\footnotesize ($+45.3\%$)} 
& {\footnotesize ($+6.4 \%$)}
& {\footnotesize ($+13.9 \%$)}
\\[0.25cm]
& \multirow{ 2}{*}{$\sqrt{s}=27$\,TeV}
& $2091.5(2)^{     +7.6 \%}_{     -8.6 \%}$
& $2988.4(3)^{     +2.8 \%}_{     -2.9 \%}$
& $3213.0(4)^{     +4.1 \%}_{     -3.2 \%}$
& $3457.(4)^{     +2.8 \%}_{     -2.4 \%}$ 
\\
&
&
& {\footnotesize ($+42.9\%$)}
& {\footnotesize ($+7.0\%$)}
& {\footnotesize ($+15.6\%$)}
\\
\midrule
\multirow{ 4}{*}{\vspace{-0.25cm}$W^+Z${}}
& \multirow{ 2}{*}{$\sqrt{s}=14$\,TeV}
& $60.322(6)^{     +3.4 \%}_{     -4.3 \%}$
& $106.15(1)^{     +3.6 \%}_{     -3.0 \%}$ 
& \multirow{ 2}{*}{---}
& $120.5(1)^{     +2.0 \%}_{     -1.9 \%}$ 
& \multirow{ 4}{*}{\vspace{-0.25cm} 2.35}
\\
&
&
& {\footnotesize ($+76.0\%$)} 
& 
& {\footnotesize ($+13.5\%$)}
\\[0.25cm]
& \multirow{ 2}{*}{$\sqrt{s}=27$\,TeV}
& $136.66(1)^{     +6.8 \%}_{     -7.8 \%}$
& $248.51(2)^{     +4.0 \%}_{     -3.3 \%}$
& \multirow{ 2}{*}{---}
& $283.4(3)^{     +2.1 \%}_{     -2.1 \%}$
\\
&
&
& {\footnotesize ($+81.8\%$)}
&
& {\footnotesize ($+14.0\%$)}

\\
\midrule
\multirow{ 4}{*}{\vspace{-0.25cm}$W^-Z${}}
& \multirow{ 2}{*}{$\sqrt{s}=14$\,TeV}
& $39.182(4)^{     +3.7 \%}_{     -4.7 \%}$
& $68.430(7)^{     +3.7 \%}_{     -3.0 \%}$ 
& \multirow{ 2}{*}{---}
& $77.63(7)^{     +1.9 \%}_{     -1.9 \%}$
& \multirow{ 4}{*}{\vspace{-0.25cm} 2.57}
\\
&
&
& {\footnotesize ($+74.6\%$)}
& 
& {\footnotesize ($+13.4\%$)}
\\[0.25cm]
& \multirow{ 2}{*}{$\sqrt{s}=27$\,TeV}
& $96.70(1)^{     +7.2 \%}_{     -8.2 \%}$
& $175.44(2)^{     +4.0 \%}_{     -3.3 \%}$
& \multirow{ 2}{*}{---}
& $199.7(2)^{     +2.0 \%}_{     -2.0 \%}$
\\
&
&
& {\footnotesize ($+81.4\%$)}
& 
& {\footnotesize ($+13.8\%$)}
\\
\midrule
\multirow{ 4}{*}{\vspace{-0.25cm}\zz{}}
& \multirow{ 2}{*}{$\sqrt{s}=14$\,TeV}
& $24.500(2)^{     +4.3 \%}_{     -5.3 \%}$
& $34.201(3)^{     +2.0 \%}_{     -1.8 \%}$ 
& $37.531(4)^{     +3.3 \%}_{     -2.6 \%}$
& $39.64(4)^{     +2.4 \%}_{     -2.1 \%}$ 
& \multirow{ 4}{*}{\vspace{-0.25cm} 2.40}
\\
&
&
& {\footnotesize ($+39.6\%$)}
& {\footnotesize ($+9.7\%$)}
& {\footnotesize ($+15.9 \%$)}
\\[0.25cm]
& \multirow{ 2}{*}{$\sqrt{s}=27$\,TeV}
& $58.622(6)^{     +7.9 \%}_{     -8.9 \%}$
& $79.757(8)^{     +2.2 \%}_{     -3.0 \%}$ 
& $89.89(1)^{     +3.7 \%}_{     -3.0 \%}$ 
& $95.20(9)^{     +2.9 \%}_{     -2.4 \%}$
\\
&
& 
& {\footnotesize ($+36.1\%$)}
& {\footnotesize ($+12.7\%$)}
& {\footnotesize ($+19.4\%$)}
&
\\
\bottomrule

\end{tabular}}
\end{center}
\renewcommand{\baselinestretch}{1.0}
\caption{\label{tab:dibosonXS} Inclusive cross sections for \ww{}, \wz{} and \zz{} production.}
\end{table}


\begin{table}[t]
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c c | c c c c c}
\toprule
\multicolumn{2}{c|}{$\sigma$ [fb]}

& LO
& NLO
& NLO$^\prime$$+gg$
& NNLO
& \multirow{2}{*}{\Large $\frac{\sigma_{\rm NNLO}({\rm 27\,TeV})}{\sigma_{\rm NNLO}({\rm 14\,TeV})}$}
\\
\multicolumn{2}{c|}{\footnotesize (correction)}
& 
& {\footnotesize (NLO/LO$-$1)}
& {\footnotesize (NLO$^\prime$$+gg$/NLO$-$1)}
& {\footnotesize (NNLO/NLO$-$1)}
\\
\midrule
\multirow{ 4}{*}{\vspace{-0.25cm}\ww{}}
& 
\multirow{ 2}{*}{$\sqrt{s}=14$\,TeV}
& $     0.920(1)^{     +2.7 \%}_{     -2.7 \%}$
& $     2.827(5)^{     +9.7 \%}_{     -8.0 \%}$
& $     2.793(7)^{     +9.9 \%}_{     -8.1 \%}$
& $      3.51(1)^{     +5.2 \%}_{     -5.0 \%}$
& \multirow{ 4}{*}{\vspace{-0.25cm} 3.93}
\\
&
&
& {\footnotesize ($+207.1 \%$)} 
& {\footnotesize ($  -1.2 \%$)}
& {\footnotesize ($ +24.3 \%$)}
\\[0.25cm]
& \multirow{ 2}{*}{$\sqrt{s}=27$\,TeV}
& $     2.847(3)^{    +0.08 \%}_{     -0.5 \%}$
& $     10.83(2)^{     +8.2 \%}_{     -6.9 \%}$
& $     10.66(2)^{     +8.4 \%}_{     -7.1 \%}$
& $     13.80(4)^{     +5.3 \%}_{     -4.8 \%}$
\\
&
&
& {\footnotesize ($+280.5 \%$)}
& {\footnotesize ($  -1.6 \%$)}
& {\footnotesize ($ +27.3 \%$)}
\\
\midrule
\multirow{ 4}{*}{\vspace{-0.25cm}$W^+Z${}}
& \multirow{ 2}{*}{$\sqrt{s}=14$\,TeV}
& $   0.06524(8)^{     +3.3 \%}_{     -3.2 \%}$
& $    0.1273(3)^{     +7.1 \%}_{     -5.8 \%}$
& \multirow{ 2}{*}{---}
& $    0.1485(9)^{     +3.4 \%}_{     -3.3 \%}$ 
& \multirow{ 4}{*}{\vspace{-0.25cm} 3.82}
\\
&
&
& {\footnotesize ($ +95.2 \%$)} 
& 
& {\footnotesize ($ +16.6 \%$)}
\\[0.25cm]
& \multirow{ 2}{*}{$\sqrt{s}=27$\,TeV}
& $    0.1919(2)^{     +0.1 \%}_{     -0.5 \%}$
& $    0.4642(8)^{     +7.0 \%}_{     -5.8 \%}$
& \multirow{ 2}{*}{---}
& $     0.568(3)^{     +3.8 \%}_{     -3.6 \%}$
\\
&
&
& {\footnotesize ($+141.9 \%$)}
&
& {\footnotesize ($ +22.5 \%$)}

\\
\midrule
\multirow{ 4}{*}{\vspace{-0.25cm}$W^-Z${}}
& \multirow{ 2}{*}{$\sqrt{s}=14$\,TeV}
& $   0.03289(4)^{     +3.1 \%}_{     -3.1 \%}$
& $    0.0641(2)^{     +7.5 \%}_{     -6.0 \%}$
& \multirow{ 2}{*}{---}
& $    0.0767(5)^{     +3.4 \%}_{     -3.5 \%}$
& \multirow{ 4}{*}{\vspace{-0.25cm} 4.34}
\\
& 
& 
& {\footnotesize ($ +94.9 \%$)}
& 
& {\footnotesize ($ +19.7 \%$)}
\\[0.25cm]
& \multirow{ 2}{*}{$\sqrt{s}=27$\,TeV}
& $    0.1121(1)^{      +0. \%}_{     -0.3 \%}$
& $    0.2719(5)^{     +7.2 \%}_{     -5.9 \%}$
& \multirow{ 2}{*}{---}
& $     0.333(2)^{     +3.7 \%}_{     -3.5 \%}$
\\
&
&
& {\footnotesize ($+142.7 \%$)}
& 
& {\footnotesize ($ +22.5 \%$)}
\\
\midrule
\multirow{ 4}{*}{\vspace{-0.25cm}\zz{}}
& \multirow{ 2}{*}{$\sqrt{s}=14$\,TeV}
& $   0.02108(3)^{     +3.1 \%}_{     -3.1 \%}$
& $    0.0318(1)^{     +3.8 \%}_{     -3.2 \%}$
& $    0.0342(1)^{     +5.4 \%}_{     -4.3 \%}$
& $    0.0371(3)^{     +3.6 \%}_{     -3.0 \%}$
& \multirow{ 4}{*}{\vspace{-0.25cm} 3.70}
\\
&
&
& {\footnotesize ($ +50.6 \%$)}
& {\footnotesize ($  +7.7 \%$)}
& {\footnotesize ($ +16.9 \%$)}
\\[0.25cm]
& \multirow{ 2}{*}{$\sqrt{s}=27$\,TeV}
& $    0.0675(1)^{      +0. \%}_{     -0.2 \%}$
& $    0.1100(3)^{     +3.5 \%}_{     -2.8 \%}$
& $    0.1235(3)^{     +5.4 \%}_{     -4.3 \%}$
& $    0.1371(7)^{     +4.3 \%}_{     -3.5 \%}$
\\
&
& 
& {\footnotesize ($ +62.9 \%$)}
& {\footnotesize ($ +12.3 \%$)}
& {\footnotesize ($ +24.7 \%$)}
&
\\
\bottomrule

\end{tabular}}
\end{center}
\renewcommand{\baselinestretch}{1.0}
\caption{\label{tab:dibosonXSpT100GeV} Cross sections with a $p_{\mathrm{T, min}}=100\,{\rm GeV}$ cut on the transverse momentum
of the charged leptons and the missing energy for \ww{}, \wz{} and \zz{} production.}
\end{table}


In Table~\ref{tab:dibosonXS} we present cross sections for \ww{}, \wz{} and \zz{} production,
inclusive over the phase space of the final-state leptons, for $pp$ collisions at $\sqrt{s}=14$\,TeV and $\sqrt{s}=27$\,TeV.
Throughout, we apply only a basic selection cut on $Z$ bosons, by requiring the invariant masses
of all opposite-sign same-flavour lepton pairs to be within a $Z$-mass window of $66\GeV<m_{\mathrm{\ell^-\ell^+}}<116\GeV$, 
which is necessary to avoid divergencies induced by soft intermediate photons. The gain in the inclusive cross section at $\sqrt{s}=27$\,TeV is 
roughly a factor of $2.5$ for all processes under consideration, see last
column of Table~\ref{tab:dibosonXS}. 
We further see the importance of QCD corrections:
Higher-order contributions are huge, especially for \wz{} production.
The NLO corrections
range from about $+36\%$ to $+82\%$ depending on process and collider energy, while 
NNLO QCD corrections are still sizeable and induce a further increase of the cross sections of $13\%$ to $20\%$.
The cross-section ratio for $W^+Z$/$W^-Z$ production is about $1.55$ at NNLO for $\sqrt{s}=14$\,TeV, changes to
$1.42$ for $\sqrt{s}=27$\,TeV, and is essentially independent on the perturbative order.

We stress that QCD radiative corrections may change quite significantly 
as soon as fiducial cuts on the leptonic final state are applied, or when 
kinematical distributions are considered. The corrections for the 
inclusive cross sections in Table~\ref{tab:dibosonXS} should therefore be understood as illustrative, and the use of inclusive $K$-factors
to obtain NNLO predictions from lower order results with different sets of cuts should be avoided in general.

It is interesting to quantify the size of the loop-induced gluon fusion contribution of the charge-neutral processes, 
which is part of the NNLO QCD corrections.
By NLO$^\prime$+$gg$ we denote its sum with the NLO cross section computed with NNLO PDFs.
The NLO$^\prime$+$gg$ result for \ww{} production is $6.4\%$ ($7.0\%$) larger than the NLO result at $\sqrt{s}=14\,(27)$\,TeV, while 
their difference is even $9.7\%$ ($12.7\%$)  for \zz{} production.
These numbers amount to roughly half of the full NNLO correction of the \ww{}
process, and even about two-thirds for \zz{} production.
However, one has to bear in mind that under typical fiducial selection requirements on 
the leptons and missing transverse energy, the impact of the loop-induced 
contribution decreases significantly, especially for \ww{} production.
Furthermore, its relative contribution is strongly suppressed as far as 
the tails of the kinematical distributions are concerned, due to the large-$x$ suppression
of the gluon density.

To illustrate how strongly the radiative corrections may depend on the fiducial cuts, in Table~\ref{tab:dibosonXSpT100GeV} we show cross sections
with a minimum $p_{\mathrm{T, min}}=100$\,GeV cut on the transverse momentum
of the charged leptons and the missing energy. More precisely, depending on the process we have applied the following cuts:
\begin{center}
\renewcommand\arraystretch{1.5}
\begin{tabular}{l|c|c|c}
  \toprule
& \ww{} & \wz{} & \zz{} \\
  \midrule
{lepton cuts} &
  $p_{\mathrm{T,\ell_{1/2}}}>p_{\mathrm{T, min}}$ &
  $p_{\mathrm{T,\ell_{1/2/3}}}>p_{\mathrm{T, min}}$ &
  $p_{\mathrm{T,\ell_{1/2/3/4}}}>p_{\mathrm{T, min}}$ \\
{neutrino cuts} &
  $p_{\mathrm{T,miss}}>p_{\mathrm{T, min}}$ &
  $p_{\mathrm{T,miss}}>p_{\mathrm{T, min}}$ &
  ---
  \\
  \bottomrule
\end{tabular}
\end{center}
As we can read from the table, radiative corrections at NLO can be enormous for some processes with $p_{\mathrm{T, min}}=100$\,GeV,
ranging from $+51\%$ to even $+281\%$. Also the NNLO corrections are significantly increased with respect to the inclusive case,
and can be as large as $+27\%$. It is also apparent that the importance of the loop-induced gluon fusion contribution
is significantly reduced. For \ww{} production, due to the applied $p_{\mathrm{T,miss}}$ cut the NLO$^\prime$+$gg$ contribution is even smaller than the NLO cross section
by $-1.2\%$ ($-1.6\%$) at $\sqrt{s}=14\,(27)$\,TeV (i.e.\ the possitive impact of the $gg$ channel is smaller than the negative effect
from using NNLO PDFs instead of NLO PDFs in the NLO$^\prime$+$gg$ prediction). For \zz{} production, it is still sizable with $7.7\%$ ($12.3\%$), but its 
relative contribution at $\mathcal{O}(\as^2)$ has decreased from roughly two-thirds in the inclusive case to less than half
of the NNLO corrections for $p_{\mathrm{T, min}}=100$\,GeV. Furthermore, compared to the inclusive results
we observe an even more substantial increase of the cross sections from $\sqrt{s}=14$\,TeV to $\sqrt{s}=27$\,TeV of roughly a factor of four.
This can be understood by the fact, that the additional energy enlarges the available phase-space, especially at high momentum transfer.

From the results in Table~\ref{tab:dibosonXS} and \ref{tab:dibosonXSpT100GeV} 
it is clear that the perturbative uncertainties at NLO cannot account for the additional loop-induced 
gluon fusion contribution that appears at NNLO. Besides that, also the genuine NNLO corrections to the quark--antiquark production mechanism
cannot be anticipated from NLO scale variations, which in turn means that the NLO uncertainties are underestimated.
The inclusion of NNLO corrections is therefore crucial. At this order all partonic channels 
are included for the first time, and scale variations can be used to obtain an estimate of the actual size of missing 
higher-order terms. However, the NLO corrections to the loop-induced gluon fusion contribution are relevant and should be included when possible,
especially at $\sqrt{s}=27$\,TeV where gluons with smaller $x$ are probed.
In particular in tails of high-energy observables, the inclusion of
NLO EW corrections and their interplay with QCD corrections will also need to be investigated.
Nevertheless we restrict ourselves to presenting NNLO QCD results in the following, but the above-mentioned extensions
will become available well before the start of the HL-LHC.

We now turn to discussing differential results in diboson processes in the light of the HL and HE upgrades of 
the LHC. Since the importance of highest-order predictions is evident from the previous discussion, we concentrate
on NNLO QCD accurate results here. We first consider the cumulative cross section with a minimum $p_{\mathrm{T, min}}$ cut, as introduced above.
In order to analyze the number of expected events as a function of $p_{\mathrm{T, min}}$, we have translated the 
cross sections to event numbers by assuming an integrated luminosity of $3$\,ab$^{-1}$ at $14\,$TeV and of $15$\,ab$^{-1}$ at $27$\,TeV.


Figure~\ref{fig:ptmin_diboson} shows the expected number of events as a function of $p_{\mathrm{T, min}}$. 
Since we are restricting the transverse momentum of all leptonic final states simultaneously, the reach in the tails may appear smaller 
than expected, and would be significantly larger if we were to consider a cut on the transverse momentum of the leading lepton
or the missing energy only.
However, the toy scenario we are considering is well suited to compare the three diboson production processes, and to 
quantify the relative gain of the additional energy and luminosity.

The curves in Figure~\ref{fig:ptmin_diboson} show all production processes under consideration:
%
\begin{figure}
\begin{center}
\includegraphics[trim = 10mm 0mm 0mm 0mm, width=.5\textheight]{\main/electroweak/img/ew_precision/combined_Nevents_27-14_pTmincut.pdf}
\caption[]{{
\label{fig:ptmin_diboson}
Cumulative number of events as a function of $ p_{\mathrm{T, min}}$.}}
\end{center}
\end{figure}
%
\ww{} (blue), \wz{} (green), and \zz{} (orange); at $14$\,TeV (dashed) and $27$\,TeV (solid). The horizontal red line shows the one-event threshold, below which no events are expected anymore.
We read the following features from the plot: At $\sqrt{s}=14$\,TeV we expect events up to $p_{\mathrm{T, min}}$ values of roughly
$550$\,GeV, $370$\,GeV, and $270$\,GeV for \ww{}, \wz{}, and \zz{} production, respectively.
At $\sqrt{s}=27$\,TeV these values read $>${}$1000$\,GeV, $740$\,GeV, and $550$\,GeV.
To put these numbers into perspective, we have added a dash-dotted red line for the present status at the end of Run II, which 
represents the one-event threshold for $150\,{\rm fb^{-1}}$ at $13\,{\rm TeV}$ 
($14\,{\rm TeV}\to13\,{\rm TeV}$ conversion approximated by a constant cross-section correction factor of $0.9$). 
Its intersection points with the $\sqrt{s}=14$\,TeV curves
  indicates the current reach of the LHC, which is roughly up to
  $350$\,GeV, $210$\,GeV, and $140$\,GeV for \ww{}, \wz{}, and \zz{} production, respectively.
The improved reach in the tails at $27$\,TeV is not only related to the larger inclusive cross section and higher luminosity, but also the enlarged phase-space available with higher energies plays an important role: Whereas the solid curves fall only by $7-8$ orders of magnitude in the range of $0\,{\rm GeV} \le p_{\mathrm{T, min}}\le 1000$\,GeV,
the dashed $14$\,TeV curves fall by more than $9$ orders of magnitude in the same region. This also explains why the $14$\,TeV \ww{} result, which has a much larger 
inclusive cross section, crosses the red one-event line at almost the same point as the $27$\,TeV \zz{} result.

In Figure~\ref{fig:mcut_diboson} we study the reach of the three vector-boson 
pair production processes for future LHC upgrades 
in the invariant-mass distributions of all produced charged leptons.
%
\begin{figure}
\begin{center}
\includegraphics[trim = 10mm 0mm 0mm 0mm, width=.5\textheight]{\main/electroweak/img/ew_precision/combined_Nevents_27-14_mcut_leptonic_pTmin20.pdf}
\caption[]{{
\label{fig:mcut_diboson}
Cumulative number of events as a function of $m_{n\ell,{\rm min}}$.}}
\end{center}
\end{figure}
%
We choose a scenario where $p_{\mathrm{T, min}}$, defined as before in the 
three processes, is $20$\,GeV in order to have at least a rough definition of the fiducial phase-space.
We show the expected number of events, assuming the same integrated luminosities
as stated above, for $\sqrt{s}=14$\,TeV (dashed) and $\sqrt{s}=27$\,TeV (solid) 
with a lower cut $m_{n\ell}>m_{n\ell,{\rm min}}$, where $n$ is the number of leptons
in the respective process, i.e., for \ww{} production it is the 
distribution in $m_{2\ell}$ (blue), for \wz{} it is the one in $m_{3\ell}$ (green),
and for \zz{} in $m_{4\ell}$ (orange). The significant reach in energy for both 
the HL run of the LHC and a potential HE upgrade is evident.
With ``reach" we refer to the point where the curves cross the red horizontal 
one-event threshold.
A resonance in the tails of the invariant masses of 
two leptons (plus missing transverse momentum) or of four leptons is
indeed a realistic signature predicted by many BSM theories. While with the current
Run II data (red, dash-dotted line crossing the $14$\,TeV results) searches can hardly pass the two TeV frontier, future LHC upgrades 
will allow us to probe mass scales of a few TeV at $14$\,TeV with $3$\,ab$^{-1}$, 
or potentially even up to ten TeV at $27$\,TeV with $15$\,ab$^{-1}$.
We also notice that despite $\sigma_{\ww{}}\gg \sigma_{\wz{}}\gg \sigma_{\zz{}}$ holds inclusively, the point where the three lines fall below one event is much 
closer. This is simply caused by the fact that the phase space of the 
four-lepton system in \zz{} production 
is larger than the one of the three-lepton system in \wz{} production, where
some energy is taken by the additional neutrino. An analogous interpretation applies
to \ww{} production. Furthermore, also here the significantly 
enlarged phase space induced by the increase in energy at $27$\,TeV is evident:
The $27$\,TeV results drop by roughly $4-5$ orders of magnitude in the displayed 
range, while the $14$\,TeV ones drop by more than $6$ orders.

We continue our study by analyzing the importance of the additional 
fiducial phase space that becomes available with detector upgrades to 
enlarge the accessible rapidity range of charged leptons. Since we found very similar results for \ww{}, \wz{} and \zz{} 
production in that respect,  in Figure~\ref{fig:rapidity_diboson} we show the rapidity efficiency of the four-lepton signature for \zz{} production only.
%
\begin{figure}
\begin{center}
\includegraphics[trim = 10mm 0mm 0mm 0mm, width=.5\textheight]{\main/electroweak/img/ew_precision/ZZ_NNLO_27-14_absetamaxveto_lep.pdf}
\caption[]{{
\label{fig:rapidity_diboson}
Rapidity efficiency of the charged leptons.}}
\end{center}
\end{figure}
%
The rapidity efficiency is defined as the ratio of the cross section with an absolute-rapidity cut $\eta_{\rm cut}$ on all four charged leptons, divided by the 
inclusive cross section. As for $\eta_{\rm cut}\rightarrow \infty$ no cut is applied, the ratio tends to unity for large $\eta_{\rm cut}$ values.
The efficiency as a function of $\eta_{\rm cut}$ is studied for three $p_{\mathrm{T, min}}$ scenarios: inclusive (light blue), $p_{\mathrm{T, min}} = 20$\,GeV (blue), and $p_{\mathrm{T, min}} = 100$\,GeV (dark blue); at $14$\,TeV (dashed) and $27$\,TeV (solid). We directly observe that the efficiency 
decreases with the machine energy. In other words, a small rapidity threshold at $27$\,TeV results in a much larger (relative) reduction
of the cross section than at $14$\,TeV. This is because the additional energy induces more forward (and boosted) leptons, and it shows that 
detector upgrades that enlarge the measurable rapidity range become even more important at the HE LHC.
Requiring minimum transverse-momentum cuts, on the other hand, has the effect
of increasing the rapidity efficiency, which is particularly striking for 
$p_{\mathrm{T, min}} = 100$\,GeV. The reason for this is simple: Leptons 
with high transverse momentum are predominantly produced at central rapidities.

Let us focus on the scenario with $p_{\mathrm{T, min}} = 20$\,GeV
as it provides the most realistic fiducial setup, which is actually not much 
different from the fully inclusive case.
Typical rapidity cuts on charged leptons with the current LHC detectors are 
of the order of $\eta_\ell = 2.5$. Future detector upgrades for the HL
phase of the LHC can be expected to reach rapidities at the level of $\eta_\ell = 4$.
At $14\,(27)$\,TeV this would allow us to improve measurements of fiducial cross 
from a $<$$60\%$ ($\sim 50\%$) efficiency 
for $\eta_{\rm cut} = 2.5$ to a $>$$90\%$ ($\lesssim 90\%$) efficiency for $\eta_{\rm cut} = 4$.
This implies that the available inclusive cross section will be hardly reduced 
by fiducial rapidity requirements anymore once the detectors have been upgraded. 
This statement holds even more when considering scenarios with boosted leptons: For
$p_{\mathrm{T, min}} = 100$\,GeV the efficiency is practically $100\%$ for 
$\eta_{\rm cut} = 4$.


\subsubsection{Projections for measurements of anomalous 3-gauge boson couplings}

%{\bf Abstract}\\
%\end{centering}
%{\it{We study the sensitivity to  anomalous gauge boson and anomalous fermion couplings in
%the production of $W^+W^-$ pairs at future LHC upgrades.}}
%\\
%\vskip .2in

The $SU(2)\times U(1)$ structure of the electroweak sector of the
Standard Model  determines the $W^+W^-V$ interactions
($V=\gamma, Z $).   The amplitudes for the production of $W^+W^-$
pairs involve subtle cancellations between contributions that grow
with energy, so  the
pair production of gauge bosons  is  extremely sensitive to new
physics interactions.
Assuming CP conservation, the most general Lorentz invariant $3-$gauge
boson couplings can be written
as~\cite{Gaemers:1978hg,Hagiwara:1986vm}
\begin{eqnarray}
 \La_{V}&=&
-ig_{WWV}\biggl\{(1+\delta g_1^V)\left(W^+_{\mu\nu}W^{-\mu}V^\nu-W_{\mu\nu}^-W^{+\mu}V^\nu\right)+(1+\delta\kappa^V)W^+_\mu
            W^-_\nu V^{\mu\nu})\nonumber \\ &&+\frac{\lambda^V}{M^2_W}W^+_{\rho\mu}{W^{-\mu}}_\nu V^{\nu\rho}\biggr\},
\label{eq:lagdef}
\end{eqnarray}  
where $V=\gamma, Z$, $g_{WW\gamma}=e$, $g_{WWZ}=g \cos\theta_W$, 
 $s_W^{} \equiv \sin\theta_W^{}$ , $c_W^{} \equiv
\cos\theta_W^{}$, and in the SM, $\delta g_1^V = \delta\kappa_{}^V
= \lambda_{}^V = 0$.  Because of gauge invariance,
  This form can  be translated into the language of effective
field theory, where $\delta g_1^V,~\delta\kappa^V,~\lambda^V\sim {v^2\over\Lambda^2}$, with $\Lambda$ the scale of
BSM physics, $\Lambda >> v$.

The effective couplings of fermions to gauge fields are parameterized as,
\begin{eqnarray}
  \La&=&{g\over c_W} Z_\mu\biggl[g_L^{Zq}+\delta g_{L}^{Zq}\biggr]
  {\overline q}_L\gamma_\mu q_L\
 +g_ZZ_\mu\biggl[g_R^{Zq}+\delta g_{R}^{Zq}\biggr]
  {\overline q}_R\gamma_\mu q_R\nonumber \\
  &&+{g\over \sqrt{2}}\biggl\{W_\mu\biggl[(1+\delta g_{L}^W){\overline q}_L\gamma_\mu q_L^\prime
  +\delta g_R^W
  {\overline q}_R\gamma_\mu q_R^\prime\biggr] +h.c.\biggr\}\, ,
  \label{eq:dgdef}
  \end{eqnarray}
 where  $Q_q$ is the electric
 charge of the quarks, and $q$ denotes up-type or down-type quarks.  The anomalous fermion
 couplings also scale as $\delta g_{L,R}^{Zq}, \delta g_{L,R}^W\sim{v^2\over\Lambda^2}$.
 The SM quark couplings are
$g_R^{Zq}=-s_W^2 Q_q$ and $g_L^{Zq}=T_3^q -s_W^2 Q_q$ with
 $T_3^q=\pm \displaystyle \frac{1}{2}$.  $SU(2)$ invariance relates
the coefficients,
$
\delta g_L^W=\delta g_L^{Zf}-\delta g_L^{Zf'}, \,
\delta g_1^Z= \delta \kappa_{}^Z+{s_W^2\over c_W^2}\delta \kappa_{}^\gamma$ and
$
\lambda_{}^\gamma = \lambda_{}^Z$,
where $f$ denotes up-type quarks and $f'$  down-type quarks. 


We have implemented both the anomalous 3-gauge boson  and fermion couplings
into the POWHEG BOX framework\cite{Melia:2011tj} for $W^+W^-$ production and generated samples of events with
 $pp\rightarrow W^+W^-\rightarrow \mu^\pm e^\mp\nu\nu$.
Fits to $8~TeV$ data\cite{Baglio:2017bfe,Alves:2018nof} illustrate the importance of including  both anomalous fermion  and 3-gauge boson couplings.
The sensitivity to anomalous couplings results almost entirely 
from contributions quadratic in the anomalous couplings and  the effects of anomalous 3-gauge boson and 
fermion couplings are numerically similar.  


To probe the sensitivity to anomalous couplings,  we generate events using the cuts
\begin{equation}
p_T^{l}>30~GeV,\,\mid \eta^l\mid<2.5,\,m_{ll}>10 ~GeV, \slashed{E}_T>20~GeV\,.
\end{equation}
These cuts are similar to those applied in the ATLAS\cite{Aad:2016wpd} and CMS\cite{Khachatryan:2015sga} extractions of anomalous coupling
limits using the $8~TeV$ data. 
We postulate a hypothetical future systematic uncertainty of 
$\delta_{sys}=16\%$ and set a cut on the $p_T$ of the leading lepton such that the systematic error
is smaller than the statistical error, $\delta_{stat}={1\over \sqrt{L\sigma(p_{l,T}^{lead}>p_T^{cut})}}>\delta_{sys}$,where $L$ is the integrated luminosity.
We look at the integrated cross section above a $p_T^{cut}$, assume a $50~\%$ efficiency and set the cuts as
\begin{eqnarray}
27~TeV~{\text{with}}~15 ~ab^{-1}: &p_T^{cut}=750~GeV,\qquad 
14~TeV~{\text{with}}~3 ~ab^{-1}: p_T^{cut}=1350~GeV\, .
\end{eqnarray}
We work at
 NLO QCD, use CT14qed-inc-proton PDFs, and take the renormalization/factorization scales to be $M_{WW}/2$. We assume the $Wl\nu$ couplings
 in the decays are SM-like.

The results of the scans are shown in Figs.~\ref{fig:atfig14} and \ref{fig:atfig27}; the 
allowed regions are within the ellipses.   We see a significant improvement going from $14~TeV$ to $27~TeV$, while
the improvement from reducing the systematic error, $\delta_{sys}=.16\rightarrow .04$, is marginal. 
We allow the fermion couplings to vary around $0$, assuming the $2\sigma$ errors from fits to LEP
data.
As can be seen, by including the anomalous fermion
couplings, the  sensitivity of the scan is significantly reduced~\cite{Baglio:2017bfe,Grojean:2018dqj}. 
 This effect is quite pronounced at $27~TeV$ and implies that global fits to both anomalous fermion and $3$ gauge boson couplings are necessary.

 \begin{figure}
  \centering
\subfloat{\includegraphics[width=0.32\textwidth]{\main/electroweak/img/ww/g2g1_14tev_ferm2.pdf}}
\subfloat{\includegraphics[width=0.32\textwidth]{\main/electroweak/img/ww/g2g3_14tev_ferm2.pdf}}
\subfloat{\includegraphics[width=0.32\textwidth]{\main/electroweak/img/ww/g3g1_14tev_ferm2.pdf}}
 \caption{Projections for $14$ TeV with $3~ab^{-1}$.
 We take $p_{T,cut}=750$~GeV, corresponding to $\delta_{stat}=.16$  and 
consider $\delta_{sys}=.04$ and $\delta_{sys}=.16$.  The curves labelled 3GB have SM $Z$-fermion couplings, while the curves labelled 3GB +Ferm' allow the $Z$-fermion couplings to vary around a central value of $0$.}
   \label{fig:atfig14}
\end{figure}

\begin{figure}
  \centering
\subfloat{\includegraphics[width=0.32\textwidth]{\main/electroweak/img/ww/g2g1_27tev_ferm2.pdf}}
\subfloat{\includegraphics[width=0.32\textwidth]{\main/electroweak/img/ww/g2g3_27tev_ferm2.pdf}}
\subfloat{\includegraphics[width=0.32\textwidth]{\main/electroweak/img/ww/g3g1_27tev_ferm2.pdf}}
 \caption{Projections for $27$ TeV with $15~ab^{-1}$.
 We take $p_{T,cut}=1350$~GeV, corresponding to $\delta_{stat}=.16$  and 
consider $\delta_{sys}=.04$ and $\delta_{sys}=.16$. The curves labelled 3GB have SM $Z$-fermion couplings, while the curves labelled 3GB +Ferm' allow the $Z$-fermion couplings to vary around a central value of $0$. }
   \label{fig:atfig27}
\end{figure}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Prospects for the measurement of the $W$-boson mass}

%%%%%%%%%%%%%%%%%%%%%%%%
%%% ATLAS Contribution
%%%%%%%%%%%%%%%%%%%%%%%%

%AT \documentclass[10pt,a4paper]{article}

%AT \addbibresource{YR_mW_git.bib}

%-------------------------------------------------------------------------------                                                                                                                          
% Generic document information                                                                                                                                                                            
%-------------------------------------------------------------------------------                                                                                                                          

% Title, abstract and document                                                                                                                                                                            
\newcommand{\avg}[1]{\ensuremath{\left< #1 \right>}}
%\newcommand*{\pT}{\ensuremath{p_\text{T}}\xspace}
\newcommand*{\pTl}{\ensuremath{\pT^{\ell}}\xspace}
\newcommand*{\met}{\ensuremath{E_{\text{T}}^{\text{miss}}}\xspace}
\newcommand*{\vecpTl}{\ensuremath{\vecpT^{\ell}}\xspace}
\newcommand*{\pTel}{\ensuremath{\pT^{e}}\xspace}
\newcommand*{\pTmu}{\ensuremath{\pT^{\mu}}\xspace}
%\newcommand*{\eta_{\ell}}{\ensuremath{\eta_{\ell}}\xspace}
\newcommand*{\phil}{\ensuremath{\phi_{\ell}}\xspace}
\newcommand*{\phimiss}{\ensuremath{\phi_\text{miss}}\xspace}
\newcommand*{\mT}{\ensuremath{m_\text{T}}\xspace}
\newcommand*{\uT}{\ensuremath{u_\text{T}}\xspace}
\newcommand*{\pTW}{\ensuremath{\pT^{W}}\xspace}
\newcommand*{\pTZ}{\ensuremath{\pT^{Z}}\xspace}
\newcommand*{\pTV}{\ensuremath{\pT^{V}}\xspace}
\newcommand*{\vecpT}{\ensuremath{\vec{p}_{\text{T}}}\xspace}
\newcommand*{\vecmet}{\ensuremath{\vec{E}_{\text{T}}^{\text{miss}}}\xspace}
\newcommand*{\ipb}{\mbox{pb$^{-1}$}}
\newcommand*{\ifb}{\mbox{fb$^{-1}$}}

\setlength\parindent{0pt}

%AT \begin{document}

%AT \title{Prospects for the measurement of the W -boson mass at the HL- and HE-LHC}

%\tableofcontents                                                                                                                                                                                         

% List of contributors - print here or after the Bibliography.                                                                                                                                            
%\PrintAtlasContribute{0.30}                                                                                                                                                                              
%\clearpage                                                                                                                                                                                               

%-------------------------------------------------------------------------------                                                                                                                         
Special low pile-up proton-proton collision data at the HL-LHC (and HE-LHC) will be of large interest for $W$ boson physics. At $\sqrt{s}=14$~TeV and for an instantaneous luminosity of ${\cal L}\sim 5\times 10^{32}$~$\text{cm}^{-2} \text{s}^{-1}$, corresponding to two collisions per bunch crossing on average, about 2$\times 10^6$ W boson events can be collected in one week. Such a sample provides a statistical sensitivity at the permille level for cross section measurements, at the percent level for measurements of the $W$ boson transverse momentum distribution, and of about 10~MeV for a measurement of $m_W$. The increased acceptance provided by the new inner detector in ATLAS, the ITk~\cite{Collaboration:2017mtb}, extends the coverage in pseudorapidity from $|\eta|<2.5$ to $|\eta|<4$ and allows further constraints on the parton density functions (PDFs) from cross section measurements, reducing the corresponding uncertainties in the measurement of $m_W$. An energy increase at the HE-LHC to $\sqrt{s}=27$~TeV~\cite{Zimmermann:2017bbr} could play a similar role. 
A first quantitative study of the potential improvement in the W-boson mass using low pile-up data at the HL-LHC and HE-LHC is discussed in~\cite{ATLAS:mWPubNote} considering only statistical and PDF uncertainties. Experimental systematic uncertainties can be maintained at a level similar to the statistical uncertainty, since they are largely dominated by the statistics of the low pile-up samples. Other theoretical uncertainties in the modelling of the $W$-boson production, like the description of the boson transverse momentum distribution, will also be constrained by measurements using these data.\\

Leptonic $W$ boson decays are characterized by an energetic, isolated electron or muon, and significant missing transverse momentum reflecting the decay neutrino. The hadronic recoil, \uT, is defined
from the vector sum of the transverse momenta of all reconstructed particles in the event excluding the charged lepton, and provides a measure of the $W$ boson transverse momentum. The lepton transverse momentum, \pTl, the missing transverse momentum, \met, and the hadronic recoil are related through $\vecmet = -(\vecpTl + \vec{\uT})$. The \pTl and \met distributions have sharp peaks at $\pTl\sim\met\sim m_W/2$. The transverse mass \mT, defined as $\mT=\sqrt{2 \pTl \met \cos(\phil-\phimiss)}$, peaks at $\mT\sim m_W$.

Events are generated at $\sqrt{s}=14$ and 27~TeV using the \textsc{W\_ew\_bmnnp} process~\cite{Barze:2012tt} of the \textsc{Powheg v1} event generator~\cite{Alioli:2010xd}, with electroweak corrections
switched off. The CT10 PDF set~\cite{Lai:2010vv} is used, and parton shower effects are included using the \textsc{Pythia8} event generator~\cite{Sjostrand:2014zea} with parameters set according to
the AZNLO tune~\cite{STDM-2012-23}. Final-state QED corrections are applied using \textsc{Photos}~\cite{Davidson:2010ew}. The energy resolutions of the lepton and hadronic recoil are parameterised as a function of the truth-related observables in order to emulate detector effects. These parameterised resolutions are checked against simulated distributions at the reconstructed level, and they agree at a few percent level. 

%During four weeks in 2017 and 2018, ATLAS recorded $pp$ collision data at low pile-up and two centre-of-mass energies, $\sqrt{s}=5$ and 13~TeV. For the analysis of these data, events generated as described above, and passed through the full ATLAS simulation~\cite{SOFT-2010-01}. Pile-up is simulated using \textsc{Pythia}, and the average number of collisions per bunch crossing is set to $\avg{\mu}\sim 2$, matching the data taking conditions. 
Events are selected applying the following cuts to the object kinematics, after resolution corrections: $\pTl>25$~GeV, $\met>25$~GeV, $\mT>50$~GeV and $\uT<15$~GeV; $|\eta_{\ell}|<2.4$ or $2.4<|\eta_{\ell}|<4$. The first set of cuts selects the range of the kinematic peaks of the $W$ boson decay products, restricting to the region of small \pTW to maximize the sensitivity of the distributions to $m_W$. Two pseudorapidity ranges are considered, corresponding to the central region accessible with the current ATLAS detector, and to the forward region accessible in the electron channel with the ITk.
%Signal cross sections, acceptance and the expected number of selected events, accounting for typical electron and muon selection efficiencies, are calculated at $O(\alpha_S)$ using \textsc{Powheg}; $O(\alpha_S^2)$ corrections would increase these numbers by 2 to 5\% depending on the $W$ boson charge and $\sqrt{s}$. Small acceptance losses in the
%transition regions between the barrel, endcap and forward calorimeter systems are neglected. \\ 

The Monte Carlo samples are produced using the CT10 PDF set, $m_W^\text{ref}=80.399$~GeV, and the corresponding Standard Model prediction for $\Gamma_W$. Kinematic distributions for the different values of $m_W$ are obtained by applying an event weight to the reference samples based on the ratio of the Breit--Wigner densities corresponding to $m_W$ and $m_W^\text{ref}$, for a given value of the final state invariant mass. A similar event weight, calculated internally by \textsc{Powheg} and corresponding to the ratio of the event cross sections predicted by CT10 and several alternate PDFs, is used to obtain final state
distributions corresponding to the CT14~\cite{Dulat:2015mca}, MMHT2014~\cite{Harland-Lang:2014zoa}, HL-LHC~\cite{Khalek:2018mdn} and LHeC~\cite{Klein:1564929} PDF sets and their associated uncertainties. Compared to current sets such as CT14 and MMHT2014, the HL-LHC set incorporates the expected constraints from present and future LHC data; it starts from the PDF4LHC convention~\cite{Butterworth:2015oua} and comes in three scenarios corresponding to more or less optimistic projections of the experimental uncertainties. The LHeC PDF set represents the impact of a proposed future high-energy, high-luminosity $ep$ scattering experiment~\cite{AbelleiraFernandez:2012cc} on the uncertainties in the proton structure, using the theoretically best understood process for this purpose.

The shift in the measured value of $m_W$ resulting from a change in the assumed PDF set is estimated as follows. Considering a set of template distributions obtained for different values of $m_W$ and
a given reference PDF set, and ``pseudo-data'' distributions obtained for $m_W=m_W^\text{ref}$ and an alternate set $i$ (representing, for example, uncertainty variations with respect to the reference
set), the preferred value of $m_W$ for this set is determined by minimizing the $\chi^2$ between the pseudo-data and the templates. The preferred value is denoted $m_W^i$, and the corresponding variation is defined as $\delta m_W^i = m_W^i -m_W^\text{ref}$. The statistical uncertainty on the measurement is estimated from the half width of the $\chi^2$ function one unit above the minimum.

The present study considers measurements of $m_W$ in separate categories, corresponding to $W^+$ and $W^-$ events; five pseudorapidity bins, $|\eta_{\ell}|<0.6$, $0.6<|\eta_{\ell}|<1.2$, $1.2<|\eta_{\ell}|<1.8$,
$1.8<|\eta_{\ell}|<2.4$, and $2.4<|\eta_{\ell}|<4$; \pTl and \mT distribution fits; and two centre-of-mass energies ($\sqrt{s}=14$ and $27$~TeV). For each category $\alpha$ and for the PDF sets considered here,
the Hessian uncertainty corresponding to a given set is estimated as $\delta m_{W\alpha}^+ = \left[\sum_i \left({\delta m_{W\alpha}^i}\right)^2\right]^{1/2}$, if $\delta m_{W\alpha}^i>0$, and as $\delta m_{W\alpha}^- = \left[\sum_i \left({\delta m_{W\alpha}^i}\right)^2\right]^{1/2}$, if $\delta m_{W\alpha}^i<0$, where $i$ runs over the uncertainty sets, and $\delta m_{W\alpha}^i$ is calculated with respect to the reference PDF set. For CT10 and CT14, the uncertainties are divided by a factor 1.645 to
match the 68\% CL. Only symmetrized uncertainties, $\delta m_{W\alpha} = (\delta m_{W\alpha}^+ + \delta m_{W\alpha}^-)/2$, are considered for simplicity. The correlation of PDF uncertainties between different measurement categories is
calculated as $\rho_{\alpha\beta} = \frac{\sum_i \delta m_{W\alpha}^i \delta m_{W\beta}^i}{\delta m_{W\alpha}\delta m_{W\beta}}$. 

PDF variations generate correlated variations in the \pTW and \pTZ distributions, while the latter are strongly constrained by experimental data~\cite{STDM-2012-23,STDM-2014-12}. These
constraints were used in the ATLAS measurement of $m_W$~\cite{STDM-2014-18}, bringing significant reduction in the PDF uncertainties. The uncertainties estimated here are thus conservative from
this perspective, and partly account for uncertainties in the \pTW distribution.

The overall measurement precision is evaluated by combining the results obtained in the different categories using the BLUE prescription~\cite{Valassi:2003mu}. Only statistical and PDF uncertainties
are considered. The former are assigned assuming an integrated luminosity of 200~\ipb, and normalizing the samples to the expected cross-sections. 
The expected measurement uncertainties, together with their statistical and PDF components, are summarized in Figure~\ref{fig:ct10unc} (a) for CT10. The numbers quoted for $0<|\eta_{\ell}|<2.4$ correspond to the combination of the four pseudorapidity bins in this range. Moderate or negative PDF uncertainty correlations, leading to reduced combined uncertainties, are observed between categories of different $W$-boson charges, and between central and forward pseudorapidities, at given $\sqrt{s}$. On the other hand, PDF uncertainty correlations tend to be large and positive between $\sqrt{s}=14$ and 27~TeV, for a given boson charge and lepton pseudorapidity range. With 200~\ipb of data collected at each energy, a total uncertainty of about 10~MeV is obtained. 

Table~\ref{tab:pdfcomp} and Figure~\ref{fig:ct10unc} (b) compare the uncertainties obtained for different PDF sets. The CT10 and CT14 sets display similar uncertainty correlations, leading to similar
improvement under combination of categories, and yielding comparable final PDF uncertainties. The MMHT2014 uncertainties are about 30\% lower. The three projected HL-LHC PDF sets give very similar
uncertainties; the most conservative one is shown here. Compared to CT10 and CT14, a reduction in PDF uncertainty of about a factor of two is obtained. The LHeC projection results from a QCD fit to 1 ab$^{-1}$ of $ep$ scattering pseudodata, with $E_e=60$~GeV and $E_p=7$~TeV. Such a sample could be collected in about five years, synchronously with the HL-LHC operation. In this configuration, the neutral- and charged-current DIS samples are sufficient to disentangle the first and second generation parton densities without ambiguity, and reduce the PDF uncertainty below 2~MeV, a factor 5--6 compared to present knowledge. Also in this case the $m_W$ measurement will benefit from the large $W$ boson samples collected at the LHC, and from the anti-correlation between central and forward categories. In this context, PDF uncertainties would still be sub-leading with 1 \ifb\ of low pile-up data. \\ 

%%%%
\begin{figure}
  \begin{center}
    \subfloat[]{\includegraphics[width=0.45\textwidth]{\main/electroweak/img/ew_precision/deltamw_statpdf.pdf}}
    \subfloat[]{\includegraphics[width=0.45\textwidth]{\main/electroweak/img/ew_precision/deltamw_allpdfs.pdf}}
  \end{center}
  \caption{Measurement uncertainty for combined fits to the \pTl and \mT distributions (a) in different lepton acceptance regions and for different centre-of-mass energies, using the CT10 PDF set and for 200~\ipb collected at each energy and (b) for different PDF sets in $|\eta_{\ell}|<4$, for 200~\ipb and 1~\ifb collected at $\sqrt{s}=14$~TeV. The numbers quoted for $0<|\eta_{\ell}|<2.4$ correspond to the combination of the four pseudorapidity bins in this range. \label{fig:ct10unc}}
\end{figure}

%%%%
\begin{table}
  \begin{center}
    \scalebox{0.9}{
    \begin{tabular}{clccccc}
      \toprule
      $\sqrt{s}$ [TeV] & Lepton acceptance  & \multicolumn{3}{c}{Uncertainty in $m_W$ [MeV]}    \\
      \multicolumn{2}{c}{} & CT10       & CT14      & MMHT2014 \\
      14    & $|\eta_{\ell}|<2.4$   & 16.0 (10.6 $\oplus$ 12.0) & 17.3 (11.4 $\oplus$ 13.0) & 15.4 (10.7 $\oplus$ 11.1) \\
      14    & $|\eta_{\ell}|<4$     & 11.9 (8.8 $\oplus$ 8.0) & 12.4 (9.2 $\oplus$ 8.4) & 10.3 (9.0 $\oplus$ 5.1) \\
      27    & $|\eta_{\ell}|<2.4$   & 18.3 (10.2 $\oplus$ 15.1) & 18.8 (10.5 $\oplus$ 15.5) & 16.5 (9.4 $\oplus$ 13.5) \\
      27    & $|\eta_{\ell}|<4$     & 12.3 (7.5 $\oplus$ 9.8) & 12.7 (8.2 $\oplus$ 9.7) & 11.4 (7.9 $\oplus$ 8.3)\\
      14+27 & $|\eta_{\ell}|<4$     & 10.1 (6.3 $\oplus$ 7.9) & 10.1 (6.9 $\oplus$ 7.4) & 8.6 (6.5 $\oplus$ 5.5) \\
      \bottomrule
    \end{tabular}}
  \end{center}
  \begin{center}
    \scalebox{0.9}{
    \begin{tabular}{clccc}
      \toprule
      $\sqrt{s}$ [TeV] & Lepton acceptance & \multicolumn{2}{c}{Uncertainty in $m_W$ [MeV]}    \\
      \multicolumn{2}{c}{} & HL-LHC & LHeC \\
      14    & $|\eta_{\ell}|<2.4$   & 11.5 (10.0 $\oplus$ 5.8 ) & 10.2 (9.9 $\oplus$ 2.2) \\
      14    & $|\eta_{\ell}|<4$     & 9.3 (8.6 $\oplus$ 3.7)    & 8.7 (8.5 $\oplus$ 1.6) \\
      \bottomrule
    \end{tabular}}
    \caption{Measurement uncertainty for different lepton acceptance regions, centre-of-mass energies and PDF sets, combined fits to the \pTl and \mT distributions, and for 200~\ipb collected at each energy. The numbers quoted for $0<|\eta_{\ell}|<2.4$ correspond to the combination of the four pseudorapidity bins in this range. In each case, the first number corresponds to the sum of statistical and PDF uncertainties, and the numbers between parentheses are the statistical and PDF components, respectively.\label{tab:pdfcomp}}
  \end{center}
\end{table}
%AT \clearpage
%AT \printbibliography
%AT \end{document}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\smallw}{{\scriptscriptstyle W}}
\newcommand{\smallv}{{\scriptscriptstyle V}}
\newcommand{\smallz}{{\scriptscriptstyle Z}}
\newcommand{\mv}{m_\smallv} 
\newcommand{\mw}{m_\smallw} 
\newcommand{\mz}{m_\smallz} 
\newcommand{\nnpdftz}{{\sc NNPDF3.0\,}} 
\newcommand{\fbinv} {\mbox{\ensuremath{\,\text{fb}^\text{$-$1}}}\xspace}
\newcommand{\powhegeww}{{\sc W\_ew-BMNNP}}
\newcommand{\powhegewz}{{\sc Z\_ew-BMNNPV}}
\newcommand{\powhegbox}{{\sc Powheg-Box}}
%\newcommand{\pt}{\ensuremath{p_{\mathrm{T}}}\xspace}

\subsubsection{Reduction of the PDF uncertainties on EWPO}
{\bf authors: Alessandro Vicini, Fulvio Piccinini}

We study the EW precision observables (EWPO) and
focus on the mass of the $W$ boson $\mw$.

\paragraph{Indirect reduction}
The runs at the HL-LHC will allow a very precise measurement
of several scattering processes
relevant for the determination of the proton PDFs.
The resulting reduction of the PDF uncertainty will allow
a new better reanalysis of the Drell-Yan (DY) kinematic distributions
and eventually a reduction of the PDF uncertainty affecting
the $\mw$ determination.
We call this approch indirect in contrast to the inclusion of new independent
determinations of $\mw$, which might contribute to the reduction of the error
of the world average value.

We estimate the impact on the prediction of an observable ${\cal O}$,
due to the improvement of the PDF parameterization,
with a reweighing approach:
\begin{enumerate}
\item
  we generate pseudodata that will play the role of the final HL-LHC results;
  to this goal we simulate DY kinematic distributions
with the central replica of a given PDF set and add to each bin some random
noise gaussianly distributed around the theoretical prediction;
  the width of the noise distribution is consistent with the projections
  for the statistical error at the end of the HL-LHC runs;
\item
  we compute the same distribution with all the 100 replicas of the PDF set;
with the current knowledge the 100 replicas are fully equivalent to each other
in the description of the old data from which they have been determined;
\item
  we compute a weigth, as described below, for each of the 100 distributions;
the weigth expresses the compatibility of each prediction with the
new (pseudo)data;
  the weight assigned to the replica $k$ is
\bea
w_k &\propto& \chi_k^{N_{bins}-1}\exp\left(-\frac12 \chi_k^2 \right)
\quad{\rm where}\quad
\chi_k^2 = \frac{1}{N_{bins}} \sum_{j=1}^{N_{bins}}
\frac{({\cal O}_j^{(k)}-{\cal O}_j^{exp}    )^2}{\left( \sigma^{exp}_j \right)^2}
\label{eq:pdfweights}
\eea
with the normalization condition $\sum_{i=1}^{N_{rep}}\,w_i\,=\,N_{rep}$.
\item
  For a generic observable ${\cal O}$
we compute now the mean value and standard deviation
with respect to the different replicas of a PDF parameterization,
taking into account the effect of the new (pseudo)data;
to this goal we evaluate a weighted average with weights $w_i$.
\bea
\langle {\cal O} \rangle_{{\scriptscriptstyle PDF}}
&=&
\frac{1}{N_{rep}}\,
\sum_{i=1}^{N_{rep}} w_i {\cal O}_i\, ,
\quad\quad
\sigma_{{\scriptscriptstyle PDF}}^2
=
\frac{1}{N_{rep}-1}\,
\sum_{i=1}^{N_{rep}}\, w_i\,
( {\cal O}_i - \langle {\cal O} \rangle_{{\scriptscriptstyle PDF}})^2
\label{eq:pdfmeanstd}
\eea
\item
  The mean value and standard deviation that ignore the impact of the new data
are recovered by setting all the weights $w_i=1$.
This reweighting technique allows to estimate the future impact of new data
on the prediction of a given observable, before a full consistent fit
becomes available.
\end{enumerate}

The $W$ boson mass $\mw$ is extracted from kinematic distributions
by means of a template fit technique:
the best available theoretical simulation tool is used to generate
several predictions for the distribution, varying $\mw$, i.e. the fit parameter;
the distribution that maximizes the agreement with the data selects
the preferred, i.e. measured, $\mw$ value.
The theoretical distributions, also called templates, depend on the assumptions
used in their evaluation, in particular on the PDF set chosen to describe the
proton. The PDF uncertainty affects the templates and in turn the final value
of the fit and has to be considered as a theoretical systematic uncertainty.

An improvement in the PDF parameterization yields a reduced spread of the
predicted templates and eventually a smaller PDF uncertainty
on the fit $\mw$ value.
With the reweighting approach we anticipate the impact that HL-LHC data
can have on a reanalysis of the current data used to extact $\mw$,
setting ${\cal O}=\mw$ in equation (\ref{eq:pdfmeanstd}).


\paragraph{Direct reduction}
At the HE-LHC, it will be possible
to perform new determinations of $\mw$ in a new experimental setup.
The different kinematic regime and, in particular, the new range
of partonic $x$ relevant for the production of a $W$ or a $Z$ boson,
will lead to PDF uncertainties different but correlated to the ones
relevant for the 13 TeV measurements.
A combination of the $\mw$ values extracted at different collider energies,
including both $W^+$ and $W^-$ channels with their correlation
with respect to PDF variations,
may have a reduced total PDF uncertainty.

This study will be conducted under the assumption
that the PDF parameterization adopted at HE-LHC
to compute the templates and analyze the data
will be the one available at the end of the HL-LHC runs.
We include in our study this assumption,
by using the weights $w_i$ derived in the HL-LHC study with
equation (\ref{eq:pdfweights}).
The impact of the correlation between the $\mw$ determination
at different energies can be derived according to standard rules
\bea
\sigma^2_{PDF,13+27} &=&
\sigma^2_{PDF,13}\,+\,\sigma^2_{PDF,13}\,+\,2\sigma_{13,27}\\
\sigma^2_{13,27} &=&
\langle m_{\smallw,13 TeV}\,\, m_{\smallw,27 TeV}  \rangle_{{\scriptscriptstyle PDF}}
-
\langle m_{\smallw,13 TeV}  \rangle_{{\scriptscriptstyle PDF}}
\langle m_{\smallw,27 TeV}  \rangle_{{\scriptscriptstyle PDF}}
\eea
for all the combinations of the $W^+$ and $W^-$ channels.

\paragraph{Results}
All the simulations used in this analysis have been obtained
with the codes \powhegeww and \powhegewz present in the \powhegbox.
The input parameters of the calculation are
\be
\alpha(0)=(137.03599911 )^{-1},\,
G_\mu=1.16637\,10^{-5}\,\, {\rm GeV}^{-2},\,
\mw=80.385\,\, {\rm GeV},\,
\mz=91.1876\,\, {\rm GeV}
\ee
and $\alpha_s(\mz^2)=0.118$ consistently with the \nnpdftz choice
for the proton parameterization.
The acceptance cuts adopted to select the final state leptons are:
\be
p_\perp^\ell>25 {\rm GeV},\quad
p_\perp^{miss}> 25 {\rm GeV},\quad
|\eta_\ell|< 2.5
\ee

We present in figure \ref{fig:wpmwlumi}
the PDF spread of the $\mw$ values according to \nnpdftz,
under the assumption of the inclusion of additional data sets
available at the end of the HL-LHC run
and compare it to the current estimate for the PDF uncertainty.
In this figure
$\mw$ is extracted from a template fit to the lepton transverse momentum
distribution of the process $pp\to \ell^+\nu_\ell+X$
at 13 TeV of collider energy.
We assume to include in the PDF determination:
the charged lepton transverse momentum distribution in CC-DY,
at large transverse momentum values;
the lepton-pair transverse momentum distribution in NC-DY,
at large transverse momentum values.
We generate pseudodata using the central replica of \nnpdftz
and add a gaussianly distributed noise corresponding to the statistical error
of the data collected with
an integrated luminosity of 6 ab$^{-1}$.
\vskip1cm


We present in figure \ref{fig:wpmwenergy}
the PDF spread of the $\mw$ values according to \nnpdftz;
In this figure $\mw$ is extracted from a template fit to the lepton
transverse momentum distribution at 13, 14 and 27 TeV of collider energy.
The combination of the results, including the evaluation of the correlation
with respect to PDF replica variations is
$\mw=80.385\pm XXX$
with $(aa,bb,cc)$ the variance of $\mw$ about its mean value at
respectively 13, 14 and 27 TeV
and with $(rr,ss,tt)$ the $(\sigma^2_{13,14},\sigma^2_{13,27},\sigma^2_{14,27})$
the three covariances between the three data sets.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Prospects for measurement of the effective weak mixing angle}

{\bf **AT** Missing Contribution expected by ATLAS}

\newcommand{\zmumu}{\ensuremath{\cPZ/\gamma^*\to \MM\xspace}}
\newcommand{\zee}{\ensuremath{\cPZ/\gamma^*\to \EE\xspace}}
\newcommand{\ztautau}{\ensuremath{\cPZ/\gamma^*\to \TT \xspace}}
\newcommand{\zll}{\ensuremath{\cPZ/\gamma^*\to \ell^+\ell^-\xspace}}
\newcommand{\csh}{\ensuremath{\cos\theta^{*}}\xspace}
\newcommand{\sineff}{\ensuremath{\sin^2\theta^{\text{lept}}_{\text{eff}}}\xspace}
\newcommand{\pt}{\ensuremath{p_{\mathrm{T}}}\xspace}
\newcommand{\llll}{\ensuremath{\ell\ell\xspace}}

\subsubsubsection{Introduction}

We report on a proposal for the  measurement of the effective weak mixing angle using the forward-backward asymmetry, $\mathrm{}{A_{FB}}$, in Drell-Yan $\mu\mu$ events at the HL-LHC at CMS. The proposal is based on techniques used in Ref.~\cite{CMS-PAS-SMP-16-007} for such a  measurement at $\sqrt{s} = 8\UTeV$.

In leading order dilepton pairs are produced through the annihilation of a quark and antiquark via the exchange of a  $\PZ$ boson or a virtual photon: $\Pq\bar{\Pq}\rightarrow Z/\gamma^*\rightarrow \ell^+\ell^-$. The definition of  $\mathrm{A_{FB}}$ is based on the angle $\theta^*$ of the lepton ($\ell^-$) in the Collins-Soper~\cite{Collins} frame of the dilepton system:
\begin{equation} \mathrm{A_{FB}}=\frac{\sigma_\text{F}-\sigma_\text{B}}{\sigma_\text{F}+\sigma_\text{B}},
\end{equation}
where $\sigma_\text{F}$ and $\sigma_\text{B}$ are the cross sections in the forward ($\csh>0$) and backward ($\csh<0$) hemispheres, respectively. In this frame the $\theta^*$ is the angle of the $\ell^-$ direction with respect to the axis that bisects the angle between the direction of the quark and opposite direction of the anti-quark. In $\Pp\Pp$ collisions the direction of the quark is assumed to be in the boost direction of the dilepton pair. Here, \csh is calculated using  laboratory-frame quantities as follows:
\begin{equation} \csh=\frac{2(p_1^+p_2^- - p_1^-p_2^+)}{\sqrt{M^2(M^2+P_\text{T}^2)}}\times\frac{P_\text{z}}{|P_\text{z}|},
\end{equation}
where $M$, $P_\text{T}$, and $P_\text{z}$ are the mass, transverse momentum, and longitudinal momentum, respectively, of the dilepton system, and $p_1(p_2)$ are defined in terms of energy, $e_1 (e_2)$, and longitudinal momentum, $p_{\text{z},1}(p_{\text{z},2})$, of the negatively (positively) charged lepton as $p_\text{i}^\pm=(e_i\pm p_{\text{z},i})/\sqrt{2}$~\cite{Collins}. 

A non-zero $\mathrm{A_{FB}}$ in dilepton events arises from the vector and axial-vector couplings of electroweak bosons to fermions. At tree level, the vector $v_\text{f}$ and axial-vector $a_\text{f}$ couplings of $\PZ$ bosons to fermions (f) are:
\begin{gather}
    \begin{align}
	v_\text{f}&= T_3^\text{f}-2Q_\text{f}\sin^2\theta_\text{W}, \\ 
	a_\text{f}&= T_3^\text{f},
    \end{align}
\end{gather}
where $T_3^\text{f}$ and $Q_\text{f}$ are the third component of the weak isospin and the charge of the fermion, respectively, and $\sin^2\theta_\text{W}$ is the weak mixing angle, which is related to the masses of the $\PW$ and $\PZ$ bosons by the relation $\sin^2\theta_\text{W} =1-M_\text{W}^2/M_\text{Z}^2$. Electroweak radiative corrections affect these leading-order relations. 
An effective weak mixing angle, 
$\sin^2\theta_{\text{eff}}^\text{f}$,  
is defined based on the relation between these couplings: 
$v_\text{f}/a_\text{f}=1-4|Q_\text{f}|\sin^2\theta_{\text{eff}}^\text{f}$, 
with 
$\sin^2\theta_{\text{eff}}^\text{f}=\kappa_{\text{f}} \sin^2\theta_\text{W}$, 
where flavor-dependent $\kappa_{\text{f}}$ is determined by electroweak corrections. 
$\mathrm{A_{FB}}$ for dilepton events is primarily sensitive to the leptonic effective weak mixing angle (\sineff).

In this analysis we measure the leptonic effective weak mixing angle  (\sineff) by fitting the mass and rapidity dependence of the observed $\mathrm{A_{FB}}$ in dilepton events. The most precise  previous measurements of \sineff were performed by the LEP and SLD experiments~\cite{ALEPH:2005ab}. There is, however, a known tension of about 3 standard deviations between the two most precise measurements. Measurements of \sineff were also reported by the LHC and Tevatron experiments~\cite{Chatrchyan:2011ya,Aad:2015uau,Aaij:2015lka,Aaltonen:2014loa,Aaltonen:2016nuy,Abazov:2014jti}. The latest and the most
precise LHC measurement was done by 
CMS~\cite{CMS-PAS-SMP-16-007}, and its machinery is 
 used in this analysis.

The analysis is based on samples of $\Pp\Pp$ collisions simulated at $\sqrt{s}=8$ and 14\UTeV with next-to-leading order (NLO) matrix element implemented in the POWHEG event generator~\cite{POWHEG0,POWHEG1,POWHEG2,POWHEG3} using the NNPDF3.0~\cite{NNPDF30} PDFs and interfaced with PYTHIA8~\cite{PYTHIA8} with CUETP8M1*~\cite{tune} underlying event tune for parton showering and hadronization and electromagnetic final-state radiation (FSR). The template variations for different values of \sineff and PDFs are modeled using the POWHEG MC generator that provides matrix-element based event-by-event weights for each variation. The samples are normalized to the integrated luminosities of 19\fbinv for $\sqrt{s} = 8\UTeV$ and to 10 -- 3000\fbinv for $\sqrt{s} = 14\UTeV$ samples. The analysis is done at the generator level, so the smearing due to detector effects is not taken into account, but 
comparison of 8\UTeV predictions and measured values suggests that this effect is not significant. Moreover since the results are presented as comparison of 8 and 14\UTeV measurements they can be directly applied to the measured 8\UTeV results with real data.  

The HL-LHC CMS detector extends the pseudorapidity, $\eta$, coverage for the muon reconstruction from current configuration of 2.4 to 2.8. In 
this analysis an event is selected if there are at least two muons with ${|\eta|} < 2.8$ and  with the leading (i.e. having the largest transverse momentum \pt muon $\pt> 25\UGeV$ and the second leading muon $\pt>15\UGeV$. 


\subsubsubsection{\texorpdfstring{\sineff}{Lg} extraction}

We extract \sineff  by minimizing the $\chi^2$ value between the simulated data and template $\mathrm{A_{FB}}$ distributions in 72 dilepton mass and rapidity bins. Figure~\ref{figure:afb} shows the $\mathrm{A_{FB}}$ distributions in bins of dimuon mass and rapidity for different energies and pseudorapidity acceptances. As expected, at higher center-of-mass energies the observed $\mathrm{A_{FB}}$ is smaller because the interacting partons have smaller $x$-values which results in a smaller fraction of dimuon events produced by the valence quarks, which also means more dilution. The simulated data are shown for $\sqrt{s} = 8\UTeV$ and $\sqrt{s}=14\UTeV$ for two 
different selection requirements, $|\eta| < 2.4$ and 2.8. 
Extending the pseudorapidity acceptance significantly increases the coverage for larger $x$-values in the production and reduces both the statistical and PDF uncertainties, as shown below.

\begin{figure}[!htbp]
\centering
    \includegraphics[scale=0.8]{\main/electroweak/img/ew_precision/afb1.pdf}
    \caption{
	Forward-backward asymmetry distribution, 
    $\mathrm{A_{FB}}(M_{\mu\mu},Y_{\mu\mu})$, in dimuon events at $\sqrt{s}=8\UTeV$ and 14\UTeV. 
	The distributions are made with POWHEG event generator using NNPDF3.0 PDFs and interfaced with PYTHIA8 for parton-showering, 
	QED final-state radiation (FSR) and hadronization. 
	Following acceptance selections are applied to the generated muons after FSR: $|\eta|<2.4$ (or $|\eta|<2.8$), $\pt^\mathrm{lead}>25\UGeV$, $\pt^\mathrm{trail}>15\UGeV$. 
	The error bars represent the statistical uncertainties for the integrated luminosities corresponding to 19\fbinv at $\sqrt{s}=8\UTeV$ and 3000\fbinv at $\sqrt{s}=14\UTeV$.}
 \label{figure:afb} 
    
\end{figure}


The observed $\mathrm{A_{FB}}$ values depend on the size of the dilution effect, as well as on the relative contributions from u and d valence quarks to the total dilepton production cross section. Therefore, the PDF uncertainties translate into sizable variations in the observed $\mathrm{A_{FB}}$ values. However, changes in PDFs affect the $\mathrm{A_{FB}}(M_{\llll},Y_{\llll})$ distribution in a different way from changes in \sineff. Changes in PDFs result in changes in $\mathrm{A_{FB}}$'s in regions where the absolute values of $\mathrm{A_{FB}}$ is large, i.e. at high and low dilepton masses. On the contrary, the effect of changes in \sineff are largest near the Z-peak and are significantly smaller at high and low masses. Because of this behavior, which is illustrated in Fig.~\ref{figure:variations}, we apply the Bayesian $\chi^2$ reweighting method to constrain the PDF uncertainties~\cite{Giele:1998gw,Sato:2013ika,Bodek:2016olg} and  reduce the PDF errors in the extracted value of \sineff.

\begin{figure}[!htbp]
\centering
    \includegraphics[scale=0.7]{\main/electroweak/img/ew_precision/variationsPDFy.pdf}
    \caption{
	Forward-backward asymmetry distribution, 
    $\mathrm{A_{FB}}(M_{\mu\mu},Y_{\mu\mu})$, in dimuon events at $\sqrt{s}=14\UTeV$. 
	The distributions are made with POWHEG event generator using NNPDF3.0 PDFs and interfaced with PYTHIA8 for parton-showering, QED final-state radiation (FSR) and hadronization. 
	Following acceptance selections are applied to the generated muons after FSR: $|\eta|<2.8$, $\pt^\mathrm{lead}>25\UGeV$, $\pt^\mathrm{trail}>15\UGeV$. 
	The solid lines in the bottom panel correspond to six variations of \sineff around the central value: $\pm0.0004$, $\pm0.0008$, and $\pm0.0012$. 
	The shaded band shows the standard deviation over the 100 NNPDF3.0 replicas. 
    \label{figure:variations} 
    }
\end{figure}

As a baseline, we use the NLO NNPDF3.0 set. In the Bayesian $\chi^2$ reweighting method, PDF replicas that better describe the observed $\mathrm{A_{FB}}$ distribution are assigned larger weights, and PDF replicas that poorly describe the $\mathrm{A_{FB}}$ are assigned smaller weights. Each weight factor is based on the best-fit $\chi^2$-value obtained with a given PDF replica $i$ used in the templates:
\begin{equation} \label{eq:bayesweight}
    w_i = \frac{e^{-\frac{\chi^2_{\text{min}}}{2}}}{\frac{1}{N}\sum_{i=1}^N e^{-\frac{\chi^2_{\text{min}}}{2}}}, 
\end{equation}
where $N$ is the number of replicas in a PDF set. The final result is then calculated as a weighted average over the PDF replicas: $\sineff=\sum_{i=1}^{N} w_i s_i/N$, where $s_i$ is the best-fit \sineff value obtained for $i$-th PDF replica. 


In the case of the 14\UTeV analysis with large number of events ($>200$~\fbinv), the pseudo-data are too precise to estimate the PDF uncertainties with the Bayesian reweighting approach because the replica distributions are too sparse compared to the statistical uncertainties. Therefore, the PDF uncertainties after the Bayesian reweighting is estimated by extrapolating from the lower values of integrated luminosities as illustrated in Fig.~\ref{figure:extrapolation}. The corresponding values for various luminosities are summarized in Table~\ref{table:extrapolation}. One can see from the Table that with the extended pseudorapidity coverage of $|\eta|<2.8$, the statistical uncertainties are reduced by about 30\% and the PDF uncertainties are reduced by about 20\%, compared to $|\eta|<2.4$ regardless of the target integrated luminosity and for both nominal and constrained PDF uncertainties. 

\begin{figure}[!htbp]
\centering
    \includegraphics[scale=0.8]{\main/electroweak/img/ew_precision/extrp.pdf}
    \caption{Projected statistical, nominal PDF and constrained PDF uncertainties in \sineff extracted by fitting 
    $\mathrm{A_{FB}}(m_{\mu\mu},y_{\mu\mu})$ distributions at $\sqrt{s}=14\UTeV$ with different values of integrated luminosities and for $|\eta|<2.4$ and $|\eta|<2.8$ acceptance selections for the muons. The nominal NNPDF3.0 uncertainty is calculated as a standard deviation of the extracted \sineff over the 100 NNPDF3.0 replicas. To calculate the constrained NNPDF3.0 uncertainty, each replica is weighted by $\exp(-\chi^2_{\mathrm{min}}/2)$, where $\chi^2_{\mathrm{min}}$ is the best-fit $\chi^2$ obtained with this replica. \label{figure:extrapolation} }
\end{figure}

\begin{table*}[!htbp]
\centering
\caption{ Statistical, nominal NNPDF3.0, and constrained NNPDF3.0 uncertainties of extracted \sineff at 14\UTeV for muon acceptance of $|\eta|<2.4$ and $|\eta|<2.8$ and for the different values of integrated luminosity. For comparison, results of the 8\UTeV estimate of this analysis are compared to the results obtained from 8 \UTeV measurement~\cite{CMS-PAS-SMP-16-007}. \label{table:extrapolation} }
\begin{tabular}{ | r | c  c | c  c |  c c |} \hline
    $L_{int}$ & \multicolumn{2}{c|}{$\delta_{\mathrm{stat}} [10^{-5}]$} & \multicolumn{2}{c|}{$\delta_{\mathrm{nnpdf3.0}}^{\mathrm{nominal}} [10^{-5}]$} & \multicolumn{2}{c|}{$\delta_{\mathrm{nnpdf3.0}}^{\mathrm{constrained}} [10^{-5}]$} \\ \hline
(\fbinv)  & $|\eta|<2.4$  & $|\eta|<2.8$  &  $|\eta|<2.4$ & $|\eta|<2.8$ & $|\eta|<2.4$ & $|\eta|<2.8$  \\ \hline
  10  & 76  & 51 & 75  & 57 & 39 & 29\\
 100  & 24  & 16 & 75  & 57 & 27 & 20\\
 500  & 11  &  7 & 75  & 57 & 20 & 16\\
1000  &  8  &  5 & 75  & 57 & 18 & 14\\
3000  &  4  &  3 & 75  & 57 & 15 & 12\\ \hline
\hline
19 & 43  &  & 49  &  & 27 & \\
19 (from \cite{CMS-PAS-SMP-16-007}) & 44  &  & 54  &  & 32 & \\
\hline

\end{tabular}
\end{table*}


The precision coverage of the forward region provided by the LHCb experiment, and its planned and proposed upgrades, offers significant advantages in the measurement of the (effective leptonic) weak mixing angle at the HL-LHC. First, in measurements of the forward-backward asymmetry (or associated angular variables) in leptonic decays of \PZ bosons, the assignation of the $z$-axis is crucial. At low rapidities, there is a two-fold ambiguity in the direction of the initial state quark and anti-quark; the colliding quark is equally likely to be in either proton, and the forward-backward asymmetry is significantly diluted. However, at higher rapidities, the $\PZ$ boson tends to be produced in the direction of travel of the quark, since the (valence) quark tends to be at higher Bjorken-$x$ than the anti-quark. This means that the dilution between parton-level and proton-level quantities is significantly smaller in the forward region than in central collisions, and consequently a larger forward-backward asymmetry is induced. In turn, this means that a shift in the weak mixing angle yields a larger shift in the angular distributions of $\PZ$ boson decay, and that PDF effects are (in relative terms) smaller, providing both statistical precision in measurements of the weak mixing angle and a reduction in PDF uncertainties. This reduction in the level of dilution between proton-level and parton-level at forward rapidities is shown in Fig.\ref{fig:s2twlhcb1}.
\begin{figure}[tb]
  \begin{center}
    \includegraphics[width=0.75\linewidth]{\main/electroweak/img/ew_precision/direction}
   
    \vspace*{-0.5cm}
  \end{center}
  \caption{
    %\small %captions should be a little bit smaller than main text
    The fraction of events where the \PZ boson travels in the same direction along the $z$-axis as the colliding quark, in proton-proton collisions with $\sqrt{s} = 14$ TeV. This increases as the event becomes more forward, reaching a maximum in the region probed by LHCb. The decrease once the rapidity is greater than 4 is because the fraction of collisions involving valence quarks decreases (the Bjorken-$x$ value of the high momentum quark in these collisions is typically greater than 0.3). No detector effects are simulated for this figure.
  }
  \label{fig:s2twlhcb1}
\end{figure}
In addition, LHCb does not simply probe forward rapidities of the $Z$ boson: the leptons themselves are located over a significant range of rapidities and transverse momenta.  The leptons themselves can be very forward, allowing extremal values of $\cos\theta^\ast$ values to be probed. Since the sensitivity of an event to the weak mixing angle increases with the values of $|\cos\theta^\ast|$, this favours measurements at LHCb. Finally, LHCb has the ability to select events in its trigger at low momentum; it is foreseen that the LHCb Upgrade II will be able to select in real time $Z$ boson decays where one lepton has transverse momentum above 20~GeV, while the other lepton has a transverse momentum above 5~GeV. Such low thresholds also increase the sensitivity to asymmetric events at high  $|\cos\theta^\ast|$. Finally, the LHCb upgrade II will collect over 300 fb$^{-1}$ of data, allowing high precision measurements.

LHCb has already made one measurement of the weak mixing angle~\cite{Aaij:2015lka}, finding
$\sin^2(\theta_{\text{eff.}}^{lept.}) = 0.23142 \pm 0.00106$ using the LHC Run-1 data. Projections of future performance have also been made~\cite{ViciniTalk}. A study of the sensitivity of the weak mixing angle from future measurements at LHCb has also been performed~\cite{tocome}. For the purpose of this study, the experiment is assumed to have coverage in the region $2.0<\eta<5$ for muons, with momentum resolution and reconstruction efficiency similar to the performance of the current detector~\cite{Aaij:2014jba}. Simulated events were generated using POWHEG with PYTHIA8~\cite{Sjostrand:2006za,Sjostrand:2007gs} for the parton shower, using NNPDF31 PDF sets~\cite{Ball:2017nwa}. Only statistical uncertainties were considered in the study alongside the effects of knowledge of PDFs. Toy measurements of the forward-backward asymmetry were used to determine the sensitivity of measurements at LHCb Upgrade II to the weak mixing angle. The statistical uncertainty on the weak mixing angle is expected to be below $5\times10^{-5}$ with 300~fb$^{-1}$ of data. The expected PDF uncertainty from current PDF knowledge is $\sim 20\times10^{-5}$, but with PDF reweighting techniques this could be reduced to the level of about $10\times10^{-5}$ (with the 300~fb$^{-1}$ dataset). This reduction assumes systematic effects are negligible in comparision to statistical uncertainties, though we note that the current knowledge of PDFs means that any measurement in the forward region is expected to offer a smaller PDF uncertainty than the previous best measurements of the weak mixing angle. A measurement at LHCb Upgrade II - assuming the sufficient control of systematic effects - should yield a precision similar to or better than the current world average. Indeed, the main challenge of such measurements at LHCb Upgrade II will be to control systematic uncertainties, though the large dataset of $J/\psi$ and $\Upsilon$ mesons to be recorded is expected to aid the understanding of effects such as the momentum scale (the main systematic effect in the Run-1 analysis at LHCb).

Finally, we note that additional techniques or improved measurement strategies, for example considering the full angular distribution rather than just the forward-backward asymmetry, and the use of dielectron final states\footnote{The LHCb detector is expected to undergo a significant calorimeter upgrade in the Upgrade II, with an extended dynamic range offering improved electron reconstruction.} as well as dimuon final states, also offer further improvements in the precision achievable at LHCb.




%%%
\subsubsection{EW fits}
%\emph{Authors: J. de Blas, M. Ciuchini, E. Franco, S. Mishima, M. Pierini,
%  L. Reina, and L. Silvestrini}
\newcommand{\HEPfit}{{\tt HEPfit}}
\newcommand{\cmrule}{\midrule[0.25mm]}
\newcommand{\lrD}{~\!\overset{\leftrightarrow}{\hspace{-0.1cm}D}\!}

The measurement of the Higgs Boson mass ($M_H$) at the Large Hadron
Collider (LHC) has provided the last input to the global fit of
electroweak (EW) precision observables (EWPO), which can now be used
to effectively constrain new physics.  Moreover, the measurement of
Higgs-boson production and decay rates that is at the core of the
physics program of the LHC Run 2 will further constrain those
interactions that directly affect Higgs-boson physics.

The high-luminosty LHC (HL-LHC) will have the potential to provide
more constraining bounds on new physics via global fit to EWPO and
Higgs data, thanks to the higher precision it will reach both in the
measurement of some of the crucial input parameters of global EW fits
(e.g. $M_W$, $m_t$, $\sin\theta_{\mathrm{eff}}$), and in the
measurement of Higgs-boson total and differential rates.  In this
study we would like to explore the reach of the HL-LHC in constraining
new physics via a global fit of electroweak precision observables.

In the following we will provide more details on the fitting procedure
and apply it to constrain new physics beyond the SM in the HL-LHC
scenario. More specifically, in Section~\ref{sec:global-fit} we will
describe the parameters and procedure of the global EW fit, while in
Sections~\ref{sec:standard-model} and \ref{sec:new-physics} we will
present results of the SM and new physics fits, respectively.

%%%
\subsubsubsection*{General framework and HEPfit}

\label{sec:global-fit}

The global fit of EWPO is performed using the
\HEPfit~package~\cite{hepfitsite}, a general tool to combine direct
and indirect constraints on the SM and its extensions in any
statistical framework.  The default fit procedure, which we use here,
follows a Bayesian statistical approach and uses BAT (Bayesan Analysis
Toolkit)~\cite{Caldwell:2008fw}. We use flat priors for all input
parameters, and build the likelihood assuming Gaussian distributions
for all experimental measurements. The output of the fit is therefore
given as the posteriors distributions for each input parameters and
observables, calculated using a Markov Chain Monte Carlo method.

Both EW and Higgs observables are calculated as a SM core plus
corrections. The SM core includes all available higher-order
corrections, including the latest theoretical developments in the
calculation of radiative corrections to the EWPO of
\cite{Dubovyk:2016aqv,Dubovyk:2018rlg}.  New-physics corrections are
computed at the leading order.  The \HEPfit~code allows for the
implementation of different models of new physics. In particular, as
explained in Sec.~\ref{sec:new-physics}, we will specialize our study
to the general framework of the so called SM effective field theory
(SMEFT), where the SM Lagrangian is extended by the addition of the
basis of operators of canonical mass dimension higher than four.

As far as EWPO are concerned, this study updates the EWPO fit of
Refs.~\cite{deBlas:2016ojx,deBlas:2016nqo,deBlas:2017wmn} by reducing
the uncertainties on some input parameters that have been obtained by
including hadron collider data, in order to account for the level of
accuracy expected for the HL-LHC. In particular we have assumed that:

\begin{enumerate}
\item{The $W$ mass, whose uncertainty obtained by combining ATLAS and
    Tevatron+LEP2 measurements is currently around
    12~MeV~\cite{deBlas:2017wmn}, will be measured at the HL-LHC with
    a precision of 10~MeV. In this fit we therefore add to the current
    combination an HL-LHC measurement of $M_W=80.379\pm 0.010$~GeV.  A
    naive combination with the current average would result in an
    total uncertainty of $\sim 8$ MeV.}
%
\item{The HL-LHC should also be able to improve the current knowledge
    on the $W$ width, whose precision of 42~MeV is currently given the
    LEP2+Tevatron combination. This uncertainty is dominated by the
    hadron collider measurement. For this fit we will use the
    conservative assumption that the HL-LHC can obtain a measurement
    at least as precise as the previous one, and add an independent
    HL-LHC measurement of $\Gamma_W=2.085\pm 0.042$~GeV. This gives a
    30~MeV uncertainty when combined with the current measurements.}
%
\item{An aggressive estimate of the current uncertainty on the top
    quark mass, obtained by combining current Tevatron and LHC
    measurements, puts the error of $m_t$ at the level of 0.4 GeV.  It
    will be difficult to further reduce this number at the HL-LHC,
    since the remaining uncertainty is mainly of systematic and
    theoretical origin. In the current fit we use
    $m_t=172.8\pm 0.4$~GeV. }
%
\item{The measurements of the effective angle
    $\sin\theta_{\mathrm{eff}}^{\mathrm{lept}}$ can also be improved
    an the HL-LHC.  Currently, a combination of the latest LHC and
    Tevatron results return a precision for this observable of
    $\sim 0.00022-0.00027$, depending on the assumptions made in the
    average regarding common uncertainties.  For the HL-LHC fit, we
    repeat the combination, assuming that statistical uncertainties
    become subdominant. By doing this, we estimate the combined value
    and uncertainty to be used in HL-LHC fits to be:
    $\sin^2\theta_{\mathrm{eff}}^{\mathrm{lept}}= 0.23137 \pm
    0.00018$. }
%
\item{ The error on the Higgs mass, currently around 0.20 GeV, can be reduced to 0.05 GeV~\cite{Dawson:2013bba}. }
\end{enumerate}
%
{\bf [NOTICE: several of the above assumptions are at best educated
  guesses, and some are just random conservative estimates (like
  2). We will need the WG's input to update them.] We could also add
  other observables, like W branching ratios, , if they are available.]}\\
%
Finally, apart from the improved precision of the HL-LHC measurements,
we will assume that, by the end of the HL-LHC run, better measurements
of some of the SM input parameters are possible from other
experiments. Following Ref.~\cite{deBlas:2016ojx,deBlas:2016nqo} we
assume that the uncertainty on
$\Delta \alpha_{\mathrm{had}}^{(5)}(M_Z)$ can be reduced to
$\pm 5 \times 10^{-5}$ using the data from currently ongoing and
future experiments measuring the $e^+ e^-\to$ hadrons cross section,
and that future lattice QCD measurements will provide a determination
of the strong coupling constant with accuracy $\delta \alpha_S(M_Z)=\pm 0.0002$. The
measurements of all other EWPO and input parameters have been kept as
currently available. These as well as the HL-LHC projections are
listed in the second and third columns of Table \ref{tab:SMfit},
respectively.

%%%
\subsubsubsection*{Global Fit: Standard Model fit results}
\label{sec:standard-model}

The result of the SM global fit to EWPO for both the present (LHC) and
future (HL-LHC) scenarios are collected in Table
\ref{tab:SMfit}. These are given in the form of the mean and standard
deviation for each of the observables, as derived from the posterior
of the fits. We also compute the ``pulls'' for the different EWPO, as
the difference between the experimental value and the SM prediction
computed removing each observable from fit (not shown in the table),
normalized to the total uncertainty. As it is apparent, the
differences in the output of the fit are quite small. Still, the
eventual improvement in the precision of $m_t$ would bring a
noticeable decrease on the parametric uncertainty on some observables,
e.g. the $W$ mass, with a total error very close to the intrinsic
uncertainty associated to missing higher-order corrections in the
calculation of $M_W$.  Moreover, the expected improvement on the
experimental precision of $M_W$, without a significant deviation on
the central value, would add some tension between theory and
experiment pushing the pull for this observable beyond the 2$\sigma$
level. The impact of the HL-LHC measurements in the EW fit on the
$M_W$ vs. $m_t$ plane is also illustrated in the left panel of
Figure~\ref{fig:MWmt_ST}.

%
\begin{table}[t]
{\footnotesize
\begin{center}
\begin{tabular}{lccccc}
\toprule
& Measurement & HLLHC &\multicolumn{2}{c}{Posterior} &Pull\\
&  & uncertainty &Current& HL-LHC&Current/HL-LHC\\
\cmrule
$\alpha_{s}(M_Z)$ & $ 0.1180 \pm 0.0010 $ & % Current exp.
$   \pm 0.0002 $  & %Fut. exp
$  0.1180 \pm  0.0009 $ & % Fit current
$  0.1180 \pm  0.0002   $ & % Fit fut
$  $\\ % Pull future
$\Delta\alpha^{(5)}_{\rm had}(M_Z)$ & $ 0.027611 \pm 0.000111 $ & % Current exp.
$   \pm 0.00005 $  & %Fut. exp
$  0.02758 \pm 0.00011$ & % Fit current
$  0.02760 \pm 0.00005  $ & % Fit fut
$  $\\ % Pull future 
$M_Z$ [GeV] & $ 91.1875 \pm 0.0021 $ & % Current exp.
$ $  & %Fut. exp
$ 91.1880  \pm 0.0020  $ & % Fit current
$ 91.1890  \pm 0.0020  $ & % Fit fut
$  $\\ % Pull future
$m_t$ [GeV] & $ 172.8 \pm 0.7 $ & % Current exp.
$  \pm 0.4 $  & %Fut. exp
$  173.2 \pm 0.66  $ & % Fit current
$  173.1 \pm 0.38  $ & % Fit fut
$  $\\ % Pull future
$m_H$ [GeV] & $ 125.13 \pm 0.17 $ & % Current exp.
$   \pm  0.05 $  & %Fut. exp
$ 125.13  \pm 0.17  $ & % Fit current
$ 125.13  \pm 0.05  $ & % Fit fut
$  $\\ % Pull future
\cmrule
$M_W$ [GeV] & $ 80.379 \pm 0.012 $ & % Current exp.
$ \pm 0.008  $  & %Fut. exp
$ 80.362  \pm 0.006   $ & % Fit current
$ 80.364  \pm 0.004   $ & % Fit fut
$ 1.6 / 2.3 $\\ % Pull future
% 
$\Gamma_{W}$ [GeV] & $ 2.085 \pm 0.042 $ & % Current exp.
$   \pm 0.030  $  & %Fut. exp
$ 2.0886  \pm 0.0006  $ & % Fit current
$ 2.0887  \pm 0.0004   $ & % Fit fut
$ -0.1 $\\ % Pull future
%
$\sin^2\theta_{\rm eff}^{\rm lept}(Q_{\rm FB}^{\rm had})$ & $ 0.2324 \pm 0.0012 $ & % Current exp.
$  $  & %Fut. exp
$ 0.23151  \pm 0.00006  $ & % Fit current
$ 0.23151  \pm 0.00005   $ & % Fit fut
$ 0.7 $\\ % Pull future
% 
$P_{\tau}^{\rm pol}={A}_\ell$ & $ 0.1465 \pm 0.0033 $ & % Current exp.
$  $  & %Fut. exp
$ 0.14711  \pm 0.0005  $ & % Fit current
$ 0.14713  \pm 0.0004  $ & % Fit fut
$  -0.2$\\ % Pull future
% 
$\Gamma_{Z}$ [GeV] & $ 2.4952 \pm 0.0023 $ & % Current exp.
$  $  & %Fut. exp
$ 2.4946  \pm 0.0007  $ & % Fit current
$ 2.4946  \pm 0.0005   $ & % Fit fut
$ 0.3 $\\ % Pull future 
$\sigma_{h}^{0}$ [nb] & $ 41.540 \pm 0.037 $ & % Current exp.
$  $  & %Fut. exp
$ 41.492 \pm 0.008  $ & % Fit current
$ 41.492 \pm 0.006   $ & % Fit fut
$  1.3$\\ % Pull future
$R^{0}_{\ell}$ & $ 20.767 \pm 0.025 $ & % Current exp.
$  $  & %Fut. exp
$ 20.749  \pm 0.008  $ & % Fit current
$ 20.749  \pm 0.006   $ & % Fit fut
$ 0.7 $\\ % Pull future
$A_{\rm FB}^{0, \ell}$ & $ 0.0171 \pm 0.0010 $ & % Current exp.
$  $  & %Fut. exp
$ 0.01623  \pm 0.0001  $ & % Fit current
$ 0.016235  \pm 0.00008   $ & % Fit fut
$ 0.9 $\\ % Pull future 
% 
${A}_{\ell}$ (SLD) & $ 0.1513 \pm 0.0021 $ & % Current exp.
$  $  & %Fut. exp
$ 0.14711  \pm 0.0005  $ & % Fit current
$ 0.14713  \pm 0.0004   $ & % Fit fut
$  1.9$\\ % Pull future
$R^{0}_{b}$ & $ 0.21629 \pm 0.00066 $ & % Current exp.
$  $  & %Fut. exp
$ 0.21586  \pm 0.0001  $ & % Fit current
$ 0.21587 \pm 0.0001   $ & % Fit fut
$ 0.7 / 0.6 $\\ % Pull future 
$R^{0}_{c}$ & $ 0.1721 \pm 0.0030 $ & % Current exp.
$  $  & %Fut. exp
$ 0.17221  \pm 0.00005  $ & % Fit current
$ 0.17221  \pm 0.00005   $ & % Fit fut
$ 0 $\\ % Pull future 
$A_{\rm FB}^{0, b}$ & $ 0.0992 \pm 0.0016 $& % Current exp.
$  $  & %Fut. exp
$ 0.10313  \pm 0.00030  $ & % Fit current
$0.10315  \pm 0.00027   $ & % Fit fut
$ -2.4 $\\ % Pull future
$A_{\rm FB}^{0, c}$ & $ 0.0707 \pm 0.0035 $ & % Current exp.
$  $  & %Fut. exp
$ 0.073692  \pm 0.0002  $ & % Fit current
$  0.073702  \pm 0.0002   $ & % Fit fut
$-0.9  $\\ % Pull future
${A}_b$ & $ 0.923 \pm 0.020 $ & % Current exp.
$  $  & %Fut. exp
$ 0.93475  \pm 0.00004 $ & % Fit current
$ 0.93475  \pm 0.00004   $ & % Fit fut
$-0.6  $\\ % Pull future
${A}_c$ & $ 0.670 \pm 0.027 $ & % Current exp.
$  $  & %Fut. exp
$ 0.66792 \pm 0.0002  $ & % Fit current
$ 0.66791 \pm 0.0002   $ & % Fit fut
$ 0.1 $\\ % Pull future
%
$\sin^2\theta_{\rm eff (Had. coll.)}^{\rm lept}$ & $ 0.23137 \pm 0.00027 $ & % Current exp.
$   \pm 0.00018  $  & %Fut. exp
$ 0.23151  \pm 0.00006 $ & % Fit current
$  0.23151  \pm 0.00005 $ & % Fit fut
$-0.5/{-0.8}  $\\ % Pull future
% 
\bottomrule
\end{tabular}
\end{center}
}
\vspace{-0.25cm}
\caption{
  Experimental measurement, HL-LHC projection for the corresponding uncertainty, posterior and pull for the 5 input
  parameters ($\alpha_s(M_Z)$, $\Delta \alpha^{(5)}_{\mathrm{had}}(M_Z)$, $M_Z$,
  $m_t$, $m_H$), and for the main EWPO considered in the SM fit.
  {\bf [HL-LHC results to be updated when final experimental projections are available]}
} 
\label{tab:SMfit}
\end{table}
%


\begin{figure}[h]
\centering
%  \includegraphics[width=.49\textwidth]{Figs/MW_vs_sin2Eff} 
%  \hspace{-3mm}
  \includegraphics[width=.49\textwidth]{\main/electroweak/img/ew_precision/MW_vs_mt} 
  \hspace{-3mm}
   \hspace{-0.1cm}\includegraphics[width=.49\textwidth]{\main/electroweak/img/ew_precision/ST-each}
  \vspace{-0.3cm} 
  \caption{Left) Comparison of the indirect constraints on $M_W$ and
    $m_t$ with the current experimental measurements and the expected
    improvements at the HL-LHC.  Right) Comparison of the currently
    allowed 68\% and 95\% probability regions in the $S$, $T$ fit
    ($U=0$) with the HL-LHC projections. The different bands
    illustrate the bounds from the different EWPO included in the fit.
    {\bf [To be updated when final experimental projections are
      available]}~\label{fig:MWmt_ST}}
\end{figure}


%%%
\subsubsubsection*{Global-Fit: constraints on new physics}
\label{sec:new-physics}

The EWPO, being measured in processes mediated by the exchange of a
$Z$ or $W$ bosons, are extremely sensitive to any new physics that
modifies the propagation of such particles. This results in a
universal modification of the interactions between the electroweak
gauge bosons and the SM fermions, which, from the point of view of
EWPO can be described in terms of only 3 parameters: the well-known
$S$, $T$, and $U$ oblique parameters~\cite{Peskin:1991sw}. The study
of the constraints on the $S$, $T$, and $U$ parameters is one of the
classical benchmarks in the study of electroweak precision constraints
on new physics, and it is well motivated from a theory point of view,
within the context of universal theories. The results of the fit to
the $S$, $T$, and $U$ parameters are given in
Table~\ref{tab:STUfit}. We show the results in terms of the full
($S$,$T$,$U$) fit and also assuming $U=0$, which is motivated in
theories where electroweak symmetry breaking is realized linearly,
since in that case $U\ll S,T$. In both cases the current constraints
are compared with the expected precision at the HL-LHC, which, in some
cases, could improve the sensitivity to such new physics effects by up
to $\sim 20\%$.  The results for the $ST$ fit ($U=0$) are shown
in the right panel of Figure~\ref{fig:MWmt_ST}, illustrating also the
constraints imposed by the different EWPO.

\begin{table}[h]
\begin{center}
\begin{tabular}{c c rrr c }
 \toprule
 & ~~Result & \multicolumn{3}{c}{Correlation Matrix} & Precision at HL-LHC \\ 
 \cmrule
$S$ & $0.04 \pm 0.10 $ & $\phantom{+}1.00$ &&&0.09 \\ 
$T$ & $0.08 \pm 0.12 $ & $\phantom{+}0.90$ & $1.00$&&0.12\\ 
$U$ & $0.00 \pm 0.09 $ & $-0.62$ & $-0.84$ & $1.00$&0.08 \\
\bottomrule
 \toprule
$S$ & $0.04 \pm 0.08 $ & $1.00$ &&&0.06\\ 
$T$ & $0.08 \pm 0.06 $ & $0.90$ & $1.00$ &&0.05\\ 
$(U=0)$ &  &  &  &  \\
\bottomrule
 \end{tabular}
 \end{center}
 \caption{Results of the fit for the oblique parameters $S$, $T$, $U$;
   and $S$, $T$ $(U=0)$. Projections for the uncertainties at the
   HL-LHC are given in the last column. \textbf{[To be updated when final experimental projections are
     available]}\label{tab:STUfit}}
\end{table}


%\begin{figure}[h]
%\centering
%  \hspace{-0.1cm}\includegraphics[width=.45\textwidth]{Figs/ST-each}
%  \vspace{-0.3cm}
%  \caption{ $68\%$ and $95\%$ probability contours for $S$ and $T$
%    $(U=0)$, together with the individual constraints from $M_W$,
%    the asymmetry parameters $\sin^2\theta_{\rm eff}^{\rm lept}$,
%    $P_\tau^{\rm pol}$, $A_f$, and $A_{\rm FB}^{0,f}$ $(f=\ell,c,b)$, 
%    and $\Gamma_Z$. TO BE UPDATED.~\label{fig:ST}}
%\end{figure}

As stressed above, the $STU$ parameterization only describes universal
deformations with respect to the SM predictions.  In order to
systematically explore the impact of global EW precision fits on new
physics, we will adopt in what follows the framework of the Standard
Model effective field theory (SMEFT). In this formalism, the SM
Lagrangian is extended via operators of dimension five and higher,
i.e.  
\begin{equation} 
\label{eq:smeft-lagrangian} 
{\cal L}_{\mathrm{eff}}={\cal
  L}_{\mathrm{SM}}+\sum_{d>4}\frac{1}{\Lambda^{d-4}}{\cal L}_d, 
~~\mbox{with}~~
{\cal L}_d=\sum_i C_i {\cal O}^{(d)}_i,~~\left[{\cal O}^{(d)}_i\right]=d\,, 
\end{equation}
%
where $\Lambda$ denotes the cut-off scale of the SMEFT.  This new
physics scale introduces a first hierarchical ordering between
contributions of operators of lower versus higher dimension, where
higher-dimension operators are suppressed by inverse powers of
$\Lambda$. Each term in ${\cal L}_d$ is a linear combination of
$d$-dimensional operators $O_i^{(d)}$ built in terms of SM fields,
with coefficients $C_i$ that can depend on both SM masses and
couplings, as well as new physics parameters.  For the analysis of
EWPO the leading new physics corrections come from dimension-six
operators (${\cal L}_6$). We will limit our study to this order in the
EFT expansion.  Using the complete basis of dimension-six interactions
presented in Ref. \cite{Grzadkowski:2010es}, the $Z$-pole and $W$
observables in Table~\ref{tab:SMfit} are corrected at the leading
order by 10 different types of operators. The bosonic operators
%
$${\cal O}_{\phi D}=\left|\phi^\dagger D^\mu \phi\right|^2\mbox{ and }{\cal O}_{\phi WB}=\left(\phi^\dagger \sigma_a \phi\right) W_{\mu\nu}^a B^{\mu\nu},$$
%
modify the gauge-boson propagators in a  way similar to  the $T$ and $S$ parameters, respectively.
The interactions
%
$${\cal O}_{\phi \psi}^{(1)}=\left(\phi^\dagger \lrD^\mu \phi\right) \left(\overline{\psi}\gamma_\mu \psi\right)\mbox{ and }{\cal O}_{\phi F}^{(3)}=\left(\phi^\dagger \sigma_a \lrD^\mu \phi\right) \left(\overline{F}\gamma_\mu \sigma_a F\right),$$
%
where $\psi=l,~e,~q,~u~,d$ denotes the SM fermion multiplets, and $F=l,~q$, the left-handed fermion doublets,
correct, upon electroweak symmetry breaking, the EW couplings of the $Z$ and $W$ bosons to the fermions.
Finally, the four-lepton operator 
%
$${\cal O}_{ll}=\left(\overline{l}\gamma_\mu l\right) \left(\overline{l}\gamma^\mu l\right)$$
%
modifies the muon decay amplitude, and therefore affects the extraction of the Fermi constant, one of the inputs
used in the SM. This effect propagates into the different observables considered in the electroweak sector.

The aim of a global fit to EWPO data is to constrain the corresponding
$C_i$ coefficients. The results of the fit to EWPO using the projected
HL-LHC data are shown in Figure ~\ref{fig:dim6}. In that figure we
show the bounds on the eight possible combinations of operators that
can be constrained using EW precision data in the case of flavor
universal couplings. This means that in the basis of
\cite{Grzadkowski:2010es} there are two flat directions which, for
simplicity, we lift by performing a field redefinition to exchange
$C_{\phi D}$ and $C_{\phi WB}$ by two interactions that do not enter
in EWPO. Compared to current numbers, the HL-LHC could improve the
global bounds on some of the leptonic coefficients by up to a 10-30\%,
although for most coefficients the effect os much milder, see
Table~\ref{tab:dim6fit}. In that table we also compare the bound
obtained assuming only operator is present in the fit at a time,
showing improvements of the same order of magnitude. \textbf{[To be
  updated when final experimental projections are available]}

\begin{figure}[t]
\centering
  \hspace{-0.1cm}\includegraphics[width=.8\textwidth]{\main/electroweak/img/ew_precision/Globalfit_dim6}
  \vspace{-0.3cm}
  \caption{$68\%$ and $95\%$ probability limits on the dimension-six operator coefficients $c_i/\Lambda^2$ [TeV$^{-2}$] from the global fit to EWPO at HLLHC including all operators (in blue), compared with the limits obtained assuming only one operator at a time (in red). See Table~\ref{tab:dim6fit} for the comparison with current uncertainties. {\bf [To be updated when final experimental projections are available]}~\label{fig:dim6}}
\end{figure}

\begin{table}[h]
\begin{center}
\begin{tabular}{l c c c c }
 \toprule
               & \multicolumn{2}{c}{Current uncertainty} & \multicolumn{2}{c}{Precision at HL-LHC} \\ 
               & \multicolumn{2}{c}{[TeV$^{-2}$]} & \multicolumn{2}{c}{ [TeV$^{-2}$]} \\ 
 Operator& 1 op. at& Global & 1 op. at  & Global  \\ 
 		&a time &fit  &a time & fit  \\ 
 \cmrule
~~~$\overline{C}_{\phi l}^{(1)}$ & 
$0.004 $ & %C-1op
$0.012 $ & %C-Glob
$0.004 $ & %HLLHC-1op
$0.012$  \\ %HLLHC-Glob
%
~~~$\overline{C}_{\phi q}^{(1)}$ & 
$0.018 $ & %C-1op
$0.044 $ & %C-Glob
$0.017 $ & %HLLHC-1op
$0.044 $  \\ %HLLHC-Glob
%
~~~$\overline{C}_{\phi e}$ & 
$0.006 $ & %C-1op
$0.010 $ & %C-Glob
$0.005 $ & %HLLHC-1op
$0.007 $  \\ %HLLHC-Glob
%
~~~$\overline{C}_{\phi u}$ & 
$0.039 $ & %C-1op
$0.146 $ & %C-Glob
$0.038 $ & %HLLHC-1op
$0.145 $  \\ %HLLHC-Glob
%
~~~$\overline{C}_{\phi d}$ & 
$0.054 $ & %C-1op
$0.243 $ & %C-Glob
$0.051 $ & %HLLHC-1op
$0.242$  \\ %HLLHC-Glob 
%
~~~$\overline{C}_{\phi l}^{(3)}$ & 
$0.004 $ & %C-1op
$0.017 $ & %C-Glob
$0.003 $ & %HLLHC-1op
$0.015 $  \\ %HLLHC-Glob
%
~~~$\overline{C}_{\phi q}^{(3)}$ & 
$0.007 $ & %C-1op
$0.040$ & %C-Glob
$0.006 $ & %HLLHC-1op
$0.038$  \\ %HLLHC-Glob
%
~~~$\overline{C}_{ll}$ & 
$0.007 $ & %C-1op
$0.028 $ & %C-Glob
$0.005 $ & %HLLHC-1op
$0.028 $  \\ %HLLHC-Glob
%
\cmrule
~~~$\overline{C}_{\phi WB}$ & 
$0.003 $ & %C-1op
$-$ & %C-Glob
$0.002 $ & %HLLHC-1op
$-$  \\ %HLLHC-Glob
%
~~~$\overline{C}_{\phi D}$ &
$0.007 $ & %C-1op
$-$ & %C-Glob
$0.005 $ & %HLLHC-1op
$-$  \\ %HLLHC-Glob 
\bottomrule
 \end{tabular}
 \end{center}
 \caption{Results of the fit to the coefficients of the SMEFT
   dimension-six Lagrangian. The uncertainties shown refer to the fit
   performed assuming the presence of only one effective operator at a
   time and to the case when all (eight) operators are active at the
   same time (global fit). Projections for the uncertainties at the HL-LHC are given in the last two columns. Result shown for the ratios $\overline{C}_i \equiv C_i/\Lambda^2$.
   {\bf [HL-LHC results to be updated when final experimental projections are available]}
   \label{tab:dim6fit}}
\end{table}




%\bibliographystyle{utphys}
%\bibliography{ww_hl}



%\end{document} 


==> electroweak/tribosons/tribosons_marek_removed.tex <==
\newcommand{\Sherpa}{S\protect\scalebox{0.8}{HERPA}\xspace}
\newcommand{\Recola}{R\protect\scalebox{0.8}{ECOLA}\xspace}
\newcommand{\shortequal}{\!\!=\!\!}
%AT \newcommand{\hl}{\vphantom{$\int_A^B$}}
%AT \newcommand{\pT}{\ensuremath{p_\mathrm{T}}}
\newcommand{\pTmis}{\ensuremath{\displaystyle{\not}\pT}}

%opening
\subsubsection{Cross-section for off-shell WWW production including NLO electroweak corrections}

%AT \author{Marek Sch\"onherr}
%AT \date{}

%\begin{document}
%\maketitle

%%%%%%%%%%%%%%%

TO BE UPDATED

%%%%%%%%%
\subsubsubsection*{Introduction}
\label{sec:offshell-WWW-intro}

Triboson production processes allow for a measurement of triple and 
quartic couplings of the Standard Model gauge bosons, which can be 
used to constain anomalous gauge couplings that frquently appear 
in BSM theories \cite{Aaboud:2016ftt}. 
In this section we calculate the production yields to fully 
off-shell $W^-W^+W^+$ production, ie.\ a 
$\ell_1^-\ell_2^+\ell_3^+\bar\nu_{\ell_4}\nu_{\ell_5}\nu_{\ell_6}$ 
final state with $\ell_i=e,\mu$, including all triple, double and 
single resonant topologies and interferences of diagrams with 
different vector boson ($W$, $Z$, $\gamma$) intermediate states. 

This calculation makes use of the automated tools 
\Sherpa \cite{Gleisberg:2008ta,Bothmann:2016nao,Schonherr:2017qcj} 
and \Recola \cite{Actis:2012qn,Actis:2016mpe}. 
While \Sherpa provides the tree-level matrix elements, infrared 
subtraction, process management and phase-space integration 
of all contributions to all processes, \Recola 
provides the renormalised virtual corrections. 
It follows the parameters of the original publication \cite{Schonherr:2018}

In the following, the production yields for the High Luminosity 
and the proposed High Energy upgrade of the LHC are presented 
in Sections \ref{sec:offshell-WWW-HL} and \ref{sec:offshell-WWW-HE}, 
respectively. 
For both collider setups we use the \texttt{NNPDF31\_nlo\_as\_0118\_luxqed} 
PDF \cite{Bertone:2017bme} containing QED effects calculated in the 
LUXqed scheme \cite{Manohar:2016nzj,Manohar:2017eqh}. 
The calculation is performed in the Standard Model using the 
complex mass scheme, defining the electroweak parameters in the 
$G_\mu$-scheme with the following input parameters
\begin{center}
  \begin{tabular}{rclrcl}
    $G_\mu$ &\shortequal& $1.16637\times 10^{-5}\; \text{GeV}^2$ &&& \\
    $m_W$ &\shortequal& $80.385\; \text{GeV}$       & $\Gamma_W$ &\shortequal& $2.0897\; \text{GeV}$ \\
    $m_Z$ &\shortequal& $91.1876\; \text{GeV}$      & $\Gamma_Z$ &\shortequal& $2.4955\; \text{GeV}$ \\
    $m_h$ &\shortequal& $125.0\; \text{GeV}$        & $\Gamma_h$ &\shortequal& $0.00407\; \text{GeV}$\\
    $m_t$ &\shortequal& $173.2\; \text{GeV}$        & $\Gamma_t$ &\shortequal& $1.3394$\; \text{GeV}\;.
  \end{tabular}
\end{center}
We choose $\mu_R=\mu_F=3\,m_W$ and a diagonal CKM matrix.
The lepton acceptance cuts specifying the fiducial region are listed in 
Table \ref{tab:offshell-WWW-cuts}. 
They are applied on dressed leptons, defined through recombining the 
bare lepton four-momenta with all photons in a cone of 
$\Delta R_\text{dress}=0.1$ around it. 
At most one jet is allowed to be present, which, however, does not 
affect the present next-to-leading order calculation.


\begin{table}[t]
  \centering
   \caption{
    Definition of the fiducial region. 
    All selection cuts are applied to dressed leptons, defined with 
    $\Delta R_\text{dress}=0.1$.}
    \label{tab:offshell-WWW-cuts}
  \begin{tabular}{|l|lc|}
  \hline
    Selection & Cut & Value \\
    \hline\hline
    General
    \hl  & $\pT(\ell)$ & $[30\,\text{GeV},\infty)$ \\
    \hl  & $y(\ell)$ & $[-4.0,4.0]$ \\
    \hl  & $\Delta R(\ell,\ell)$ & $[0.2,\infty)$ \\\hline
    1, 2 SFOS
    \hl  & $\pTmis$ & $[50\,\text{GeV},\infty)$ \\
    \hl  & $m_{\ell\ell}^\text{SFOS}$ & $[0,70\,\text{GeV}]\wedge[100\,\text{GeV},\infty)$\\
\hline 
 \end{tabular}
\end{table}

%%%
\subsubsubsection*{Cross sections for 14\,TeV}
\label{sec:offshell-WWW-HL}

In this section the integrated production yields for $W^-W^+W^+$ 
production are presented for the High Luminosity upgrade of the 
LHC at a centre-of-mass energy of 14\,TeV and an integrated 
luminostiy of 300\,fb$^{-1}$.

\textit{About 2/3 pages figures and short description.}

\begin{figure}
  %AT \includegraphics[width=0.47\textwidth]{plots/}
  \hfill
  %AT \includegraphics[width=0.47\textwidth]{plots/}
  \caption{
    Event yields at the High Luminosity LHC at 14\,TeV with 300\,fb$^{-1}$ 
    depending on a minimum transverse mass (left) or a minimum missing 
    transverse momentum (right). }
\end{figure}

%%%
\subsubsubsection*{Cross sections for 27\,TeV}
\label{sec:offshell-WWW-HE}

In this section the integrated production yields for $W^-W^+W^+$ 
production are presented for the High Luminosity upgrade of the 
LHC at a centre-of-mass energy of 27\,TeV and an integrated 
luminosity of 15\,ab$^{-1}$.

\textit{About 2/3 pages figures and short description.}

\begin{figure}
  %AT \includegraphics[width=0.47\textwidth]{plots/}
  \hfill
  %AT \includegraphics[width=0.47\textwidth]{plots/}
  \caption{
    Event yields at the High Energy LHC at 27\,TeV with 15\,ab$^{-1}$ 
    depending on a minimum transverse mass (left) or a minimum missing 
    transverse momentum (right).}
\end{figure}

%%%
\subsubsubsection*{Conclusions}
\label{sec:offshell-WWW-conclusions}

\textit{About 1/3 pages short summary.}

%\end{document}


==> pdefs.tex <==
\symexamp{etal}{\etal}
\symexamp{ie}{\ie}
\symexamp{eg}{\eg}
\symexamp{etc}{\etc}
\symexamp{vs}{\vs}
\symexamp{mdash}{\mdash}
\symexamp{Lone}{\Lone}
\symexamp{Ltwo}{\Ltwo}
\symexamp{Lthree}{\Lthree}
\symexamp{ACERMC}{\ACERMC}
\symexamp{ALPGEN}{\ALPGEN}
\symexamp{CHARYBDIS}{\CHARYBDIS}
\symexamp{CMKIN}{\CMKIN}
\symexamp{CMSIM}{\CMSIM}
\symexamp{CMSSW}{\CMSSW}
\symexamp{COBRA}{\COBRA}
\symexamp{COCOA}{\COCOA}
\symexamp{COMPHEP}{\COMPHEP}
\symexamp{EVTGEN}{\EVTGEN}
\symexamp{FAMOS}{\FAMOS}
\symexamp{GARCON}{\GARCON}
\symexamp{GARFIELD}{\GARFIELD}
\symexamp{GEANE}{\GEANE}
\symexamp{GEANTfour}{\GEANTfour}
\symexamp{GEANTthree}{\GEANTthree}
\symexamp{GEANT}{\GEANT}
\symexamp{HDECAY}{\HDECAY}
\symexamp{HERWIG}{\HERWIG}
\symexamp{HIGLU}{\HIGLU}
\symexamp{HIJING}{\HIJING}
\symexamp{IGUANA}{\IGUANA}
\symexamp{ISAJET}{\ISAJET}
\symexamp{ISAPYTHIA}{\ISAPYTHIA}
\symexamp{ISASUGRA}{\ISASUGRA}
\symexamp{ISASUSY}{\ISASUSY}
\symexamp{ISAWIG}{\ISAWIG}
\symexamp{MADGRAPH}{\MADGRAPH}
\symexamp{MCATNLO}{\MCATNLO}
\symexamp{MCFM}{\MCFM}
\symexamp{MILLEPEDE}{\MILLEPEDE}
\symexamp{ORCA}{\ORCA}
\symexamp{OSCAR}{\OSCAR}
\symexamp{PHOTOS}{\PHOTOS}
\symexamp{PROSPINO}{\PROSPINO}
\symexamp{PYTHIA}{\PYTHIA}
\symexamp{SHERPA}{\SHERPA}
\symexamp{TAUOLA}{\TAUOLA}
\symexamp{TOPREX}{\TOPREX}
\symexamp{XDAQ}{\XDAQ}
\symexamp{DZERO}{\DZERO}
\symexamp{de}{\de}
\symexamp{ten\{x\}}{\ten{x}}
\symexamp{unit\{x\}}{\unit{x}}
\symexamp{mum}{\mum}
\symexamp{micron}{\micron}
\symexamp{cm}{\cm}
\symexamp{mm}{\mm}
\symexamp{mus}{\mus}
\symexamp{keV}{\keV}
\symexamp{MeV}{\MeV}
\symexamp{GeV}{\GeV}
\symexamp{gev}{\gev}
\symexamp{TeV}{\TeV}
\symexamp{PeV}{\PeV}
\symexamp{keVc}{\keVc}
\symexamp{MeVc}{\MeVc}
\symexamp{GeVc}{\GeVc}
\symexamp{TeVc}{\TeVc}
\symexamp{keVcc}{\keVcc}
\symexamp{MeVcc}{\MeVcc}
\symexamp{GeVcc}{\GeVcc}
\symexamp{TeVcc}{\TeVcc}
\symexamp{pbinv}{\pbinv}
\symexamp{fbinv}{\fbinv}
\symexamp{nbinv}{\nbinv}
\symexamp{percms}{\percms}
\symexamp{lumi}{\lumi}
\symexamp{Lumi}{\Lumi}
\symexamp{LvLow}{\LvLow}
\symexamp{LLow}{\LLow}
\symexamp{lowlumi}{\lowlumi}
\symexamp{LMed}{\LMed}
\symexamp{LHigh}{\LHigh}
\symexamp{hilumi}{\hilumi}
\symexamp{PT}{\PT}
\symexamp{pt}{\pt}
\symexamp{ET}{\ET}
\symexamp{HT}{\HT}
\symexamp{et}{\et}
\symexamp{Em}{\Em}
\symexamp{Pm}{\Pm}
\symexamp{PTm}{\PTm}
\symexamp{PTslash}{\PTslash}
\symexamp{ETm}{\ETm}
\symexamp{MET}{\MET}
\symexamp{ETmiss}{\ETmiss}
\symexamp{ETslash}{\ETslash}
\symexamp{VEtmiss}{\VEtmiss}
\symexamp{dd\{y\}\{x\}}{\dd{y}{x}}
\symexamp{ddinline\{y\}\{x\}}{\ddinline{y}{x}}
\symexamp{abs\{x\}}{\abs{x}}
\symexamp{zp}{\zp}
\symexamp{JPsi}{\JPsi}
\symexamp{Z}{\Z}
\symexamp{ttbar}{\ttbar}
\symexamp{cPgn}{\cPgn}
\symexamp{cPagn}{\cPagn}
\symexamp{cPgg}{\cPgg}
\symexamp{cPJgy}{\cPJgy}
\symexamp{cPZ}{\cPZ}
\symexamp{cPZpr}{\cPZpr}
\symexamp{cPqt}{\cPqt}
\symexamp{cPqb}{\cPqb}
\symexamp{cPqc}{\cPqc}
\symexamp{cPqs}{\cPqs}
\symexamp{cPqu}{\cPqu}
\symexamp{cPqd}{\cPqd}
\symexamp{cPq}{\cPq}
\symexamp{cPg}{\cPg}
\symexamp{cPG}{\cPG}
\symexamp{cPaqt}{\cPaqt}
\symexamp{cPaqb}{\cPaqb}
\symexamp{cPaqc}{\cPaqc}
\symexamp{cPaqs}{\cPaqs}
\symexamp{cPaqu}{\cPaqu}
\symexamp{cPaqd}{\cPaqd}
\symexamp{cPaq}{\cPaq}
\symexamp{PH}{\PH}
\symexamp{PJGy}{\PJGy}
\symexamp{PBzs}{\PBzs}
\symexamp{Pg}{\Pg}
\symexamp{PSg}{\PSg}
\symexamp{PSq}{\PSq}
\symexamp{AFB}{\AFB}
\symexamp{wangle}{\wangle}
\symexamp{stat}{\stat}
\symexamp{syst}{\syst}
\symexamp{kt}{\kt}
\symexamp{BC}{\BC}
\symexamp{bbarc}{\bbarc}
\symexamp{bbbar}{\bbbar}
\symexamp{ccbar}{\ccbar}
\symexamp{bspsiphi}{\bspsiphi}
\symexamp{EE}{\EE}
\symexamp{MM}{\MM}
\symexamp{TT}{\TT}
\symexamp{HGG}{\HGG}
\symexamp{GAMJET}{\GAMJET}
\symexamp{PPTOJETS}{\PPTOJETS}
\symexamp{PPTOGG}{\PPTOGG}
\symexamp{PPTOGAMJET}{\PPTOGAMJET}
\symexamp{MH}{\MH}
\symexamp{RNINE}{\RNINE}
\symexamp{DR}{\DR}
\symexamp{ga}{\ga}
\symexamp{la}{\la}
\symexamp{swsq}{\swsq}
\symexamp{cwsq}{\cwsq}
\symexamp{tanb}{\tanb}
\symexamp{tanbsq}{\tanbsq}
\symexamp{sidb}{\sidb}
\symexamp{alpS}{\alpS}
\symexamp{alpt}{\alpt}
\symexamp{QL}{\QL}
\symexamp{sQ}{\sQ}
\symexamp{sQL}{\sQL}
\symexamp{ULC}{\ULC}
\symexamp{sUC}{\sUC}
\symexamp{sULC}{\sULC}
\symexamp{DLC}{\DLC}
\symexamp{sDC}{\sDC}
\symexamp{sDLC}{\sDLC}
\symexamp{LL}{\LL}
\symexamp{sL}{\sL}
\symexamp{sLL}{\sLL}
\symexamp{ELC}{\ELC}
\symexamp{sEC}{\sEC}
\symexamp{sELC}{\sELC}
\symexamp{sEL}{\sEL}
\symexamp{sER}{\sER}
\symexamp{sFer}{\sFer}
\symexamp{sQua}{\sQua}
\symexamp{sUp}{\sUp}
\symexamp{suL}{\suL}
\symexamp{suR}{\suR}
\symexamp{sDw}{\sDw}
\symexamp{sdL}{\sdL}
\symexamp{sdR}{\sdR}
\symexamp{sTop}{\sTop}
\symexamp{stL}{\stL}
\symexamp{stR}{\stR}
\symexamp{stone}{\stone}
\symexamp{sttwo}{\sttwo}
\symexamp{sBot}{\sBot}
\symexamp{sbL}{\sbL}
\symexamp{sbR}{\sbR}
\symexamp{sbone}{\sbone}
\symexamp{sbtwo}{\sbtwo}
\symexamp{sLep}{\sLep}
\symexamp{sLepC}{\sLepC}
\symexamp{sEl}{\sEl}
\symexamp{sElC}{\sElC}
\symexamp{seL}{\seL}
\symexamp{seR}{\seR}
\symexamp{snL}{\snL}
\symexamp{sMu}{\sMu}
\symexamp{sNu}{\sNu}
\symexamp{sTau}{\sTau}
\symexamp{Glu}{\Glu}
\symexamp{sGlu}{\sGlu}
\symexamp{Wpm}{\Wpm}
\symexamp{sWpm}{\sWpm}
\symexamp{Wz}{\Wz}
\symexamp{sWz}{\sWz}
\symexamp{sWino}{\sWino}
\symexamp{Bz}{\Bz}
\symexamp{sBz}{\sBz}
\symexamp{sBino}{\sBino}
\symexamp{Zz}{\Zz}
\symexamp{sZino}{\sZino}
\symexamp{sGam}{\sGam}
\symexamp{chiz}{\chiz}
\symexamp{chip}{\chip}
\symexamp{chim}{\chim}
\symexamp{chipm}{\chipm}
\symexamp{Hone}{\Hone}
\symexamp{sHone}{\sHone}
\symexamp{Htwo}{\Htwo}
\symexamp{sHtwo}{\sHtwo}
\symexamp{sHig}{\sHig}
\symexamp{sHa}{\sHa}
\symexamp{sHb}{\sHb}
\symexamp{sHpm}{\sHpm}
\symexamp{hz}{\hz}
\symexamp{Hz}{\Hz}
\symexamp{Az}{\Az}
\symexamp{Hpm}{\Hpm}
\symexamp{sGra}{\sGra}
\symexamp{mtil}{\mtil}
\symexamp{rpv}{\rpv}
\symexamp{LLE}{\LLE}
\symexamp{LQD}{\LQD}
\symexamp{UDD}{\UDD}
\symexamp{Lam}{\Lam}
\symexamp{Lamp}{\Lamp}
\symexamp{Lampp}{\Lampp}
\symexamp{MD}{\MD}
\symexamp{Mpl}{\Mpl}
\symexamp{Rinv}{\Rinv}


==> qcd/pdefs.tex <==
\symexamp{etal}{\etal}
\symexamp{ie}{\ie}
\symexamp{eg}{\eg}
\symexamp{etc}{\etc}
\symexamp{vs}{\vs}
\symexamp{mdash}{\mdash}
\symexamp{Lone}{\Lone}
\symexamp{Ltwo}{\Ltwo}
\symexamp{Lthree}{\Lthree}
\symexamp{ACERMC}{\ACERMC}
\symexamp{ALPGEN}{\ALPGEN}
\symexamp{CALCHEP}{\CALCHEP}
\symexamp{CHARYBDIS}{\CHARYBDIS}
\symexamp{CMKIN}{\CMKIN}
\symexamp{CMSIM}{\CMSIM}
\symexamp{CMSSW}{\CMSSW}
\symexamp{COBRA}{\COBRA}
\symexamp{COCOA}{\COCOA}
\symexamp{COMPHEP}{\COMPHEP}
\symexamp{EVTGEN}{\EVTGEN}
\symexamp{FAMOS}{\FAMOS}
\symexamp{FEWZ}{\FEWZ}
\symexamp{GARCON}{\GARCON}
\symexamp{GARFIELD}{\GARFIELD}
\symexamp{GEANE}{\GEANE}
\symexamp{GEANTfour}{\GEANTfour}
\symexamp{GEANTthree}{\GEANTthree}
\symexamp{GEANT}{\GEANT}
\symexamp{HDECAY}{\HDECAY}
\symexamp{HERWIG}{\HERWIG}
\symexamp{HERWIGpp}{\HERWIGpp}
\symexamp{POWHEG}{\POWHEG}
\symexamp{HIGLU}{\HIGLU}
\symexamp{HIJING}{\HIJING}
\symexamp{IGUANA}{\IGUANA}
\symexamp{ISAJET}{\ISAJET}
\symexamp{ISAPYTHIA}{\ISAPYTHIA}
\symexamp{ISASUGRA}{\ISASUGRA}
\symexamp{ISASUSY}{\ISASUSY}
\symexamp{ISAWIG}{\ISAWIG}
\symexamp{MADGRAPH}{\MADGRAPH}
\symexamp{MCATNLO}{\MCATNLO}
\symexamp{MCFM}{\MCFM}
\symexamp{MILLEPEDE}{\MILLEPEDE}
\symexamp{ORCA}{\ORCA}
\symexamp{OSCAR}{\OSCAR}
\symexamp{PHOTOS}{\PHOTOS}
\symexamp{PROSPINO}{\PROSPINO}
\symexamp{PYTHIA}{\PYTHIA}
\symexamp{SHERPA}{\SHERPA}
\symexamp{TAUOLA}{\TAUOLA}
\symexamp{TOPREX}{\TOPREX}
\symexamp{XDAQ}{\XDAQ}
\symexamp{DZERO}{\DZERO}
\symexamp{de}{\de}
\symexamp{ten\{x\}}{\ten{x}}
\symexamp{unit\{x\}}{\unit{x}}
\symexamp{mum}{\mum {\tiny[Most units include leading thinspace]}}
\symexamp{micron}{\micron}
\symexamp{cm}{\cm}
\symexamp{mm}{\mm}
\symexamp{mus}{\mus}
\symexamp{keV}{\keV}
\symexamp{MeV}{\MeV}
\symexamp{MeVns}{\MeVns\hspace{\fill}{\tiny[\textit{no} leading thinspace with \textit{ns} suffix]}}
\symexamp{GeV}{\GeV}
\symexamp{GeVns}{\GeVns}
\symexamp{gev}{\gev}
\symexamp{TeV}{\TeV}
\symexamp{TeVns}{\TeVns}
\symexamp{PeV}{\PeV}
\symexamp{keVc}{\keVc}
\symexamp{MeVc}{\MeVc}
\symexamp{GeVc}{\GeVc}
\symexamp{GeVcns}{\GeVcns}
\symexamp{TeVc}{\TeVc}
\symexamp{keVcc}{\keVcc}
\symexamp{MeVcc}{\MeVcc}
\symexamp{GeVcc}{\GeVcc}
\symexamp{GeVccns}{\GeVccns}
\symexamp{TeVcc}{\TeVcc}
\symexamp{pbinv}{\pbinv}
\symexamp{fbinv}{\fbinv}
\symexamp{nbinv}{\nbinv}
\symexamp{mubinv}{\mubinv}
\symexamp{percms}{\percms}
\symexamp{lumi}{\lumi}
\symexamp{Lumi}{\Lumi}
\symexamp{LvLow}{\LvLow}
\symexamp{LLow}{\LLow}
\symexamp{lowlumi}{\lowlumi}
\symexamp{LMed}{\LMed}
\symexamp{LHigh}{\LHigh}
\symexamp{hilumi}{\hilumi}
\symexamp{PT}{\PT}
\symexamp{pt}{\pt}
\symexamp{ET}{\ET}
\symexamp{HT}{\HT}
\symexamp{et}{\et}
\symexamp{Em}{\Em}
\symexamp{Pm}{\Pm}
\symexamp{PTm}{\PTm}
\symexamp{PTslash}{\PTslash}
\symexamp{ETm}{\ETm}
\symexamp{MET}{\MET}
\symexamp{ETmiss}{\ETmiss}
\symexamp{ETslash}{\ETslash}
\symexamp{VEtmiss}{\VEtmiss}
\symexamp{ptvec}{\ptvec}
\symexamp{ptvecmiss}{\ptvecmiss}
\symexamp{dd\{y\}\{x\}}{\dd{y}{x}}
\symexamp{ddinline\{y\}\{x\}}{\ddinline{y}{x}}
\symexamp{rd}{\rd}
\symexamp{re}{\re}
\symexamp{abs\{x\}}{\abs{x}}
\symexamp{zp}{\zp}
\symexamp{JPsi}{\JPsi}
\symexamp{Z}{\Z}
\symexamp{ttbar}{\ttbar}
\noindent%
\textcolor{gray}{\rule{\columnwidth}{0.2pt}}
\noindent%
Extensions to PENNAMES\\
\symexamp{cPgn}{\cPgn}
\symexamp{Pgn}{\Pgn}
\symexamp{cPagn}{\cPagn}
\symexamp{Pagn}{\Pagn}
\symexamp{cPgg}{\cPgg}
\symexamp{cPJgy}{\cPJgy}
\symexamp{cPZ}{\cPZ}
\symexamp{cPZpr}{\cPZpr}
\symexamp{cPqt}{\cPqt}
\symexamp{cPqb}{\cPqb}
\symexamp{cPqc}{\cPqc}
\symexamp{cPqs}{\cPqs}
\symexamp{cPqu}{\cPqu}
\symexamp{cPqd}{\cPqd}
\symexamp{cPq}{\cPq}
\symexamp{cPg}{\cPg}
\symexamp{cPG}{\cPG}
\symexamp{cPaqt}{\cPaqt}
\symexamp{cPaqb}{\cPaqb}
\symexamp{cPaqc}{\cPaqc}
\symexamp{cPaqs}{\cPaqs}
\symexamp{cPaqu}{\cPaqu}
\symexamp{cPaqd}{\cPaqd}
\symexamp{cPaq}{\cPaq}
\symexamp{cPKstz}{\cPKstz}
\noindent%
\textcolor{gray}{\rule{\columnwidth}{0.2pt}}
\noindent%
Future PENNAMES2\hspace{\fill}{\tiny{include \verb|\xspace|}}\\
\symexamp{PH}{\PH}
\symexamp{Ph}{\Ph}
\symexamp{PJGy}{\PJGy}
\symexamp{PBzs}{\PBzs}
\symexamp{Pg}{\Pg}
\symexamp{PSg}{\PSg}
\symexamp{PSQ}{\PSQ}
\symexamp{PXXG}{\PXXG}
\symexamp{PXXSG}{\PXXSG}
\symexamp{PSGcp}{\PSGcp}
\symexamp{PSGc}{\PSGc}
\symexamp{PSGcz}{\PSGcz}
\symexamp{PSGczDo}{\PSGczDo}
\symexamp{PSGczDt}{\PSGczDt}
\symexamp{PSGcpm}{\PSGcpm}
\symexamp{PSGcpDo}{\PSGcpDo}
\symexamp{Pl}{\Pl}
\symexamp{PAl}{\PAl}
\symexamp{PGnl}{\PGnl}
\symexamp{PAGnl}{\PAGnl}
\symexamp{PQtpr}{\PQtpr}
\symexamp{PAQtpr}{\PAQtpr}
\symexamp{PQbpr}{\PQbpr}
\symexamp{PAQbpr}{\PAQbpr}
\symexamp{PGg}{\PGg}
\symexamp{PKzS}{\PKzS}
\symexamp{PBs}{\PBs}
\symexamp{PSQu}{\PSQu}
\symexamp{PSQd}{\PSQd}
\symexamp{PSQc}{\PSQc}
\symexamp{PSQs}{\PSQs}
\symexamp{PSQt}{\PSQt}
\symexamp{PSQb}{\PSQb}
\symexamp{PASQt}{\PASQt}
\symexamp{PASQb}{\PASQb}
\symexamp{PSGt}{\PSGt}
\symexamp{PZpr}{\PZpr}
\symexamp{PGn}{\PGn}
\symexamp{PAGn}{\PAGn}
\symexamp{PSQtDo}{\PSQtDo}
\symexamp{PSQtDt}{\PSQtDt}
\symexamp{PQt}{\PQt}
\symexamp{PAQt}{\PAQt}
\symexamp{PQb}{\PQb}
\symexamp{PAQb}{\PAQb}
\symexamp{PGm}{\PGm}
\symexamp{PGt}{\PGt}
\symexamp{PQq}{\PQq}
\symexamp{PQd}{\PQd}
\symexamp{PQu}{\PQu}
\symexamp{PQs}{\PQs}
\symexamp{PQc}{\PQc}
\symexamp{PAQq}{\PAQq}
\symexamp{PAQd}{\PAQd}
\symexamp{PAQu}{\PAQu}
\symexamp{PAQs}{\PAQs}
\symexamp{PAQc}{\PAQc}
\symexamp{PGne}{\PGne}
\symexamp{PAGne}{\PAGne}
\symexamp{PGnGm}{\PGnGm}
\symexamp{PAGnGm}{\PAGnGm}
\symexamp{PGnGt}{\PGnGt}
\symexamp{PAGnGt}{\PAGnGt}
\noindent%
\textcolor{gray}{\rule{\columnwidth}{0.2pt}}\\
\symexamp{AFB}{\AFB}
\symexamp{wangle}{\wangle}
\symexamp{stat}{\stat\hspace{\fill}{\tiny[Includes leading thinspace]}}
\symexamp{syst}{\syst\hspace{\fill}{\tiny[Includes leading thinspace]}}
\symexamp{thy}{\thy\hspace{\fill}{\tiny[Includes leading thinspace]}}
\symexamp{lum}{\lum\hspace{\fill}{\tiny[Includes leading thinspace]}}
\symexamp{kt}{\kt}
\symexamp{BC}{\BC}
\symexamp{bbarc}{\bbarc}
\symexamp{bbbar}{\bbbar}
\symexamp{ccbar}{\ccbar}
\symexamp{bspsiphi}{\bspsiphi}
\symexamp{EE}{\EE}
\symexamp{MM}{\MM}
\symexamp{TT}{\TT}
\symexamp{HGG}{\HGG}
\symexamp{GAMJET}{\GAMJET}
\symexamp{PPTOJETS}{\PPTOJETS}
\symexamp{PPTOGG}{\PPTOGG}
\symexamp{PPTOGAMJET}{\PPTOGAMJET}
\symexamp{MH}{\MH}
\symexamp{RNINE}{\RNINE}
\symexamp{DR}{\DR}
\symexamp{ga}{\ga}
\symexamp{la}{\la}
\symexamp{swsq}{\swsq}
\symexamp{cwsq}{\cwsq}
\symexamp{tanb}{\tanb}
\symexamp{tanbsq}{\tanbsq}
\symexamp{sidb}{\sidb}
\symexamp{alpS}{\alpS}
\symexamp{alpt}{\alpt}
\symexamp{QL}{\QL}
\symexamp{sQ}{\sQ}
\symexamp{sQL}{\sQL}
\symexamp{ULC}{\ULC}
\symexamp{sUC}{\sUC}
\symexamp{sULC}{\sULC}
\symexamp{DLC}{\DLC}
\symexamp{sDC}{\sDC}
\symexamp{sDLC}{\sDLC}
\symexamp{LL}{\LL}
\symexamp{sL}{\sL}
\symexamp{sLL}{\sLL}
\symexamp{ELC}{\ELC}
\symexamp{sEC}{\sEC}
\symexamp{sELC}{\sELC}
\symexamp{sEL}{\sEL}
\symexamp{sER}{\sER}
\symexamp{sFer}{\sFer}
\symexamp{sQua}{\sQua}
\symexamp{sUp}{\sUp}
\symexamp{suL}{\suL}
\symexamp{suR}{\suR}
\symexamp{sDw}{\sDw}
\symexamp{sdL}{\sdL}
\symexamp{sdR}{\sdR}
\symexamp{sTop}{\sTop}
\symexamp{stL}{\stL}
\symexamp{stR}{\stR}
\symexamp{stone}{\stone}
\symexamp{sttwo}{\sttwo}
\symexamp{sBot}{\sBot}
\symexamp{sbL}{\sbL}
\symexamp{sbR}{\sbR}
\symexamp{sbone}{\sbone}
\symexamp{sbtwo}{\sbtwo}
\symexamp{sLep}{\sLep}
\symexamp{sLepC}{\sLepC}
\symexamp{sEl}{\sEl}
\symexamp{sElC}{\sElC}
\symexamp{seL}{\seL}
\symexamp{seR}{\seR}
\symexamp{snL}{\snL}
\symexamp{sMu}{\sMu}
\symexamp{sNu}{\sNu}
\symexamp{sTau}{\sTau}
\symexamp{Glu}{\Glu}
\symexamp{sGlu}{\sGlu}
\symexamp{Wpm}{\Wpm}
\symexamp{sWpm}{\sWpm}
\symexamp{Wz}{\Wz}
\symexamp{sWz}{\sWz}
\symexamp{sWino}{\sWino}
\symexamp{Bz}{\Bz}
\symexamp{sBz}{\sBz}
\symexamp{sBino}{\sBino}
\symexamp{Zz}{\Zz}
\symexamp{sZino}{\sZino}
\symexamp{sGam}{\sGam}
\symexamp{chiz}{\chiz}
\symexamp{chip}{\chip}
\symexamp{chim}{\chim}
\symexamp{chipm}{\chipm}
\symexamp{Hone}{\Hone}
\symexamp{sHone}{\sHone}
\symexamp{Htwo}{\Htwo}
\symexamp{sHtwo}{\sHtwo}
\symexamp{sHig}{\sHig}
\symexamp{sHa}{\sHa}
\symexamp{sHb}{\sHb}
\symexamp{sHpm}{\sHpm}
\symexamp{hz}{\hz}
\symexamp{Hz}{\Hz}
\symexamp{Az}{\Az}
\symexamp{Hpm}{\Hpm}
\symexamp{sGra}{\sGra}
\symexamp{mtil}{\mtil}
\symexamp{rpv}{\rpv}
\symexamp{LLE}{\LLE}
\symexamp{LQD}{\LQD}
\symexamp{UDD}{\UDD}
\symexamp{Lam}{\Lam}
\symexamp{Lamp}{\Lamp}
\symexamp{Lampp}{\Lampp}
\symexamp{MD}{\MD}
\symexamp{Mpl}{\Mpl}
\symexamp{Rinv}{\Rinv}


==> test <==
This is BibTeX, Version 0.99d (TeX Live 2015)
The top-level auxiliary file: report.aux
White space in argument---line 1191 of file report.aux
 : \citation{CMS
 :               Endcap TDR}
I'm skipping whatever remains of this command
White space in argument---line 1203 of file report.aux
 : \citation{CMS
 :               ENDCAP TDR}
I'm skipping whatever remains of this command
White space in argument---line 1204 of file report.aux
 : \citation{CMS
 :               ENDCAP TDR}
I'm skipping whatever remains of this command
The style file: report.bst
Database file #1: ./bib/chapter.bib
Database file #2: ./section1/bib/section.bib
Database file #3: ./electroweak/electroweak.bib
Repeated entry---line 3634 of file ./electroweak/electroweak.bib
 : @article{Alioli:2010xd
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 3668 of file ./electroweak/electroweak.bib
 : @article{Sjostrand:2014zea
 :                           ,
I'm skipping whatever remains of this entry
Repeated entry---line 3830 of file ./electroweak/electroweak.bib
 : @article{Butterworth:2015oua
 :                             ,
I'm skipping whatever remains of this entry
Repeated entry---line 3873 of file ./electroweak/electroweak.bib
 : @article{Ballestrero:2018anz
 :                             ,
I'm skipping whatever remains of this entry
Repeated entry---line 3932 of file ./electroweak/electroweak.bib
 : @article{Agashe:2014kda
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 4002 of file ./electroweak/electroweak.bib
 : @article{Gleisberg:2008ta
 :                          ,
I'm skipping whatever remains of this entry
Repeated entry---line 4262 of file ./electroweak/electroweak.bib
 : @article{Denner:2014gla
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 4281 of file ./electroweak/electroweak.bib
 : @article{Denner:2016kdg
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 4299 of file ./electroweak/electroweak.bib
 : @article{Ossola:2007ax
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 4372 of file ./electroweak/electroweak.bib
 : @article{Denner:2005fg
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 4393 of file ./electroweak/electroweak.bib
 : @article{Harland-Lang:2014zoa
 :                              ,
I'm skipping whatever remains of this entry
Repeated entry---line 4428 of file ./electroweak/electroweak.bib
 : @article{Alwall:2014hca
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 4514 of file ./electroweak/electroweak.bib
 : @article{Cowan:2010js
 :                      ,
I'm skipping whatever remains of this entry
Repeated entry---line 4643 of file ./electroweak/electroweak.bib
 : @techreport{CERN-LHCC-2015-020
 :                               ,
I'm skipping whatever remains of this entry
Repeated entry---line 4723 of file ./electroweak/electroweak.bib
 : @article{Ridder:2015dxa
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 4786 of file ./electroweak/electroweak.bib
 : @article{deFlorian:2016spz
 :                           ,
I'm skipping whatever remains of this entry
Repeated entry---line 4800 of file ./electroweak/electroweak.bib
 : @article{Cacciari:2015jma
 :                          ,
I'm skipping whatever remains of this entry
Repeated entry---line 4819 of file ./electroweak/electroweak.bib
 : @article{Ciccolini:2007ec
 :                          ,
I'm skipping whatever remains of this entry
Repeated entry---line 4836 of file ./electroweak/electroweak.bib
 : @article{Ciccolini:2007jr
 :                          ,
I'm skipping whatever remains of this entry
Repeated entry---line 4852 of file ./electroweak/electroweak.bib
 : @article{Denner:2011id
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 4869 of file ./electroweak/electroweak.bib
 : @article{Denner:2014cla
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 4887 of file ./electroweak/electroweak.bib
 : @article{Campanario:2018ppz
 :                            ,
I'm skipping whatever remains of this entry
Repeated entry---line 4986 of file ./electroweak/electroweak.bib
 : @article{Platzer:2011bc
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 5018 of file ./electroweak/electroweak.bib
 : @article{Bellm:2017bvx
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 5031 of file ./electroweak/electroweak.bib
 : @article{Arnold:2008rz
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 5047 of file ./electroweak/electroweak.bib
 : @article{Arnold:2011wj
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 5061 of file ./electroweak/electroweak.bib
 : @article{Baglio:2014uba
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 5090 of file ./electroweak/electroweak.bib
 : @article{Cacciari:2011ma
 :                         ,
I'm skipping whatever remains of this entry
Repeated entry---line 5105 of file ./electroweak/electroweak.bib
 : @article{Cacciari:2005hq
 :                         ,
I'm skipping whatever remains of this entry
Repeated entry---line 5199 of file ./electroweak/electroweak.bib
 : @article{Cruz-Martinez:2018rod
 :                               ,
I'm skipping whatever remains of this entry
Repeated entry---line 5446 of file ./electroweak/electroweak.bib
 : @article{Alioli:2010xd
 :                       ,
I'm skipping whatever remains of this entry
I was expecting a `,' or a `}'---line 5548 of file ./electroweak/electroweak.bib
 :    
 :    %   SLACcitation   = "%%CITATION = HEP-EX/0509008;%%"
(Error may have been on previous line)
I'm skipping whatever remains of this entry
Repeated entry---line 5552 of file ./electroweak/electroweak.bib
 : @article{Aaboud:2017ffb
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 5598 of file ./electroweak/electroweak.bib
 : @techreport{CERN-LHCC-2015-020
 :                               ,
I'm skipping whatever remains of this entry
Repeated entry---line 5612 of file ./electroweak/electroweak.bib
 : @article{Alioli:2010xd
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 5630 of file ./electroweak/electroweak.bib
 : @article{Sjostrand:2007gs
 :                          ,
I'm skipping whatever remains of this entry
Repeated entry---line 5648 of file ./electroweak/electroweak.bib
 : @techreport{CERN-LHCC-2015-020
 :                               ,
I'm skipping whatever remains of this entry
Repeated entry---line 5711 of file ./electroweak/electroweak.bib
 : @article{Paukkunen:2014zia
 :                           ,
I'm skipping whatever remains of this entry
Repeated entry---line 5727 of file ./electroweak/electroweak.bib
 : @article{Alekhin:2014irh
 :                         ,
I'm skipping whatever remains of this entry
Repeated entry---line 5760 of file ./electroweak/electroweak.bib
 : @article{Khalek:2018mdn
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 5774 of file ./electroweak/electroweak.bib
 : @article{Butterworth:2015oua
 :                             ,
I'm skipping whatever remains of this entry
Repeated entry---line 5791 of file ./electroweak/electroweak.bib
 : @article{Klein:1564929
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 5816 of file ./electroweak/electroweak.bib
 : @article{Aaij:2015lka
 :                      ,
I'm skipping whatever remains of this entry
Repeated entry---line 5834 of file ./electroweak/electroweak.bib
 : @article{Aad:2015uau
 :                     ,
I'm skipping whatever remains of this entry
Database file #4: ./top/top.bib
Repeated entry---line 343 of file ./top/top.bib
 : @article{Butterworth:2015oua
 :                             ,
I'm skipping whatever remains of this entry
Repeated entry---line 843 of file ./top/top.bib
 : @article{Dulat:2015mca
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 920 of file ./top/top.bib
 : @article{ATLAS-CONF-2018-030
 :                             ,
I'm skipping whatever remains of this entry
Repeated entry---line 1114 of file ./top/top.bib
 : @article{Alekhin:2014irh
 :                         ,
I'm skipping whatever remains of this entry
I was expecting an "="---line 1514 of file ./top/top.bib
 :  *** 
 :      Not Found with lookup: 'find r FTR-16-006'
I'm skipping whatever remains of this entry
Repeated entry---line 1822 of file ./top/top.bib
 : @article{Frederix:2018nkq
 :                          ,
I'm skipping whatever remains of this entry
Repeated entry---line 1923 of file ./top/top.bib
 : @article{AguilarSaavedra:2018nen
 :                                 ,
I'm skipping whatever remains of this entry
I was expecting an "="---line 2221 of file ./top/top.bib
 :  *** 
 :      Non-standard form, no INSPIRE lookup performed ***
I'm skipping whatever remains of this entry
Repeated entry---line 2224 of file ./top/top.bib
 : @article{Patrignani:2016xqp
 :                            ,
I'm skipping whatever remains of this entry
Repeated entry---line 2343 of file ./top/top.bib
 : @article{Jezo:2016ujg
 :                      ,
I'm skipping whatever remains of this entry
Repeated entry---line 2496 of file ./top/top.bib
 : @article{Czakon:2013goa
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 2564 of file ./top/top.bib
 : @article{Czakon:2013goa
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 2582 of file ./top/top.bib
 : @article{Khachatryan:2016mqs
 :                             ,
I'm skipping whatever remains of this entry
Repeated entry---line 2606 of file ./top/top.bib
 : @article{Aad:2014kva
 :                     ,
I'm skipping whatever remains of this entry
Repeated entry---line 2686 of file ./top/top.bib
 : @article{Gao:2012ja
 :                    ,
I'm skipping whatever remains of this entry
Repeated entry---line 2705 of file ./top/top.bib
 : @article{Brucherseifer:2013iv
 :                              ,
I'm skipping whatever remains of this entry
Repeated entry---line 2724 of file ./top/top.bib
 : @article{Hoang:2017kmk
 :                       ,
I'm skipping whatever remains of this entry
I was expecting a `,' or a `}'---line 3033 of file ./top/top.bib
 : 
 : @article{Gauld:2014pxa,
(Error may have been on previous line)
I'm skipping whatever remains of this entry
You're missing a field name---line 3139 of file ./top/top.bib
 :     
 :     %doi            = "10.1140/epjc/s10052-010-1403-6",
(Error may have been on previous line)
I'm skipping whatever remains of this entry
Repeated entry---line 3161 of file ./top/top.bib
 : @booklet{ATL-PHYS-PUB-2018-009
 :                               ,
I'm skipping whatever remains of this entry
Repeated entry---line 3172 of file ./top/top.bib
 : %@booklet{CMS-PAS-TOP-12-030
 :                             ,
I'm skipping whatever remains of this entry
Database file #5: ./qcd/qcd.bib
Repeated entry---line 33 of file ./qcd/qcd.bib
 : @article{AbelleiraFernandez:2012cc
 :                                   ,
I'm skipping whatever remains of this entry
Repeated entry---line 148 of file ./qcd/qcd.bib
 : @article{Currie:2017eqf
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 157 of file ./qcd/qcd.bib
 : @article{Berger:2017zof
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 336 of file ./qcd/qcd.bib
 : @article{Paukkunen:2014zia
 :                           ,
I'm skipping whatever remains of this entry
Repeated entry---line 346 of file ./qcd/qcd.bib
 : @article{Sjostrand:2007gs
 :                          ,
I'm skipping whatever remains of this entry
Repeated entry---line 611 of file ./qcd/qcd.bib
 : @article{Bellm:2015jjp
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 631 of file ./qcd/qcd.bib
 : @article{Buckley:2010ar
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 691 of file ./qcd/qcd.bib
 : @article{Gehrmann:2018szu
 :                          ,
I'm skipping whatever remains of this entry
Repeated entry---line 713 of file ./qcd/qcd.bib
 : @article{Dulat:2015mca
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 734 of file ./qcd/qcd.bib
 : @article{Currie:2016bfm
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 757 of file ./qcd/qcd.bib
 : @article{Buckley:2014ana
 :                         ,
I'm skipping whatever remains of this entry
Repeated entry---line 777 of file ./qcd/qcd.bib
 : @article{Cacciari:2008gp
 :                         ,
I'm skipping whatever remains of this entry
Repeated entry---line 798 of file ./qcd/qcd.bib
 : @article{Currie:2018xkj
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 992 of file ./qcd/qcd.bib
 : @article{Harland-Lang:2014zoa
 :                              ,
I'm skipping whatever remains of this entry
Repeated entry---line 1015 of file ./qcd/qcd.bib
 : @article{Cacciari:2011ma
 :                         ,
I'm skipping whatever remains of this entry
Repeated entry---line 1031 of file ./qcd/qcd.bib
 : @article{Cacciari:2008gp
 :                         ,
I'm skipping whatever remains of this entry
Repeated entry---line 1150 of file ./qcd/qcd.bib
 : @article{Khalek:2018mdn
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 1183 of file ./qcd/qcd.bib
 : @article{Harland-Lang:2014zoa
 :                              ,
I'm skipping whatever remains of this entry
Repeated entry---line 1218 of file ./qcd/qcd.bib
 : @article{Dulat:2015mca
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 1237 of file ./qcd/qcd.bib
 : @article{Gehrmann:2018szu
 :                          ,
I'm skipping whatever remains of this entry
Repeated entry---line 1257 of file ./qcd/qcd.bib
 : @article{Currie:2016bfm
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 1274 of file ./qcd/qcd.bib
 : @article{Currie:2017eqf
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 1292 of file ./qcd/qcd.bib
 : @article{Currie:2018xkj
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 1476 of file ./qcd/qcd.bib
 : @article{Aaboud:2017vol
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 1530 of file ./qcd/qcd.bib
 : @article{Catani:2018krb
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 1578 of file ./qcd/qcd.bib
 : @article{Andersen:2014efa
 :                          ,
I'm skipping whatever remains of this entry
Repeated entry---line 1589 of file ./qcd/qcd.bib
 : @article{Frixione:1998jh
 :                         ,
I'm skipping whatever remains of this entry
Repeated entry---line 1635 of file ./qcd/qcd.bib
 : @article{Aad:2012tba
 :                     ,
I'm skipping whatever remains of this entry
Repeated entry---line 1652 of file ./qcd/qcd.bib
 : @article{Chatrchyan:2014fsa
 :                            ,
I'm skipping whatever remains of this entry
Repeated entry---line 1700 of file ./qcd/qcd.bib
 : @article{Diehl:2017kgu
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 1715 of file ./qcd/qcd.bib
 : @article{Buffing:2017mqm
 :                         ,
I'm skipping whatever remains of this entry
Repeated entry---line 1732 of file ./qcd/qcd.bib
 : @article{Cotogno:2018mfv
 :                         ,
I'm skipping whatever remains of this entry
Repeated entry---line 1743 of file ./qcd/qcd.bib
 : @article{Diehl:2015bca
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 1760 of file ./qcd/qcd.bib
 : @article{Diehl:2011yj
 :                      ,
I'm skipping whatever remains of this entry
Repeated entry---line 1778 of file ./qcd/qcd.bib
 : @article{Gaunt:2009re
 :                      ,
I'm skipping whatever remains of this entry
Repeated entry---line 1794 of file ./qcd/qcd.bib
 : @article{Ceccopieri:2017oqe
 :                            ,
I'm skipping whatever remains of this entry
Repeated entry---line 1811 of file ./qcd/qcd.bib
 : @misc{CMSTDR
 :             ,
I'm skipping whatever remains of this entry
Repeated entry---line 1818 of file ./qcd/qcd.bib
 : @article{Kasemets:2012pr
 :                         ,
I'm skipping whatever remains of this entry
Repeated entry---line 1833 of file ./qcd/qcd.bib
 : @article{Diehl:2013mla
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 1848 of file ./qcd/qcd.bib
 : @article{Diehl:2014vaa
 :                       ,
I'm skipping whatever remains of this entry
Database file #6: ./frwd_physics/frwd_physics.bib
Repeated entry---line 369 of file ./frwd_physics/frwd_physics.bib
 : @article{Albrow:2010yb
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 542 of file ./frwd_physics/frwd_physics.bib
 : @article{Lebiedowicz:2013ika
 :                             ,
I'm skipping whatever remains of this entry
Repeated entry---line 558 of file ./frwd_physics/frwd_physics.bib
 : @article{Lebiedowicz:2018eui
 :                             ,
I'm skipping whatever remains of this entry
Repeated entry---line 608 of file ./frwd_physics/frwd_physics.bib
 : @article{Harland-Lang:2014lxa
 :                              ,
I'm skipping whatever remains of this entry
Database file #7: ./eft/eft.bib
Repeated entry---line 34 of file ./eft/eft.bib
 : @article{AguilarSaavedra:2018nen
 :                                 ,
I'm skipping whatever remains of this entry
Repeated entry---line 141 of file ./eft/eft.bib
 : @article{AguilarSaavedra:2008zc
 :                                ,
I'm skipping whatever remains of this entry
Repeated entry---line 278 of file ./eft/eft.bib
 : @article{Sirunyan:2016cdg
 :                          ,
I'm skipping whatever remains of this entry
I was expecting an "="---line 299 of file ./eft/eft.bib
 :  *** 
 :      Not Found with lookup: 'find r Khachatryan:2017-018'
I'm skipping whatever remains of this entry
I was expecting an "="---line 330 of file ./eft/eft.bib
 :  *** 
 :      Not Found with lookup: 'find r Khachatryan:2016-023'
I'm skipping whatever remains of this entry
Repeated entry---line 533 of file ./eft/eft.bib
 : @article{Ibrahim:2010hv
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 602 of file ./eft/eft.bib
 : @article{Grzadkowski:2010es
 :                            ,
I'm skipping whatever remains of this entry
Repeated entry---line 650 of file ./eft/eft.bib
 : @article{Alwall:2014hca
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 672 of file ./eft/eft.bib
 : @article{Artoisenet:2012st
 :                           ,
I'm skipping whatever remains of this entry
Repeated entry---line 711 of file ./eft/eft.bib
 : @article{Sjostrand:2007gs
 :                          ,
I'm skipping whatever remains of this entry
Repeated entry---line 734 of file ./eft/eft.bib
 : @article{Sjostrand:2014zea
 :                           ,
I'm skipping whatever remains of this entry
Repeated entry---line 759 of file ./eft/eft.bib
 : @article{deFavereau:2013fsa
 :                            ,
I'm skipping whatever remains of this entry
Repeated entry---line 779 of file ./eft/eft.bib
 : @article{Cacciari:2011ma
 :                         ,
I'm skipping whatever remains of this entry
Repeated entry---line 796 of file ./eft/eft.bib
 : @article{Cacciari:2008gp
 :                         ,
I'm skipping whatever remains of this entry
Repeated entry---line 833 of file ./eft/eft.bib
 : @article{Aaboud:2016xve
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 855 of file ./eft/eft.bib
 : @article{Chatrchyan:2013qca
 :                            ,
I'm skipping whatever remains of this entry
Repeated entry---line 874 of file ./eft/eft.bib
 : @article{Khachatryan:2014ewa
 :                             ,
I'm skipping whatever remains of this entry
Repeated entry---line 895 of file ./eft/eft.bib
 : @article{Khachatryan:2015sha
 :                             ,
I'm skipping whatever remains of this entry
Database file #8: ./theory_tools/theory_tools.bib
Repeated entry---line 144 of file ./theory_tools/theory_tools.bib
 : @article{Cascioli:2011va
 :                         ,
I'm skipping whatever remains of this entry
Repeated entry---line 445 of file ./theory_tools/theory_tools.bib
 : @article{Dreyer:2016oyx
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 817 of file ./theory_tools/theory_tools.bib
 : @article{vanHameren:2010cp
 :                           ,
I'm skipping whatever remains of this entry
Repeated entry---line 890 of file ./theory_tools/theory_tools.bib
 : @article{Bizon:2018foh
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 1096 of file ./theory_tools/theory_tools.bib
 : @article{Chen:2018pzu
 :                      ,
I'm skipping whatever remains of this entry
Repeated entry---line 1314 of file ./theory_tools/theory_tools.bib
 : @article{Czakon:2017wor
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 1452 of file ./theory_tools/theory_tools.bib
 : @article{Aaltonen:2018dxj
 :                          ,
I'm skipping whatever remains of this entry
Repeated entry---line 1519 of file ./theory_tools/theory_tools.bib
 : @article{Dulat:2015mca
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 1530 of file ./theory_tools/theory_tools.bib
 : @article{Harland-Lang:2014zoa
 :                              ,
I'm skipping whatever remains of this entry
Repeated entry---line 1540 of file ./theory_tools/theory_tools.bib
 : @article{Currie:2016bfm
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 1551 of file ./theory_tools/theory_tools.bib
 : @article{Ball:2017nwa
 :                      ,
I'm skipping whatever remains of this entry
Repeated entry---line 1587 of file ./theory_tools/theory_tools.bib
 : @article{Czakon:2016dgf
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 1653 of file ./theory_tools/theory_tools.bib
 : @article{Czakon:2018nun
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 1676 of file ./theory_tools/theory_tools.bib
 : @article{Mangano:2016jyj
 :                         ,
I'm skipping whatever remains of this entry
Repeated entry---line 2187 of file ./theory_tools/theory_tools.bib
 : @inproceedings{Badger:2016bpw
 :                              ,
I'm skipping whatever remains of this entry
Repeated entry---line 2307 of file ./theory_tools/theory_tools.bib
 : @article{Barze:2012tt
 :                      ,
I'm skipping whatever remains of this entry
Repeated entry---line 2393 of file ./theory_tools/theory_tools.bib
 : @article{AguilarSaavedra:2018nen
 :                                 ,
I'm skipping whatever remains of this entry
Repeated entry---line 2574 of file ./theory_tools/theory_tools.bib
 : @article{Bellm:2015jjp
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 2836 of file ./theory_tools/theory_tools.bib
 : @article{Zhang:2016omx
 :                       ,
I'm skipping whatever remains of this entry
Repeated entry---line 2854 of file ./theory_tools/theory_tools.bib
 : @article{Bylund:2016phk
 :                        ,
I'm skipping whatever remains of this entry
Repeated entry---line 2892 of file ./theory_tools/theory_tools.bib
 : @article{Degrande:2018fog
 :                          ,
I'm skipping whatever remains of this entry
Repeated entry---line 2911 of file ./theory_tools/theory_tools.bib
 : @article{deBeurs:2018pvs
 :                         ,
I'm skipping whatever remains of this entry
Warning--I didn't find a database entry for "Bauer:xxx"
Warning--I didn't find a database entry for "allyourbases"
Warning--I didn't find a database entry for "atlas-higgs"
Warning--I didn't find a database entry for "cms-higgs"
Warning--I didn't find a database entry for "CMSPaperCombinationLong"
Warning--I didn't find a database entry for "PhysRevD.87.093005"
Warning--I didn't find a database entry for "PhysRevD.87.055017"
Warning--I didn't find a database entry for "ATL-PHYS-PUB-2018-030"
Warning--I didn't find a database entry for "STDM-2015-07"
Warning--I didn't find a database entry for "Schonherr:2018"
Warning--I didn't find a database entry for "Grojean:2018dqj"
Warning--I didn't find a database entry for ""
Warning--I didn't find a database entry for "TOP-16-008"
Warning--I didn't find a database entry for "TOP-17-002"
Warning--I didn't find a database entry for "tracker"
Warning--I didn't find a database entry for "barrel"
Warning--I didn't find a database entry for "endcap"
Warning--I didn't find a database entry for "muon"
Warning--I didn't find a database entry for "PUPPI"
Warning--I didn't find a database entry for "ATLAS-PUB-4top"
Warning--can't use both volume and number fields in pordes2007open
You can't pop an empty literal stack for entry Sirunyan:2278242
while executing---line 1208 of file report.bst
Warning--empty author in UpgradeFunctions
Warning--empty author in BosonTagPreRec
Warning--empty author in CMS:2017adb
Warning--empty author in ATL-PHYS-PUB-2017-023
Warning--empty booktitle in SchwanTalk
`howpublished' is a missing field, not a string, for entry CERN-ATS-2012-236
while executing---line 1208 of file report.bst
`howpublished' is a missing field, not a string, for entry CERN-ACC-2015-0140
while executing---line 1208 of file report.bst
You can't pop an empty literal stack for entry PhysRevLett.103.082001
while executing---line 1208 of file report.bst
Warning--empty author in CMS-PAS-SMP-16-007
Warning--empty author in CMS-PAS-SMP-17-014
`howpublished' is a missing field, not a string, for entry nason
while executing---line 1208 of file report.bst
Warning--all relevant fields are empty in nason
Warning--empty publisher in Nason:2017cxd
`howpublished' is a missing field, not a string, for entry HLLHCSystRecommendations
while executing---line 1208 of file report.bst
Warning--empty author in LHCb-PII-Physics
Warning--empty author in ATLAS:2018ac006
Warning--empty author in ATLAS:2018bpl
Warning--empty author in ATLAS:2018xcf
You can't pop an empty literal stack for entry PhysRevD.2.1285
while executing---line 1208 of file report.bst
You can't pop an empty literal stack for entry PhysRevD.44.1473
while executing---line 1208 of file report.bst
Warning--empty author in ATL-PHYS-PUB-2016-019
Warning--empty author in ATL-PHYS-PUB-2013-012
`howpublished' is a missing field, not a string, for entry Khachatryan:2017-018
while executing---line 1208 of file report.bst
Warning--all relevant fields are empty in Khachatryan:2017-018
`howpublished' is a missing field, not a string, for entry Khachatryan:2016-023
while executing---line 1208 of file report.bst
Warning--all relevant fields are empty in Khachatryan:2016-023
(There were 162 error messages)


==> theorists.tex <==
\author{{\bf Editors and Conveners:} \\
{\rm 
Patrizia Azzi$^1$, Stephen Farry$^2$, Paolo Nason$^3$, Alessandro Tricoli$^4$, Dieter Zeppenfeld$^5$ 
}
\\
{\bf Contributors:} {\rm 

A. Denner,                           00076731    Ansgar.Denner.1
A. Ferroglia,                        00053574    A.Ferroglia.1
A. Hoang,                            00379674    A.H.Hoang.1
A. Huss,                             00397696    A.Huss.1
A. Karlberg (VBF)                    00245334    A.Karlberg.1
A. Mitov,                            00055444    A.Mitov.1
A. Papanastasiou                     00415760    A.S.Papanastasiou.1
A. Vicini                            00320190    A.Vicini.1
D. Pagani,                           00418125    D.Pagani.1       
E. Franco,                           00082153    E.Franco.1
E. Re,                               00347723    Emanuele.Re.1
E. Vryonidou (EFT),                  00383402    E.Vryonidou.1
F. Caola,                            00016890    F.Caola.1
F. Piccinini,                        00116245    F.Piccinini.1
F. Rikkert,                          00030894    Rikkert.Frederix.1
G. Corcella,                         00074472    G.Corcella.1
G. Ferrera,                          00176935    Giancarlo.Ferrera.1
G. Zanderighi (QCD calculations),    00138061    G.Zanderighi.1
H. Yokoya,                           00137569    H.Yokoya.2
I. M. Lewis,                         00228845    I.M.Lewis.1
J. Baglio                            00225573    J.Baglio.1
J. Gao,                              00396468    Jun.Gao.1
J. Gaunt                             00414088    J.R.Gaunt.1
J. M. Cruz-Martinez,                 00487210    J.M.Cruz.Martinez.1
J. Pires,                            00416457    Joao.Pires.1
J. Rojo                              00355525    J.Rojo.1
J. de Blas,                          00053038    J.de.Blas.1
L. Cieri,                            00414259    L.Cieri.1
L. Harland-Lang,                     00433911    L.A.Harland.Lang.1
L. Reina,                            00119566    L.Reina.1
L. Silvestrini (EW Fit),             00126473    L.Silvestrini.1
M. Ciuchini,                         00164508    Marco.Ciuchini.1
M. Czakon,                           00405905    M.Czakon.1
M. Grazzini,                         00415500    M.Grazzini.1
M. Pellen,                           00476960    M.Pellen.1
M. Rauch                             00058274    Michael.Rauch.1
M. Sch\"onherr                       00399234    M.Schonherr.1
M. Wiesemann,                        00486920    M.Wiesemann.1
M. Zaro,                             00180631    M.Zaro.1 
P. Nason,                            00110545    P.Nason.1
S. Dawson,                           00155294    Sally.Dawson.1
S. Kallweit (Dibosons - Matrix),     00437098    S.Kallweit.1
T. Figy,                             00056260    T.M.Figy.1



==> top/top_xsec/top_xsec_v2.tex <==
\subsection{Top Cross Section contribution for V2 version}

{\bf **** Missing Contribution expected by ATLAS on single top}
% single-top physics specific
\subsubsection{Single top production ATLAS}
\emph{Contributors: ***********}

Among other interesting features, single top-quark $s$-channel production is sensitive
to new particles proposed by several beyond SM models, such as charged Higgs or
$W'$ production\cite{charged_higgs_wprime}.  Furthermore, it provides, as well
as the other two production channels, a direct determination of the absolute
value of the CKM matrix element $V_{tb}$ without the assumption of three quark
families.  Single top-quark production was first observed by the CDF and D0
collaborations in combined measurements of the $s$ and
$t$-channel~\cite{d0_obs,cdf_obs}. Recently, evidence for the $s$-channel alone
was reported in a combination of the results from both
collaborations~\cite{comb_sch}. At the Large Hadron Collider (LHC) the
production of single top-quarks was studied in a search at $\sqrt{s} =
{8}\text{TeV}$, using an integrated luminosity of
${20.3}{\mbox{fb$^{-1}$}}$~\cite{atlas_bdt8tev}.  This study was based on a Boosted
Decision Tree (BDT) event classifier and led to an upper limit of
${14.6}\text{pb}$ at the 95\% confidence level.  The obtained cross-section was
$\sigma_{s\text{-channel}} = 5.0 \pm {4.3}\text{pb}$ with an observed signal significance of
$1.3 \sigma$. Another ATLAS measurement in the $s$-channel was performed, using
the Matrix Element Method (MEM) instead of a BDT analysis~\cite{atlas_mem8tev}.
This measurement, using the same dataset, resulted in an observed cross-section
of $\sigma_{s\text{-channel}} = 4.8 \pm 0.8 \text{(stat.)} \pm 1.6 \text{(syst.)}$ pb.
The signal significance was observed to be $3.9\sigma$.

%common material for ATLAS
Following the end of Run 3, the LHC will be upgraded to the High-Luminosity LHC
(HL-LHC), significantly increasing the instantaneous luminosity of the LHC
machine~\cite{hllhc_refs}.
Upgrades of the ATLAS detector will be necessary to maintain its performance in
the higher luminosity environment and to mitigate the impact of radiation damage
and detector aging~\cite{atlas_phase2_refs}. A new inner tracking system,
extending the tracking region from $|\eta| < 2.7$ up to $|\eta| < 4$, will provide
the ability to reconstruct forward charged particle tracks, which can be matched
to calorimeter clusters for forward electron reconstruction, or associated to
forward jets. The inner tracker extension also enables muon identification at
high pseudorapidities if additional detectors are installed in the region
$2.7<|\eta|<4$~\cite{muonUpgradeTwiki}.

The following section describes the prospects for measurement of the $s$-channel
production cross-section at the HL-LHC, using the full expected luminosity of
${3000}{\mbox{fb$^{-1}$}}$ of proton-proton collisions at $\sqrt{s} =
{14}\text{TeV}$ with $\langle \mu \rangle = 200$. The strategy follows closely the
Run 1 analyses mentioned above, and uses a BDT rather than the MEM
approach.

%Can be made common for all ATLAS analyses
Samples used in ATLAS upgrade studies are based
on related $\sqrt{s}={13}\text{TeV}$ samples used for Run 2 analysis.
The mass of the top quark is set to {172.5} {GeV} in all of the top quark
samples here.

%s-channel
Signal events from $s$-channel production were generated using the Powheg-box
v2 generator for matrix element (ME) generation interfaced with Pythia 8 for parton
showering (PS), hadronization, and underlying event
generation~\cite{powhegbox,pythia8}. The NNPDF NLO 3.0 PDF set is used in ME
generation, and NNPDF LO 2.3 is used in the shower generator~\cite{NNPDF}.  The
A14 tune is used for the underlying event and other
tunable parameters~\cite{A14tune}.

%t-channel
Background $t$-channel events are generated also using the Powheg-box v2
generator for ME generation interfaced with Pythia 8 for PS, hadronization, and
underlying event generation. The 4-flavor numbering scheme is used to generate
this process, and the PDF and tune choice
is the same as for $s$-channel above.

%tW
Production of $tW$ events is simulated using Powheg-box v1 with the CT10 PDF set,
interfaced to Pythia 6 with Perugia P2012C tune. Overlap with the $t\bar{t}$ sample
is addressed using the diagram removal (DR) scheme.

%ttbar
Top quark pair-production is simulated using the Powheg-box v2 generator for
ME generation interfaced with Pythia 8 for PS, hadronization,
and underlying event generation, using NNPDF NLO 3.0 with the A14 tune and NNPDF
LO 2.3 for ME and PS respectively.

%W+jets
The $W+$jets samples are simulated in slices of $H_T$ and separated with $B$,
$C$, or light filters using MadGraph interfaced with Pythia 8~\cite{Madgraph}.
%Z+jets
The $Z/\gamma^{*}+$jets/Drell-Yan samples are produced inclusively, using
Powheg-box with Pythia 8.  For diboson production, Sherpa 2.2.2 with the CT10
PDF set is used.

%Also common for ATLAS
Electrons, muons, and jets in ATLAS upgrade studies are reconstructed starting with particle-level
information from MC simulation, then direclty applying parameterized smearing
and efficiency corrections to simulate reconstructed objects.

Electrons and muons are required to have $p_{\text{T}} > {25}\text{GeV}$ and pseudorapidity
$|\eta| < 4.0$, electrons from the calorimter crack region ($1.37<|\eta|<1.52$) rejected.
Selected electrons also include contributions from light-flavor jets
faking electrons (both pileup and hard-scatter jets).

Jets are selected with $p_{\text{T}} > {25}\text{GeV}$, in pseudorapidity range $|\eta| < 4.0$.
Additionally, the collection of selected jets includes simulated pileup effects
for HL-LHC ($\langle \mu \rangle =200$) conditions. A track-based pileup jet
rejection technique is simulated, assuming 2\% efficiency to select a pileup jet
as a real hard-scatter jet.
Jets are $b$-tagged using the \texttt{mv2c10} algorithm at a 70\% efficient
working point. Both pileup and hard-scatter jets may be tagged or mis-tagged.
$E_{\text{T}}^{\text{miss}}$ is simulated with parameterized contributions to soft terms.

%%%%%%%%%%%%%%%%%%%%%%%%
%s-channel specific parts
%%%%%%%%%%%%%%%%%%%%%%%%
Events with exactly one lepton with $p_{\text{T}}>{25}\text{GeV}$ and two $b$-tagged jets are accepted
as signal region events (2j2b region). These lepton and jets must fall within
$|\eta|<2.5$ (forward leptons and jets are counted and used in the
signal/background discriminant, described later) Additionally, minimal
requirement are placed on $E_{\text{T}}^{\text{miss}}$ and $m_t(W)$, requiring both $E_{\text{T}}^{\text{miss}}>{20}\text{GeV}$
and $m_t(W)>{20}\text{GeV}$.

This study uses the TMVA~\cite{TMVA} package
to train a gradient-boosted decisions tree discriminant.
A list of input variables is developed from combinations of the
four-vectors of the lepton, two jets, and $E_{\text{T}}^{\text{miss}}$ in the event.  Where $E_{\text{T}}^{\text{miss}}$ needs
to be treated as a 4-vector, it is considered massless and points along the
transverse plane.  Also included in the list are variables such as thrust\footnote{%
    The thrust vector $T$ is defined as $T= \max_{|n|=1} \frac{\sum_i |p_i n|}{\sum_i |p_i|}$
    where $n$ is a unit vector called the thrust axis, the sums iterate over all relevant
    particles, and $p_i$ are the particle momentum vectors.}%
    and centrality (transverse momentum divided by total momentum).
BDTG hyperparameters are optimized by sequentially scanning 2D slices of the
parameter space. In each scan, overtrained points are rejected with a KS test
filter requiring $p>0.1$, and the point with the largest area under curve of
signal efficiency versus background rejection proceeds to the next round of the
scan. The final list consists of 21 variables, with the most significant being
$\Delta \phi (\ell, j_1)$, the thrust magnitude, and the lepton centrality.

Systematic uncertainties in this study are extrapolated from the {8} {TeV} MEM
analysis~\cite{atlas_mem8tev}.  In addition to the conventions applied to
systematic uncertainties in other ATLAS upgrade studies, shape uncertainties are
considered for a few systematic effects.  An ad-hoc shape uncertainty is applied
for uncertainties that were considered significant in the Run 1 analysis,
constructing a weighting function to generate a sloped shape uncertainty.
Different functional forms are chosen for each shape uncertainty for a given
sample.  The shape uncertainties which are considered include jet energy
resolution, various components of the jet energy scale, and the
muon $p_{\text{T}}$ scale.

A fit is performed with a single signal region
(2j2b) as opposed to Run 1 analyses which used a control region in addition.
This is because of the more than adequate statistics in the signal region, which
are able to constrain all background uncertainties well enough.  Although a very
large number of bins could be used in a future HL-LHC analysis, the limitations
of MC statistics and the ad-hoc approach to shape uncertainties motivate a more
conservative binning, so a total of 20 bins are used. The pre-fit distribution
of the BDT discriminant are shown in Figure~{\ref{fig:sch_prefit}}.

\begin{figure}[ht]
	%no graphic available right now
    %\begin{tabular}{cc}
        %\includegraphics[width=.45\textwidth]{fitter/Plots/SR} \\
    %\end{tabular}
    \caption{BDT response distribution with binning used in likelihood fit,
    pre- and post-fit uncertainty bands}
    \label{fig:sch_prefit}
\end{figure}

Many parameters are heavily constrained in fit, particularly the
normalization-only uncertainties.
The highest-impact uncertainties are $s$-channel scale variation and $tW$
cross-section. It is important to emphasize that these uncertainties are
normalization-only effects, so their large rank is not necessarily indicative
of any physics effects of $s$-channel modelling, simply that large normalization
uncertainties on the $s$ channel process translate to large uncertainties
on the total cross-section measurement.
The final expected cross-section uncertainty with 3000 \mbox{fb$^{-1}$} at 14 {TeV} is:\\
$\sigma/\sigma_{\text{expected}} = 1 \pm 2.13\%$\\

%%End of ATLAS s-channel text

{\bf **** Missing Contribution expected by ATLAS on ttgamma}

{\bf **** Missing Contribution expected by CMS on ttZ}

{\bf **** Missing Contribution expected by ATLAS on 4tops}

{\bf **** Missing contribution expected by CMS on 4 tops}

